Parallel Range, Segment and Rectangle Queries with Augmented Maps

The range, segment and rectangle query problems are fundamental problems in computational geometry, and have extensive applications in many domains. Despite the significant theoretical work on these problems, efficient implementations can be complicated. We know of very few practical implementations of the algorithms in parallel, and most implementations do not have tight theoretical bounds. We focus on simple and efficient parallel algorithms and implementations for these queries, which have tight worst-case bound in theory and good parallel performance in practice. We propose to use a simple framework (the augmented map) to model the problem. Based on the augmented map interface, we develop both multi-level tree structures and sweepline algorithms supporting range, segment and rectangle queries in two dimensions. For the sweepline algorithms, we propose a parallel paradigm and show corresponding cost bounds. All of our data structures are work-efficient to build in theory and achieve a low parallel depth. The query time is almost linear to the output size. We have implemented all the data structures described in the paper using a parallel augmented map library. Based on the library each data structure only requires about 100 lines of C++ code. We test their performance on large data sets (up to $10^8$ elements) and a machine with 72-cores (144 hyperthreads). The parallel construction achieves 32-68x speedup. Speedup numbers on queries are up to 126-fold. Our sequential implementation outperforms the CGAL library by at least 2x in both construction and queries. Our sequential implementation can be slightly slower than the R-tree in the Boost library in some cases (0.6-2.5x), but has significantly better query performance (1.6-1400x) than Boost.

==> algo.tex <==
\begin{newpart}
\section{Algorithms and Functions}
\label{sec:algorithm}

In this section we introduce the functions supported by our library and briefly describe the algorithms to implement them.
Some of the contents are just revisited version of \cite{ours}.


\subsection{Subroutines: Join, Split and Join2}

In our library, the only subroutine that needs to be implemented differently for each balancing scheme is \join$(T_L,k,T_R)$ which takes a key $k$ and two ordered sets L and R such that
$L < k < R$ and returns the union of the keys. However the intuition for all the four balancing scheme is similar. Suppose that $T_L$ is larger\footnote{The definition of ``larger'' varies for different schemes, e.g., for height balanced trees, ``larger'' means to have a larger height. }, then we need to go along the right spine of $T_L$ until a node $v$ that is balanced with $T_R$, is found,. We then connect $v$ and $T_R$ by $k$ at this point. Note that now $k$ is a valid balanced BST, and $k$ then take the original position of $v$. Now imbalance may occur at $k$'s (original $v$'s) parent. Thus some rotation are required to keep the tree valid, and this varies for different schemes. When $T_R$ is larger the algorithm is symmetric. Note that for treaps the decision to go left or right can occur in an interleaving way if $k$ is not the most prior one among all nodes.

Some properties of tree nodes (e.g., height, size) are changed during the rotation. Note that only those nodes along the path from the root to the connecting point need to get updated. Thus we call the private method \texttt{update} for all nodes along the way rotating back to the root.

Based on \join{}, the split function can be implemented generally across balancing schemes. This function takes a BST $T$ and a key $k$ as input, and returns a triple $(T_L, b, T_R)$, where $T_L (T_R)$ is a tree containing all keys in $T$ that are smaller (larger) than $k$, and $b$ is a flag indicating whether $k \in T$. It basically searches $k$ in $T$ and then merges all subtrees on the left (right) side of the searching path by \join{} respectively (using keys on the path as intermediate nodes) from bottom to top.

The function \joinTwo{} is similar to \join{} except that it does not have a middle key. This function first split out the last key $k'$ of the left tree and then call \join{} on the left tree without $k'$, $k'$ and the right tree together.

More algorithmic details of the three functions can be seen in \cite{ours}.

---
\subsection{Basic Tree Operations: Insert, Delete and Find}
As a library based on BSTs, our implementation also supports basic tree operations such as insertion, deletion and searching. These three functions are all methods of a tree-implemented ordered sets. The function \find{} takes a key $k$ as input and returns the pointer to the entry in the tree whose key is $k$ if $k$ exists and a null pointer otherwise.

As for insertion and deletion, besides the classic implementation that deals with different balancing conditions separately, we also support a version of general \insertnew{} and \delete{} functions using \join{} as subroutine such that it leaves all balancing issue to the \join{} function. When inserting a key $k$ into a tree, the tree is first split by $k$ into two parts. Then the two parts are connected by $k$ using \join{}. Similarly when deleting a key $k$ in the tree is first split into two parts by $k$ and then re-connected directly excluding $k$ using \joinTwo{}.

---
\subsection{Set Operations: Union, Intersection and Difference}
The library also supports set functions such as \union{}, \intersect{} and \difference{}. Those functions are defined as usual, and for maps, they are on the level of keys. They are also implemented based on the \join{} function, so they are general across balancing schemes.

As an example, we only introduce the algorithm of \union{} here, and the details can be found in \cite{ours}. This function takes two sets (maps) as input and returns a new set contains all keys appear in either set (map) using a classic divide-and-conquer scheme. It first \split{} $T_1$ by the root of $T_2$, and then \union{} the left result of \split{} with $T_2.lc$ and the right result of \split{} with $T_2.rc$. Then the results of the two \union{} are connected with $T_2.root$ by \join{}.

For set functions defined on maps, we specially support another version of \union{} and \intersect{} which takes a binary operation $g(\cdot,\cdot)$ as an extra parameter. This binary operation takes two operands of the value type of the map and returns a result of the same type. In \union{}$(T_1,T_2)$ or \intersect{}$(T_1,T_2)$, if $(k,v_1)\in T_1$ and $(k,v_2)\in T_2$, then in the result tree, the value assigned to key $k$ is $g(v_1,v_2)$. This can be done simply by returning the value of the input key in \split{} (if it is found). If \split{} finds the key in $T_1$, this means that the key of the root of $T_2$ appears in both maps, and hence we re-calculated the value by $g(\cdot,\cdot)$ before the very last \join{}.

\subsection{Tree Construction}

\end{newpart}


==> application-backup.tex <==
\begin{newpart}
\section{Applications}

\subsection{2D Range Query}

Given a set of points $P=\{p_i=(x_i, y_i)| 0\le i < n\}$ on a 2D planar, each is assigned a weight $w_i$, a range query asks the following problem: given the horizontal and vertical range $(x_L, x_R)$ and $(y_L, y_R)$ respectively, report the sum of the weight of all points inside the rectangle restricted by the two ranges, namely,
$$\sum_{{\mbox{\tiny$\begin{array}{c}
x_L\le x_i \le x_R\\
y_L\le y_i \le y_R\end{array}$}}}w_i$$

Many tree structures are designed specially for or can be adapted to this problem. In this section, we introduce two data structures implemented under our framework, which utilize the property of our augmented tree.

\para{Prefix-Union Trees (correct name?).} This data structure is a series of trees. Assume that all points in $P$ are sorted by the x-coordinate, which means $\forall i, j$ where $i<j$, we have $x_i\le x_j$. Then each point is assigned a BST $T_i$ storing all points $\{(x_j, y_j)|1\le j\le i\}$. This means that $T_i$ stores the ``prefix sum (union)'' of the points prior to it. We call $T_i$ \emph{prefix-union trees}. In these prefix-union trees, elements are organized by the key of y-coordinate, and the weight as value. If we define the reduction operation to be ``add'', then because of the augmenting property of the tree, the total weight of all points in a subtree can be returned in constant time given the pointer to the subtree root. To report the total weight of points in the box of $(x_L, x_R, y_L, y_R)$, we first binary search $x_L$ and $x_R$ in the sequence of $\{x_i\}$, which means to find $l$ and $r$ that satisfy $x_l<x_L\le x_{l+1}$ and $x_r\le x_R< x_{r+1}$. We can narrow the range of x-coordinate into $(x_L,x_R)$ by looking at only the points in $T_r-T_l$. Then the final answer is to report the sum of weight of all points within range of $(y_L,y_R)$ in $T_r-T_l$.
%$(T_r-T_l).$\texttt{range}$(y_L,y_R)=T_r.$\texttt{range}$(y_L,y_R)-T_l.$\texttt{range}$(y_L,y_R)$.

\emph{Tree Construction.} From a practical point of view, we do not calculate the prefix union one by one, which means to insert $(x_i, y_i)$ into $T_{i-1}$ to get $T_i$ because it lacks parallelism. Instead, after sorting all points by x-coordinate, we partition all points into $k$ blocks, each block having $t=\lfloor\frac{n}{k}\rfloor$ points. Points from $p_{(j-1)t}$ to $p_{jt-1}$ are in block $k$. We first build $k$ small trees $T'_{i}$ ($0\le i \le k$) corresponding to the $k$ blocks in parallel using \texttt{build\_fast}. This takes work $O(k\cdot \frac{n}{k}\log \frac{n}{k})=O(n\log \frac{n}{k})$ and depth $O(\log \frac{n}{k})$.

Next, we compute the prefix union among these $k$ small trees. These trees are the exact prefix-union trees of $T_{jt}$. This can be done sequentially using $T_{jt}=$\texttt{union}$(T_{(j-1)t}, T'_{j})$. Consider that the work of union is $O\left(m\log (\frac{n}{m}+1)\right)$, the total cost of this step is bounded by:
\begin{align*}
&c\sum_{i=1}^{k} t\log (\frac{it}{t} +1)\\
=&ct\sum_{i=1}^{k} \log (i+1)\\
=&O(n\log k)
\end{align*}
, where $c$ represents the constant hidden by big-O. The depth is:
\begin{align}
&\sum_{i=1}^{k}\log t \log it\\
=&\log t\cdot \left(k\log t+\sum_{i=1}^{k}\log i\right)\\
=&k\log \frac{n}{k}\left(\log \frac{n}{k}+\log k\right)\\
=&O(k\log \frac{n}{k}\log n)
\end{align}
%$O(k\log \frac{n}{k}\log n)$.

In the final step we build all the other prefix-union trees based on the above-built $T_{jt}$ in the corresponding blocks. All the $k$ blocks can be done in parallel. In each block, the points $p_i$ are inserted in order sequentially into its previous tree $T_{i-1}$. The total work is bounded by:
\begin{align*}
c'\sum_{i=1}^{n} \log i=O(n\log n)
\end{align*}
, where $c'$ represents the constant hidden by big-O. The depth can be reduced to $O(\frac{n}{k}\log n)$.

In total, this process costs work $O(n\log n)$ and depth $O(k\log^n+\frac{n}{k}\log n)$. When $k=\Theta(\sqrt{\frac{n}{\log n}})$, the depth is $O(\sqrt{n}\log^{1.5}n)$.

In practice, we set $k=O(p)$ where $p$ is the number of available cores.

\emph{Answering Queries.} With the prefix-union tree constructed, we can answer a query in $O(\log n)$ time. We first see how to return the total weight of all nodes in a certain range $(y_L,y_R)$ of y-coordinate in a single prefix-union tree. This is the same as in 1D range tree: we search $y_L$ and $y_R$ in the tree until we get a node $v_{\tiny\mbox{split}}$ that $y_L$ and $y_R$ go to different subtrees; then we continue to search $y_L$ in the left subtree, and if we go left, report the sum (the \texttt{accumulation} field) of weights in the right subtree. Similarly we continue to search $y_R$ in the right subtree, and report the accumulation in the left tree when we go right. %We call this process \texttt{reportRange}$(y_L,y_R)$.

As for prefix-union trees, the query an be answered by simply binary search $x_L$ and $x_R$ in the sequence of $\{x_i\}$, which means to find $l$ and $r$ that $x_l<x_L\le x_{l+1}$ and $x_r\le x_R< x_{r+1}$. Then we report the sum of weights of all nodes within range $(y_L,y_R)$ in $T_{x_l}$ and $T_{x_r}$ respectively, and the difference of the two weight sums is the answer. Two independent binary searches costs work $O(\log n)$ respectively, and reporting the answer for y-coordinate in each tree costs work $O(\log n)$. Thus total cost of a single query is $O(\log n)$.

\par

\para{Range Tree.}
Range tree is a two-level tree structure. It stores all the input points by the key of the x-coordinate on its first level (the main tree), and each node $v$ in the tree has a pointer to an associated tree (the second-level tree), storing all nodes in the subtree of the main tree rooted at $v$ but using the y-coordinate as key. Then the range query can be done by two nested queries on x- and y-coordinate respectively.

There has been plenty of studies on range trees, both sequentially and in parallel. Sequential range tree construction and query algorithms can be found in many papers and text books \cite{bentley1979data,de2000computational,samet1990design}. The construction time of In distributed system, recent work~\cite{agarwalparallel} has shown that both the construction and query of a 2-D range tree can be done in constant rounds. The pre-processing can be done within $O(n\log^2 n)$ work and $O(s\log^2 s)$ time where $n$ is the total number of points in the tree and $s$ is the number of points stored in each machine, and each query takes $O(\log^2 n+k)$ work and $O(\log n+k)$ time. There also have been works on I/O efficient range trees \cite{arge2002external}.

\emph{Tree Construction.} The associated tree of each node $v$ stores all the nodes in $v$'s two children, which is exact the \union{} of the associated trees of $L(v)$ and $R(v)$. Thus we can implement the range tree under our augmented tree framework. As shown in Figure \ref{fig:range_tree}, the first level tree (\texttt{range\_tree}) is an augmented tree whose keys are points (sorted by the comparison function on x-coordinate). The value, as well as the accumulation of each node, are of the type of another augmented tree (\texttt{sec\_tree}) which stores the y-coordinate as key and the weight of the node as value. Especially, the value of each node is a singleton of this node's y-coordinate and weight. The accumulation, which is also the associated tree of each node, is then the \union{} of the two accumulations of its children and its own value.
%basicstyle=\ttfamily\small
%\renewcommand\ttdefault{Computer Modern Typewriter}
\begin{figure*}[!h!t]
\ttfamily\small
\begin{lstlisting}[language=C, frame=lines]
struct Point {
    value_type x, y, w;
    bool operator < (const Point& p) const {
        return x < p.x;
    }
};
using y_type=int;
using w_type=int;

template<typename value_type> struct add_op {
    int operator() (value_type a, value_type b) {
        return a+b;
    }
};
template<typename K, typename V, typename Op> struct union_op {
    augmented_map<K, V, Op> operator() (augmented_map<K, V, Op> a, augmented_map<K, V, Op> b) {
		Op op;
		return map_union(a, b, op);
    }
};

augmented_map<y_type, w_type, add_op<value_type> > sec_tree;
augmented_map<Point, sec_tree, union_op<y_type, w_type, add_op<int> > > range_tree;
\end{lstlisting}
\caption{The data structure of the range tree under our augmented tree framework.}
\label{fig:range_tree}
\end{figure*}

Note that unlike the conversional range trees which only store the data in the leaves, our general framework requires every node to store a key-value pair in it. This allows the tree rotation, which means the tree can be easier updated dynamically.

\para{Experiments.} We implement both augmented tree node inherited from our AVL tree node.
\end{newpart} 

==> application1.tex <==
\section{2D Range Query}
\label{sec:range}

Given a set of points $P=\{p_i=(x_i, y_i)~|~0\le i < n\}$ in the
plane, each with weight $w_i$, a \emph{range query} asks for
some information (e.g., count, weight sum, or the full list) of points within a rectangle defined by a horizontal range
$(x_L, x_R)$ and vertical range $(y_L, y_R)$.  \hide{More formally:
$$\sum_{{\mbox{\tiny$\begin{array}{c}
x_L\le x_i \le x_R\\
y_L\le y_i \le y_R\end{array}$}}}w_i$$
}
In real settings the x- and y-coordinates can be of different types, but are necessary to be ordered. We assume $x_i\in X$, $y_i\in Y$ where $X$ and $Y$ are two sets with total order defined by $<_X$ and $<_Y$ respectively. $w_i\in W$ is not necessarily to be ordered, but need to be able to be accumulated by function $+_W$.
In this paper we discuss two algorithms addressing
this problem: 2D range tree \cite{de2000computational,samet1990design} and a sweepline algorithm.
%We also show how to update the range tree dynamically with reasonable (logarithmic) cost in Section \ref{sec:rangetree}.

\subsection{2D Range Tree}
\label{sec:rangetree}
The 2D range tree is a two-level tree structure.  The outer tree stores all the input points ordered by
x-coordinate, and each node in this tree stores
an inner tree with all nodes in its
subtree ordered by y-coordinate.  Then a range query can be done by
two nested queries on x- and y-coordinate respectively. It can answer many sorts of queries including reporting the count, weight sum or the full list of all points in the query window.
%Construction time and query time in the sequential setting is $O(n\log
%n)$ and $O(\log^2 n)$ respectively (although the query time can be
%reduced to $O(\log n)$ with reasonably complicated approaches).

Applying PAM to 2D range tree is relatively straight-forward \cite{ourppopp}. It only requires to set the key of the outer tree to be the coordinate of a point (sorted by x-coordinate) and the value to be the weight. The augmented value of a tree node is
the inner tree, containing all points in its subtree but sorted by y-coordinate. The base function of the outer tree is just a singleton on the point stored in the node itself
and the combine function is the union. Considering the persistence of PAM library, in real implementation, taking the union of the inner trees of the two children would create a new version of map for the augmented value of the parent node, without affecting the two input inner trees.
The augmented map structure on a 2D range tree is shown below. Here $\boldsymbol{M_{\text{Rin}}}$ and $\boldsymbol{M_{\text{Rout}}}$ are the inner and outer tree respectively.
%For completeness, we give detailed introduction of applying PAM to 2D range tree in Appendix \ref{app:rangetree}.
\hide{\mapstructure{
{\small
\begin{tabular}{|r@{ }@{ }c@{ }@{ }c@{ }llllllll|}
  \hline
  $\boldsymbol{M_{\text{Rin}}}$ &=& (& $X\times Y$; &$W$; &$<_{Y}$;&  $W$;& $(k,v)\mapsto v$; &$+_W$; & $0$ &)\\
  $\boldsymbol{M_{\text{Rout}}}$ &=& (& $X\times Y$; &$W$;& $<_{X}$; &$M_{\text{Rin}}$; & $(k,v)\mapsto M_{\text{Rin}}$.Single$(k,v)$; & $\cup$;& $\emptyset$ &)\\
  \hline
\end{tabular}
}}}

\mapstructure{
{\small
\begin{tabular}{|r@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }lllllll@{ }l|}
  \hline
  $\boldsymbol{M_{\text{Rin}}}$ &=& \textbf{AM} &(& $\boldsymbol{K}$: $X\times Y$;& $\boldsymbol{V}$: $W$; &$\boldsymbol{\prec}$: $<_{Y}$;&  $\boldsymbol{A}$: $W$;& $\boldsymbol{g(k,v)}$: $v$; &$\boldsymbol{f}$: $+_W$; &$\boldsymbol{a_{\emptyset}}=0$ &)\\
  $\boldsymbol{M_{\text{Rout}}}$ &=& \textbf{AM} &(& $\boldsymbol{K}$: $X\times Y$;& $\boldsymbol{V}$: $W$; &$\boldsymbol{\prec}$: $<_{X}$; & $\boldsymbol{A}$: $M_{\text{Rin}}$; & $\boldsymbol{g(k,v)}$: $M_{\text{Rin}}$.Single$(k,v)$; &$\boldsymbol{f}$: $\cup$;& $\boldsymbol{a_{\emptyset}}$: $\emptyset$ &)\\
  \hline
\end{tabular}
}}

\hide{
\para{Dynamically update.}
In this paper we also show how to dynamically update (insert or delete) the range tree with reasonably low cost.
}

\subsection{Sweepline Algorithm using \rangesweep}
\label{sec:rangesweep}
In this section we present a sweepline algorithm to address the 2D range query problem using the PrefixSweep paradigm introduced above. It can answer queries such as count or weight sum efficiently.

We set the processing order to be the order of the x-coordinate. %We note the sorted sequence of points as $\{p_i\}$ and the x- and y-coordinate as $x_i$ and $y_i$ respectively.
Each \sweepstructure{} is a set tracking all points up to the current point. Thus the update operation
is just an insertion. The \sweepstructure{}s are augmented maps, with the same form as the inner tree structure ($M_{\text{Rin}}$) in range trees. Entries are sorted by the y-coordinate, values are set to be weights, and the augmented value accumulates weights over y-ranges. The abstraction of this sweepline structure, with the \sweepstructure{}s as augmented maps, is defined as:
\mapstructure{
{\small
\begin{tabular}{|r@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }l@{ }l|}
  \hline
  $\boldsymbol{S_{\text{Rin}}}$ &=& \textbf{AM} &(& $\boldsymbol{K}$: $X\times Y$;\quad $\boldsymbol{V}$: $W$; \quad$\boldsymbol{\prec}$: $<_{Y}$; \quad$\boldsymbol{A}$: $W$; \quad$\boldsymbol{g(k,v)}$: $v$; \quad$\boldsymbol{f}$: $+_W$; \quad$\boldsymbol{A_{\emptyset}}$: $0$ &)\\
  $\boldsymbol{S_{\text{Rout}}}$ &=& \textbf{PS} &(& $\boldsymbol{P}$: $X\times Y$; \quad$\boldsymbol{\prec}$: $<_X$; \quad $\boldsymbol{T}$: $\boldsymbol{S_{\text{Rin}}}$; \quad$\boldsymbol{h(p,t)}$: insert$(t,p)$ &)\\
  \hline
\end{tabular}
}}

\para{Tree Construction.} The combine function $h$ (insert) in the RangeSweep scheme can be easily batched using \texttt{union} function $\funcb:S_{\text{Rin}}\times S_{\text{Rin}}\mapsto S_{\text{Rin}}$. Accordingly the fold function $\funca$ would be to build an augmented map $S_{\text{Rin}}$ from a sequence of points, and same as $T$, the type $T'$ is an augmented map $S_{\text{Rin}}$. Thus to parallelize the sequential $S_{\text{Rout}}$ scheme we can use the parallel sweepline paradigm:
\mapstructure{
{\small
\begin{tabular}{|r@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }l@{ }l|}
  \hline
  \textbf{RangeSweep} &=& \textbf{PP} &(& \textbf{PS}: $S_{\text{Rout}}$;\quad $\boldsymbol{T'}$: $S_{\text{Rin}}$; \quad$\boldsymbol{\rho(\{p_i\})}$: $S_{\text{Rin}}$.build$(\{p_i\})$; \quad $\boldsymbol{\phi}$: $\cup$; \quad&)\\
  \hline
\end{tabular}
}}


For this specific problem the parallel algorithm and its corresponding cost is:
\begin{enumerate}\setlength\itemsep{-.4em}
\item \textbf{Batching}. Build $k$ trees $T'_{i}$ ($0\le i \le k$) corresponding to the blocks in parallel. Considering that there are $k$ trees of size $n/k$, this step takes work $O(k\cdot \frac{n}{k}\log \frac{n}{k})=O(n\log \frac{n}{k})$ and depth $O(\log \frac{n}{k})$.

\item \textbf{Getting prefix}. Compute $T_{jt}=$\texttt{union}$(T_{(j-1)t}, T'_{j})$. Consider the work of union is $O\left(m\log (\frac{n}{m}+1)\right)$, the total cost of this step is bounded by: $O\left(\sum_{i=1}^{k} t\log (\frac{it}{t} +1)\right)=O\left(t\sum_{i=1}^{k} \log (i+1)\right)=O(n\log k)$. The depth is:\vspace{-1em}
\begin{equation}
O\left(\sum_{i=1}^{k}\log t \log it\right)=O\left(\log t\cdot \left(k\log t+\sum_{i=1}^{k}\log i\right)\right)=O(k\log \frac{n}{k}\log n)\vspace{-1em}
\end{equation}
%$O(k\log \frac{n}{k}\log n)$.

\item \textbf{Refining}. For each block, build all the other trees based on $T_{jt}$ by inserting points into it in turn. All the $k$ blocks can be done in parallel. The total work is bounded by: $c\sum_{i=1}^{n} \log i=O(n\log n)$.
The depth is the cost to finish all work in one block, which is $O(\frac{n}{k}\log n)$.\vspace{-1em}
\end{enumerate}

In total, this process costs work $O(n\log n)$ and depth $O(\left(k\log \frac{n}{k}+\frac{n}{k}\right)\log n)$. When $k=\Theta(\sqrt{n/\log n})$, the depth is $O(\sqrt{n}\log^{1.5}n)$. By repeatedly applying this process we can reduce the depth to $O(n^{\epsilon})$ where $0<\epsilon<1$ can be arbitrarily small (See details in Appendix \ref{app:rangesweep}. In practice, we set $k=O(p)$ where $p$ is the number of threads. Note that this data structure is not highly theoretically efficient in construction depth (e.g., building a range tree would only cost $O(\log^3 n)$ depth), but in Section \ref{sec:exp} we will show that it has good practical performance.% and is especially efficient in query.

Also, notice that naively such a data structure would cost $O(n^2)$ space as the \sweepstructure{} sizes are $1$ through $n$. However functions in the PAM library will keep data persistent, and will create at most one new tree node in one single operation. Thus the extra space it requires is asymptotically no more than its time complexity, which is $O(n\log n)$. 

\para{Answering Queries.}
With the RangeSweep, we can answer a weight-sum query in $O(\log n)$ time. We first binary search $x_L$ and $x_R$ in the sorted sequence of $\{x_i\}$, finding $l$ and $r$ satisfying $x_l<x_L\le x_{l+1}$ and $x_r\le x_R< x_{r+1}$. Now that we can narrow the range of x-coordinate into $(x_L,x_R)$ by looking at only the points in $T_r-T_l$. We then get the weight sum of all points within range $(y_L,y_R)$ in $T_{x_l}$ and $T_{x_r}$ using two range queries, and the difference of them is the answer. 
Two independent binary searches cost $O(\log n)$ respectively, and the range search on y-coordinate costs work $O(\log n)$. Thus total cost of a single query is $O(\log n)$.

\para{Extension to Report All Points.} The RangeSweep can answer weight sum efficiently, but reporting all points would be inefficient as to explicitly computing $T_r-T_l$ is costly\footnote{Especially when $|T_l|$ is large but $|T_r-T_l|$ is small.}. Here we propose another sweepline algorithm for that. It is similar to the RangeSweep, yet with a different augmentation. Instead of weight, we store the x-coordinates as values, and set the augmented value to be the maximum x-coordinate among all points in the subtree. To answer queries we first narrow the range to the points in tree $T_r$ by just searching $x_r$. Then all queried points are those in $T_r$ with x-coordinates larger than $x_l$ and y-coordinate in $[y_l,y_r]$. We still conduct a range query in $[y_l, y_r]$ on $T_r$, but adapt an optimization that if the augmented value of a tree node is less than $x_l$, the whole subtree is discarded.
Otherwise, at least part of the points in the tree would be relevant and we recursively deal with its two subtrees.
The work of one query is $O(k\log (\frac{n}{k}+1))$, where $k$ is the output size. Pseudocode and detailed analysis are given in Appendix \ref{app:rangesweeplist}.

\hide{As mentioned above, the final answer is the difference of two such sets (subsets of $T_{x_l}$ and $T_{x_r}$). Since the complexity of the difference function depends on the size of both sets ($O(n\log (m/n+1))$), it is possible that the subset of $T_{x_l}$ is larger than the output size and the cost would be far higher than optimal. For example, when $x_l=O(n)$ and $x_r=x_l+c$ where $c$ is a constant, and the query range of y-coordinate is $(-\infty, +\infty)$. In this case reporting all points by taking the difference of $T_{x_l}$ and $T_{x_r}$ requires $O(n)$ time, but using a range tree would only take $O(\log^2 n)$ time (considering the output size is no more than $c$).}

\hide{In all, the augmented structure is defined as:
{\ttfamily\small
\begin{lstlisting}[language=C++,frame=lines,escapechar=@]
struct aug_max {
  using aug_t = int;
  static aug_t base(int y, int x){ return x;}
  static aug_t combine(int a, int b){ return max(a, b);}
  static aug_t get_empty() {return 0;}
};
\end{lstlisting}
}
}

%The construction of the tree is the same as the weighted version, while the query process is slightly different.





==> augmap.tex <==
\section{Augmented Maps}
\label{sec:augmap}
For a universe of keys $K$ and values $V$, a \emph{map} is a relation
$R \subset K \times V$ (set of key-value pairs), such that a key can
only appear in one element.  An \emph{ordered map} is a map for which
the keys $K$ have a total order defined by $<_K$ (we drop the
subscript).  We denote each entry (the key-value pair) in a map as
$(k,v)$ or $e$, and the functions to extract the key and value from $e$
as $k(e)$ and $v(e)$.  Many functions can be defined on ordered
maps. Table \ref{tab:mapfunctions} lists some common map functions
along with their mathematical definitions.

\begin{table} [!h!t]
\begin{center}
	\begin{tabular}{>{\bf}l<{}|cc}
	\hline
	\textit{\textbf{Function}} &\textbf{Description}  \\
	\hline
\hline
\texttt{domain}$(M)$ & $\{k(e)\,:\,e\in M\}$\\
\hline
\texttt{size}$(M)$ & $|M|$\\
\hline
\texttt{find}$(M,k)$ & $v$ \textbf{if}  $ (k,v) \in M$ \textbf{else} $\Box$\\
\hline
\texttt{delete}$(M,k)$ & $\{ (k',v) \in M~|~k' \neq k \}$\\
\hline
\texttt{insert}$(M,e)$& \texttt{delete}$(M,k(e)) \cup \{e\}$\\
\hline
\texttt{first}$(M)$&  $\arg\min_{e\in M} k(e)$ \textbf{if} $M\ne \emptyset$ \textbf{else} $\Box$\\
\hline
\texttt{last}$(M)$&  $\arg\max_{e\in M} k(e)$ \textbf{if} $M\ne \emptyset$ \textbf{else} $\Box$\\
\hline
\texttt{next}$(M,k)$ &  \texttt{first}$(\{(k',v) \in M~|~k' > k\})$\\
\hline
\texttt{prev}$(M,k)$ &  \texttt{last}$(\{(k',v) \in M~|~k' < k\})$\\
\hline
\texttt{rank}$(M,k)$ & $|\{(k',v)\in M~|~k' < k\}|$\\
\hline
\multirow{2}{*}{\texttt{split}$(M,k)$} & $\langle \{e\in M\,|\,k(e)<k\}, \mathbbm{1}(k\in M),$\\
&$ \{e\in M\,|\,k(e)<k\} \rangle$\\
\hline
\multirow{2}{*}{\texttt{select}$(M,i)$}&\multicolumn{1}{l}{Argument $i\in \mathbb{Z_{+}}$ }\\
\cline{2-2}
 & $e : e \in M\,|\, i= |\{e' \in M~|~k(e') < k(e)\}| $\\
\hline
\multirow{2}{*}{\texttt{forall}$(M,\sigma)$} &
                                             \multicolumn{1}{l}{Argument $\sigma :(K\times V)\rightarrow V'$}\\
\cline{2-2}
& $\{(k,\sigma(k,v)) : (k,v) \in M\}$ \\
\hline
\multirow{2}{*}{\texttt{filter}$(M,\phi)$} &
                                             \multicolumn{1}{l}{Argument $\phi:(K\times V)\rightarrow \{\textbf{false},\textbf{true}\}$}\\
\cline{2-2}
& $\{e \in M~|~\phi(e)\}$ \\
\hline
\texttt{range}$(M,k_1,k_2)$ & $\{e \in M\,|\,k_1<k(e)<k_2\}$ \\
\hline
\texttt{intersect}& \multirow{2}{*}{$\{e \in M_1~|~ k(e) \in
                                \texttt{domain}(M_2)\}$}\\
\hspace*{.4in}$(M_1,M_2)$ & \\

\hline
\texttt{diff}$(M_1,M_2)$ & $\{e \in M_1~|~ k(e) \not\in \texttt{domain}(M_2)\}$\\
\hline
\texttt{union}$(M_1,M_2)$&$M_1 \cup \texttt{diff}(M_2,M_1)$ \\
\hline
%\texttt{filter}$(s,\phi)$&$\langle s'_i=s_{m_i}\,:\, \phi(s_{m_i}), \forall x<y, m_x<m_y\rangle$ \\
%\hline
\multirow{3}{*}{\texttt{build}$(s)$} & \multicolumn{1}{l}{Argument $s=\langle e_1,\dots, e_n \rangle, e_i\in K\times V,$}\\
%& \multicolumn{1}{c}{$\forall i,j, k(e_i)\ne k(e_j)$}\\
\cline{2-2}
%& $\{ e \,|\, e\in s\}$\\
& $\{ (k',v(s'_0))\,|\, \exists e\in s, k(e)=k', $\\
%&$s'=\texttt{filter}(s,\mathbbm{1}(k(\cdot)==k'))^{*} \}$\\
& $s'=\langle e\,:\, e\in s \,|\, k(e)=k' \rangle $\\
\hline
\texttt{seq}$(M)$ & sequence $\langle(k,v) \in M\rangle$ ordered by $k$\\
\hline
\multirow{2}{*}{\texttt{reduce}$(M, \sigma)$} &
                                             \multicolumn{1}{l}{Argument $\sigma:(V\times V)\rightarrow V$}\\
\cline{2-2}
& $\Sigma_{\sigma}\langle v(e) : e \in \texttt{seq}(M) \rangle$\\
\hline
	\end{tabular}
	\end{center}
    \vspace{-0.2in}
\caption{The core functions on ordered maps. Throughout the table we assume $k,k_1,k_2\in K$, $v,v_1,v_2\in V$ and $e\in K\times V$, $M, M_1, M_2$ are ordered maps. $|\cdot|$ denotes the cardinality of a set. $\Box$ represents a empty element. $\mathbbm{1}(\cdot)$ is the indicator function. Some notations are defined in Equation (\ref{equ:f1}), (\ref{equ:f2}), (\ref{equ:fseq}) and (\ref{equ:gseq}).}
    \label{tab:mapfunctions}
    \vspace{-0.1in}
\end{table}

In this paper we augment maps by associating them with an augmented
value.
% using augmented balanced binary search trees. We first introduce the concept of augmented value on a map.
For a map $M$ with keys $\in K$ and values $\in V$, we define its
\emph{augmented value} $\in \augtype$ along with two functions $f$ and $g$.
The \emph{augmented base function} $g:K\times V \rightarrow \augtype$
converts a key-value pair to an augmented value, and the
\emph{augmented combine function}
$f:\augtype \times \augtype \rightarrow \augtype$ combines two
augmented values.    We assume $f$ is associative, and
define:
\begin{align}
\label{equ:f1}
f(v_1) &\equiv v_1\\
\label{equ:f2}
f(v_1, v_2, \dots, v_n) &\equiv f(v_1, f(v_2, v_3, \dots, v_n))
\end{align}
We define $\Sigma_f (s)$ as applying the function $f$ to a sequence of elements $s=\langle s_1, s_2, \dots, s_n\rangle$, i.e.,
\begin{align}
\label{equ:fseq}
\Sigma_f(s) = f(s_1, s_2, \dots, s_n)
\end{align}
and $\langle g(e)\,:\, e\in s \rangle$ as applying the function $g$ in turn on a sequence of elements $s=\langle s_1, s_2, \dots, s_n\rangle$ to get another sequence, and keep the order in the original sequence, i.e.,
\begin{align}
\label{equ:gseq}
\langle g(e)\,:\, e\in s \rangle = \langle g(s_1),g(s_2),\dots,g(s_n) \rangle
\end{align}
For a map $M$ let $\texttt{seq}(M)$ be the sequence of entries in $M$
ordered by the key. Then the formal definition of an augmented value is given as follows:

\begin{definition}[Augmented Value]
\label{def:augvalue}
Given a map $M$ over keys $K$ and values $V$, and functions $g$ and
$f$ as defined above, its \emph{augmented value} is
\begin{align}
\label{equ:augvalue}
%\augvalue{f}{g}{M} = \Sigma_f \langle g(k,v) : (k,v) \in \texttt{ord}(M)\rangle
\augvalue{f}{g}{M} = \Sigma_f \langle g(k(e),v(e))\,:\, e\in \texttt{seq}(M)\rangle
\end{align}
\end{definition}
The ordering is important since the function $f$ might not be
commutative.  With clear context we omit the subscript.

Table \ref{tab:augfunctions} lists some functions that are useful for
augmented maps.  In addition we augment some of the standard functions
(\ctext{insert}, \ctext{intersect}, \ctext{union}, and \ctext{build})
so they combine values.  For example, \texttt{union} and
\texttt{intersect} accept a third argument $\sigma$, which is itself a
function.  If any keys appear in both maps, the function is applied
to the corresponding pair of values to generate a new value to
associate with that key. Similarly for \texttt{insert} if the key
already exists in the map, the $\sigma$ function is applied on the
value in the map and the new value to be inserted as the new value.
Also, the \texttt{build} function takes a reduce function $\sigma$ as
input. When the input sequence contains duplicates among its keys, all the
values of the same key $k$ will be reduced to a single value by this
reduce function $\sigma$, and will appear in the output map as the
value of key $k$.  This can be used, for example, to keep a count for
each key, and have union and intersection sum the counts, insert add
the counts, and build keep the total counts in the sequence.


\begin{table}[!h!t]
\begin{center}
	\begin{tabular}{>{\bf}l<{}|c}
	\hline
	\textit{\textbf{Function}} &\textbf{Description}  \\
	\hline\hline
\multicolumn{2}{l}{\textbf{Functions on Augmented Maps}}\\
\hline
\texttt{aug\_val}$(M)$  &$\augvalueone{M}$ \\
\hline
\texttt{aug\_left}$(M,k)$  &$\augvalueone{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')<k\}$ \\
\hline
\texttt{aug\_right}$(M,k)$  &$\augvalueone{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')>k\}$ \\
\hline
\texttt{aug\_range} &$\augvalueone{M'} \,:\, M'=\{e'\,|\,e'\in M,$ \\
\multicolumn{1}{r|}{$(M,k_1,k_2)$}&$  k_1<k(e')<k_2\}$\\
\hline
\texttt{aug\_find}$(M,a)$  &$\texttt{last}(\{e\in M \,|\, \texttt{aug\_l}(M,k(e))\le a\})$ \\
\hline
\multicolumn{2}{l}{\textbf{Augmented Functions}}\\
\hline
\multirow{2}{*}{\texttt{insert}}&\multicolumn{1}{l}{Argument $\sigma:V\times V\rightarrow V$}\\
\multirow{2}{*}{$(M,e,\sigma)$}& \texttt{delete}$(M,k(e)) \cup $\\
&$\{ (k(e), \sigma(v(e),\texttt{find}(M,k(e)))) \}$\\
\hline
\multirow{2}{*}{\texttt{intersect}}& \multicolumn{1}{l}{Argument $\sigma:V\times V\rightarrow V$}\\
\cline{2-2}
\multirow{2}{*}{$(M_1, M_2, \sigma)$}&
%$\{( k,\sigma(v_1,v_2))\,|\,\langle k,v_1\rangle\in M_1,\langle k,v_2\rangle\in M_2\}$\\
$\{ (k, \sigma(\texttt{find}(M_1,k),\texttt{find}(M_2,k)))$\\
&\multicolumn{1}{r}{$|\,k \in \texttt{domain}(M_1)\cap \texttt{domain}(M_2)\}$}\\
\hline
\multirow{2}{*}{\texttt{union}}& \multicolumn{1}{l}{Argument $\sigma:V\times V\rightarrow V$} \\
\cline{2-2}
\multirow{2}{*}{$(M_1, M_2, \sigma)$}&\texttt{diff}$(M_1,M_2)~\cup$ \texttt{diff}$(M_2,M_1)$\\
&$\cup$ \texttt{intersect}$(M_1,M_2,\sigma)$\\
\hline
\multirow{4}{*}{\texttt{build}$(s, \sigma)$} & \multicolumn{1}{l}{Argument $\sigma:V\times V\rightarrow V$}\\
& \multicolumn{1}{l}{Argument $s=\langle e_1, e_2,\dots, e_n \rangle$ }\\
\cline{2-2}
& $\{ \langle k',\Sigma_{\sigma}(s')\rangle \,|\, \exists e\in s, k(e)=k',$\\
&$s'=\langle e\,:\, e\in s \,|\, k(e)=k' \rangle $\\
\hline
	\end{tabular}
	\end{center}
\caption{The core functions on augmented ordered maps. Throughout the table we assume $k,k_1,k_2\in K$, and $e'\in K\times V$, $M$ is an augmented ordered maps. Some notations are defined in Equation (\ref{equ:f1}), (\ref{equ:f2}), (\ref{equ:fseq}), (\ref{equ:gseq}) and (\ref{equ:augvalue}).}
    \label{tab:augfunctions}
\end{table}

\para{Implementing Augmented Maps with Augmented Trees.}
An augmented tree structure is a search tree (possibly but not
necessarily binary) in which each node is augmented with a value
recording some information about its subtree.  Although this concept
is widely-used in textbooks \cite{CormenLeRi90}, we have not found a
formal definition.  In this paper, we use augmented trees to implement
augmented maps, and give a definition specific to implementing maps.

\begin{definition}[Augmented Tree]
  An augmented tree $T$ for a map $M$ is a search-tree associated
  with two functions $f$ and $g$, for which each node $v$ is augmented
  with an value $\augvalue{f}{g}{M_v}$ (see in
  Definition \ref{def:augvalue}), where $M_v\subseteq M$ is the
  range of $M$ belonging to the subtree rooted at $v$.
\end{definition}

In this paper, with clear context, we also use a tree node $v$ to
denote the whole subtree $T_v$ rooted at it, the entry stored in it,
as well as the map that its subtree $T_v$ represents.  The notation we
use in this paper is summarized in Table~\ref{fig:notation}.

\hide{
In this paper, we augment \emph{balanced binary search trees}, which refer to binary search trees obeying specific balancing schemes, to implement maps.
A \emph{binary tree} is either a \leaf{}, or a node consisting of a
\emph{left} binary tree $\Tl$, a value (or key) $v$, and a
\emph{right} binary tree $\Tr$. A \emph{binary search tree} is a binary tree whose in-order traversing is the sorted order of all
of its keys.
A \emph{balancing scheme} for binary trees is an invariant (or set of
invariants) that is true for every node of a tree, and is for the
purpose of keeping the tree nearly balanced.  In this paper we
consider four balancing schemes that ensure the height of every tree
of size $n$ is bounded by $O(\log n)$: AVL trees~\cite{avl},
Red-black (RB) trees~\cite{redblack}, Weight-balanced (WB) trees
and Treaps~\cite{SA96}.
}


\begin{table}
  \centering
  \begin{tabular}{c|c}
    \hline
    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    \textbf{Notation} & \textbf{Description} \\
    \hline
    $k(\cdot)$ & The key of a tree node\\
    $v(\cdot)$ & The value of a tree node\\
    %\hline
    $L(\cdot)$ & The left child of a tree node \\
    %\hline
    $R(\cdot)$ & The right child of a tree node  \\
    $\augvalueone{\cdot}$ & The augmented value of a map\\
  %  $K$& The domain of key or the type of key in programming\\
  %  $V$& The domain of value or the type of value in programming\\
  %  $AV$& The domain of augmented value or the type of augmented value in programming\\
    %\texttt{expose}$(T)$ & A function to get triple $(L(T),k(T),R(T))$ \\
    %\hline
    %$k.{\rm{data}}$ & The data stored in node $k$ \\
    %$k_1<k_2$ & $k_1.{\rm{data}}<k_2.{\rm{data}}$ \\
    %$T_1<T_2$ & $\forall k_1 \in T_1, k_2\in T_2$, $k_1<k_2$ \\
    %$T_1<k$ & $\forall k_1 \in T_1$, $k_1<k$ \\
    \hline
  \end{tabular}
  \caption{Summary of notation.}\label{fig:notation}
\end{table}


\begin{comment}
 However, and obviously, it is
unsafe to call \texttt{clear} or \texttt{final} on a map that is still
being operated on concurrently by any other function.  All results are
fully deterministic independent of interleaving of concurrent tasks
since the functions create new values instead of mutating old ones
(unless final, in which case other copies should no longer be
accessed).
\end{comment}

\begin{comment}
The difference between a tree map and an augmented map is that the latter accepts a binary operator as its thrid argument.
Each node of an augmented map stores the application of the binary operator on the values of the tree rooted at itself.
For this reason augmented maps support an \texttt{accumulate} function. It accepts a key $k'$, and returns the application
of the binary operator on all nodes with a key $k \leq k'$. Table \ref{tab:interface} lists the core functions which are supported by all of our containers.

Most of the functions mentioned in Table \ref{tab:interface} are self-explanatory, and we won't go in much detail into them.
In Table \ref{tab:interface} we didn't list any of the methods which are responsible for allocating and freeing nodes.
The memory allocator is not bound to individual object instances, as it is usually implemented. The reason for this
is that due to persistence two or more objects can share a subset of nodes with each other. The memory allocator we provide
operates on the level of class instances and is accessed through three methods: \texttt{init} is used to initialize the memory allocator of a particular map or set class,
\texttt{reserve} accepts a number $n$ and allocates memory for $n$ nodes, and \texttt{finish} destroys the memory allocator and frees all the memory occupied by it. \\

The method responsible for freeing nodes of individual objects is \texttt{clear}, which effectively empties the content of the container.
\texttt{clear} invokes the garbage collection and recollects all nodes which don't belong to a tree anymore.
\end{comment}




\hide{
\multicolumn{3}{l}{\textbf{Augmented operations of map $M$}}\\
\hline
\texttt{aug\_left}$(k)$  & $k\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')<k\}$ \\
\hline
\texttt{aug\_right}$(k)$  & $k\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')>k\}$ \\
\hline
\texttt{aug\_range}$(k_1,k_2)$  & $k_1,k_2\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k_1<k(e')<k_2\}$ \\
\hline
\hline
\multirow{2}{*}{\texttt{join}$(M_1,k',M_2)$} & $M_1,M_2\subseteq U, k'\in K$ & \multirow{2}{*}{$M_1\cup\{k'\}\cup M_2$} \\
& $\max_{e\in M_1}k(e)<k'<\min_{e\in M_2}k(e)$ &\\
\hline
\multirow{2}{*}{\texttt{joinTwo}$(M_1,M_2)$} & $M_1,M_2\subseteq U$ & \multirow{2}{*}{$M_1\cup M_2$} \\
& $\max_{e\in M_1}k(e)<\min_{e\in M_2}k(e)$ &\\
\texttt{split}$(k')$ &$k'\in K$ & $\langle \, \{e\,|\,e\in M, k(e)<k'\}, \mathbbm{1}\left[k'\in M\right], \{e\,|\,e\in M, k(e)>k'\} \,\rangle$\\
\hline
----
\multicolumn{3}{l}{\textbf{Aggregate operations}}\\
\hline
\multirow{3}{*}{\texttt{union}$(M_1, M_2, \sigma)$}& \multirow{2}{*}{$M_1,M_2\subseteq U$} & $\{\langle k,v\rangle\,|\,\langle k,v\rangle\in M_1,\forall v', \langle k',v\rangle\notin M_2\}\cup$\\
&\multirow{2}{*}{$\sigma:V\times V \rightarrow V$}&$\{\langle k,v\rangle\,|\,\langle k,v\rangle\in M_2,\forall v', \langle k',v\rangle\notin M_1\}\cup$\\
&&$\{\langle k,\sigma(v_1, v_2)\rangle\,|\,\langle k,v_1\rangle\in M_1,\langle k,v_2\rangle\in M_2\}$\\
\hline
\multirow{2}{*}{\texttt{intersection}$(M_1, M_2, \sigma)$}& \multirow{1}{*}{$M_1,M_2\subseteq U$} & \multirow{2}{*}{$\{\langle k,\sigma(v_1,v_2)\rangle\,|\,\langle k,v_1\rangle\in M_1,\langle k,v_2\rangle\in M_2\}$}\\
&\multirow{1}{*}{$\sigma:V\times V \rightarrow V$}&\\
\hline
\texttt{difference}$(M_1,M_2)$ & $M_1,M_2\subseteq U$& $M_1-M_2$\\
\hline
\multicolumn{3}{l}{\textbf{Map constructions}}\\
\hline
\texttt{singleton}$(e)$  & $e\in K\times V$ &$\{e\}$ \\
\hline
\multirow{2}{*}{\texttt{build}$(s, \sigma)$} & $s=\langle e_1, e_2,\dots, e_n \rangle$ & $\{ \langle k(e),\Sigma_{\sigma}(s')\rangle \,|\, e\in s, s'=\langle v(e_{i_1}), v(e_{i_2}), \dots v(e_{i_m})\,:\, $ \\
&$\sigma:V\times V\rightarrow V$& $\forall j, 1\le j\le m, e_{i_j}\in s,k(e_{i_j})=k(e), i_1<i_2\dots<i_m\rangle\}$\\
\hline
}

\hide{
\begin{table*}[!h!t]
\begin{center}
	\begin{tabular}{l|c|c}
	\hline
	\textit{\textbf{Function}} &\textbf{Parameters} &\textbf{Description}  \\
	\hline
\multicolumn{3}{l}{\textbf{Map operations of $M$}}\\
\hline
\texttt{content}$()$ & & M\\
\hline
\texttt{insert}$(e)$& $e\in K \times V$ & $M\cup \{e\}$\\
\hline
\texttt{delete}$(e)$& $e\in K \times V$ & $M - \{e\}$\\
\hline
\texttt{find}$(k)$& $k\in K$ & $v:\langle k,v\rangle\in M$\\
\hline
\texttt{next}$(k)$& $k\in K$ & $e:e\in M, k(e)=\min_{e\in M} k(e)>k$\\
\hline
\texttt{previous}$(k)$& $k\in K$ & $e:e\in M, k(e)=\max_{e\in M} k(e)<k$\\
\hline
\texttt{first}$()$&  & $e:e\in M, k(e)=\min_{e\in M} k(e)$\\
\hline
\texttt{last}$()$&  & $e:e\in M, k(e)=\max_{e\in M} k(e)$\\
\hline
\texttt{item\_rank}$(k)$& $k\in K$ & $|\{e|e\in M, k(e)<k\}|$\\
\hline
\texttt{select}$(i)$ & $i\in \mathbb{Z_{+}}$ & $e:\left|\{e'|e'\in M, k(e')<k(e)\}\right|=i-1$\\
\hline
\texttt{forall}$()$ & ?? & ??\\
\hline
\texttt{filter}$(\phi)$ & $\phi:K\rightarrow \{0,1\}$ & $\{e\,|\,\phi(k(e))\}$ \\
\hline
\texttt{range}$(k_1,k_2)$ & $k_1,k_2\in K$ & $\{e\,|\,k_1<k(e)<k_2\}$ \\
\hline
\texttt{split}$(k')$ &$k'\in K$ & $\langle \, \{e\,|\,e\in M, k(e)<k'\}, \mathbbm{1}\left[k'\in M\right], \{e\,|\,e\in M, k(e)>k'\} \,\rangle$\\
\hline
\multicolumn{3}{l}{\textbf{Augmented operations of map $M$}}\\
\hline
\texttt{aug\_left}$(k)$  & $k\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')<k\}$ \\
\hline
\texttt{aug\_right}$(k)$  & $k\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')>k\}$ \\
\hline
\texttt{aug\_range}$(k_1,k_2)$  & $k_1,k_2\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k_1<k(e')<k_2\}$ \\
\hline
\multicolumn{3}{l}{\textbf{Aggregate operations}}\\
\hline
\multirow{2}{*}{\texttt{join}$(M_1,k',M_2)$} & $M_1,M_2\subseteq U, k'\in K$ & \multirow{2}{*}{$M_1\cup\{k'\}\cup M_2$} \\
& $\max_{e\in M_1}k(e)<k'<\min_{e\in M_2}k(e)$ &\\
\hline
\multirow{2}{*}{\texttt{joinTwo}$(M_1,M_2)$} & $M_1,M_2\subseteq U$ & \multirow{2}{*}{$M_1\cup M_2$} \\
& $\max_{e\in M_1}k(e)<\min_{e\in M_2}k(e)$ &\\
\hline
\multirow{3}{*}{\texttt{union}$(M_1, M_2, \sigma)$}& \multirow{2}{*}{$M_1,M_2\subseteq U$} & $\{\langle k,v\rangle\,|\,\langle k,v\rangle\in M_1,\forall v', \langle k',v\rangle\notin M_2\}\cup$\\
&\multirow{2}{*}{$\sigma:V\times V \rightarrow V$}&$\{\langle k,v\rangle\,|\,\langle k,v\rangle\in M_2,\forall v', \langle k',v\rangle\notin M_1\}\cup$\\
&&$\{\langle k,\sigma(v_1, v_2)\rangle\,|\,\langle k,v_1\rangle\in M_1,\langle k,v_2\rangle\in M_2\}$\\
\hline
\multirow{2}{*}{\texttt{intersection}$(M_1, M_2, \sigma)$}& \multirow{1}{*}{$M_1,M_2\subseteq U$} & \multirow{2}{*}{$\{\langle k,\sigma(v_1,v_2)\rangle\,|\,\langle k,v_1\rangle\in M_1,\langle k,v_2\rangle\in M_2\}$}\\
&\multirow{1}{*}{$\sigma:V\times V \rightarrow V$}&\\
\hline
\texttt{difference}$(M_1,M_2)$ & $M_1,M_2\subseteq U$& $M_1-M_2$\\
\hline
\multicolumn{3}{l}{\textbf{Map constructions}}\\
\hline
\texttt{singleton}$(e)$  & $e\in K\times V$ &$\{e\}$ \\
\hline
\multirow{2}{*}{\texttt{build}$(s, \sigma)$} & $s=\langle e_1, e_2,\dots, e_n \rangle$ & $\{ \langle k(e),\Sigma_{\sigma}(s')\rangle \,|\, e\in s, s'=\langle v(e_{i_1}), v(e_{i_2}), \dots v(e_{i_m})\,:\, $ \\
&$\sigma:V\times V\rightarrow V$& $\forall j, 1\le j\le m, e_{i_j}\in s,k(e_{i_j})=k(e), i_1<i_2\dots<i_m\rangle\}$\\
\hline

%\multicolumn{3}{l}{Memory management}\\
%\hline
%\texttt{reserve}, \texttt{init} & n & $1$ \\
%\hline
%\texttt{clear}, \texttt{finish} & $1$ &$1$ \\
%\hline
	\end{tabular}
	\end{center}
	%\nocaptionrule
\caption{The core functions.}
    \label{tab:functions}
\end{table*}
}


==> exp-old.tex <==
\section{Experiments}
\label{sec:exp}
To evaluate the performance of our library we performed several
experiments across the four balancing schemes, a variety of functions,
varying core counts, two different machine types, and varying sizes.
We compare the performance our library on a single core to the C++
Standard Template Library (STL) implementation of ordered maps, which is
based on red-black trees, and their generic implementation of
\union{}.

\paragraph{Set up}
For the experiments we use a 64-core machine with 4 x AMD Opteron(tm)
Processor 6278 (16 cores, 2.4GHz, 1600MHz bus and 16MB L3 cache), and
a 40-core (with two-way hyperthreading) machine with 4 x Intel E7-8870
Xeon processors (10 cores, 2.4GHz, 1066MHz bus and 30MB L3 cache).
For the Intel machine we had hyper-threading enabled during the
experiments, yielding a total of 80 hyper-threads.  The library was
compiled using the \texttt{g++} 4.8 compiler with the Cilk Plus
extensions, and using \texttt{-O2} flag.  For testing purposes we
choose our map implementation, but we note that the set implementation
would lead to similar results.  For all timings reported we use an
integer key and an integer value.  Each node is about 48 bytes,
including the two child pointers, the key and value, the balance
information, the size of the subtree, and a reference count.  We
generate multiple maps varying in size from $10^4$ to $10^8$.  Each
map contains randomly chosen keys and values.   Throughout $n$ and $m$ represent
the two input sizes for functions with two input maps.

\newcommand{\figscale}{0.5}
\begin{figure*}[t!]
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/graphs/tree_comp} \\ (a)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering \includegraphics[scale=\figscale]{figures/graphs/union_speedup} \\ (b)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering \includegraphics[scale=\figscale]{figures/graphs/union_speedup2} \\ (c)
\end{minipage}
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/graphs/other} \\ (d)
\end{minipage}

\vspace{.1in}
\begin{minipage}{.24\textwidth}
  \centering \includegraphics[scale=\figscale]{figures/graphs/build} \\ (e)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering\includegraphics[scale=\figscale]{figures/graphs/union_vs_deunion}\\(f)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering\includegraphics[scale=\figscale]{figures/graphs/insertion}\\(g)
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering   \includegraphics[scale=\figscale]{figures/graphs/union_sequential}\\(h)
\end{minipage}
%\nocaptionrule
\caption{
(a) Times for \union{} as a function of size ($n = m$) for different
BBSTs;
(b, c) speed up of \union{} for different BBSTs on both of our machines;
(d) times for various operations on AVL trees as a function of size ($m  = 10^8$);
(e) times for different versions of \build{} as a function of size. \union{}-\build{} I is taking a presorted sequence, while
\union{}-\build{} II is taking a permuted one;
(f) Persistent vs. destructive \union{};
and
(g) insertion comparison with the STL;
(h) comparing STLs \texttt{set\_union} with our \union{}
implementation.
}
\label{fig:times}
\end{figure*}

\paragraph{Comparing the balancing schemes}
To compare the four balancing schemes we choose \union{} as the
representative operation.  Other operations would lead to similar
results since all operations except \join{} are generic across the
trees.  We compare the schemes across different thread counts, the two
different machines, and across different sizes.
Figure~\ref{fig:times} (a) shows the runtime for \union{} for varying
sizes across the four balancing schemes on all 64
cores of the AMD-based machine.  The first thing to note is that the
times are very similar across the balancing schemes---they
differ by no more than 10\% once the size is $10^6$ or greater.  For
smaller inputs there is some difference, with treaps up to three times
slower than AVL trees at $10^4$.  However we did not optimize our code
for small sizes so we would not put much significance on those times.

Figure~\ref{fig:times} (b) shows the speedup curves for the AMD-based
machine for \union{} on two inputs of size $10^8$.  All balancing
schemes achieve a speedup of about 40 on 64 cores, and about 30 on 32
cores.  The less-than-linear speedup beyond 32 cores is not
due to lack of parallelism, since when we ran the same experiments on
significantly smaller input (and hence less parallelism) we get very
similar curves (not shown).  Instead it seems to be due to saturation
of the memory bandwidth.  Figure~\ref{fig:times} (c) shows the speedup
curves for the Intel-based machine.  The speedups are similar, also
achieving about 40 fold speedup.  Note, however, that the Intel
machine is hyperthreaded so there are only 40 cores.  Beyond 40
threads one should expect less than linear speedup due to sharing of
the cores by the threads.

Since all code except for \join{} is shared among the balancing
schemes, the experiments are a good indication of the relative merits
of the balancing scheme while controlling for other factors.  The
conclusion is that all schemes perform about equally.  This is perhaps
not surprising since the dominant cost is in cache misses along the
paths in the tree, and all schemes keep the trees reasonably balanced.
The AVL trees are always slightly faster than the other trees and this
is likely due to the fact they maintain slightly stricter balance than
the other trees, and hence the paths that need to be traversed are
slightly shorter.

\paragraph{Comparing functions}
We use AVL trees as the representative trees to compare different
functions on maps.  Figure~\ref{fig:times} (d) compares the \union,
\intersect, \difference, and \filter{} functions.  For the first three
the size of the larger tree is fixed, while the size of the smaller
tree is varied from $10^4$ to $10^8$.  Since \filter{} only operates
on a single tree, it uses the smaller tree as its input.  For the
filter condition we choose to keep all entries with a value that is
even.  Since values are random, about half are kept.    As the
plot indicates, the first three functions (\union, \intersect, and
\difference) have very similar performance, while \filter{} is a
factor of between two and three times faster for larger inputs.  This
is not surprising given the similarity of the code for the first three
functions, and the fact that \filter{} effectively works on half as
many keys since it takes one input instead of two.

Figure~\ref{fig:times} (e) compares two approaches for building a
tree from a sequence of (unsorted) key-value pairs.  One of them uses
\build{} as introduced in section \ref{sec:operations}.  The second
approach presorts the data using the parallel STL sorting routine, and then
uses a recursive application of \join{} to build the tree from the
resulting array.  Both methods require $O(n \log n)$ work, although
the \join{}-based method only does $O(n)$ work on the trees, and the
rest in the sort.  The experiments show that the \join{}-based \build{}
performs better than the \union{}-based one for all but the smallest
input.  On the largest input it is an order of magnitude better.  This
is because directly sorting is significantly faster than sorting based
on union (with all the overhead of maintaining trees).  The cost of
joining is then a small part ($O(n)$ work).  On the small input it appears that the
STL parallel sort is not suited for small problems and the bad
performance is due to lack of parallelism.    We make use of the \join{}-based
version in our library.

Figure~\ref{fig:times} (f) compares \union{} when applied
destructively and persistently.  The code is the same, but for the
destructive version we wrap a \texttt{final} around both input
arguments first, allowing the code to update the nodes in place.  The
destructive application ends up non needing any new nodes, and only
frees nodes when a duplicate is found.  The version without
\texttt{final}s, on the other hand, has to create a linear number of
new nodes.  The experiments indicate that the destructive version is
about 40\% faster.  This is a good indication of the extra cost of
copying nodes and shows that the optimization for in-place updates
have practical consequence.

\paragraph{Comparing to STL} 
The STL supports ordered maps and sets
using red-black trees.  The interface includes basic functions such as
insertion and deletion, and also supports the aggregate function
\texttt{set\_union}, \texttt{set\_intersection}, and
\texttt{set\_difference}.  The functions are not parallel, not
persistent and not safe for concurrency.  Figure~\ref{fig:times} (g)
compares times for our \join{}/\split{} based implementation (as defined in
Figure~\ref{fig:insertanddelete}), a direct implementation based on our
AVL trees, and the STL insert.  All experiments insert key-value pairs
in a random order, and are with our parallel code running on a single core.  The
experiments show that our direct insert is about twice as fast as the
\join{}/\split{} version, and about 15\% slower than the STL insert.
One would expect the \join{}/\split{} version to be slower since it
has to traverse the tree twice, once to split and once to join.  One
would also expect our version to be slower than STL since we have to
maintain all the reference counts and be safe for concurrency.

STL supports \union{} on any sorted container class, including maps
based on red-black trees, and sorted vectors (arrays).  We
compare our \union{} to both, even though sorted vectors are clearly
not efficient for other operations such as insert or delete.  The STL
\union{} merges the two sorted containers by moving from left to right
on the two inputs, comparing the current values, and writing the lesser
to the end of the output.  For two inputs of size $n$ and $m$, $m >
n$, it takes $O(m + n)$ time on vectors, and $O((m+ n) \log (n+m))$
time on red-black trees (each insertion at the end of the output
red-black tree takes $O(\log(n+m))$ time).  Figure~\ref{fig:times} (h)
compares times for \union{}.  For equal lengths our implementation is
about a factor of 8 faster than STL maps (red-black trees), and about
8 times slower than STL vectors.  This is not surprising since we are
asymptotically faster than their red-black tree implementation, and
their array-based implementation just reads and writes the values in
order from flat arrays, and therefore has much less overhead and many
fewer cache misses.  For taking the union of smaller and larger inputs
our \union{} is orders of magnitude faster than either STL version.
This is because they both take time proportional to the larger length
while ours takes $O(n \log (m/n))$  work (time).


==> exp__.tex <==
\section{Experiments}
\label{sec:exp}
We implement our algorithms for range queries and segment queries using a parallel augmented map library (PAM)~\cite{ourppopp}. This library provides simple and efficient interface for augmented map functions, on top of which all of our algorithms only need about 100 lines of code. Some examples are given in Appendix \ref{app:codeexample} and we plan to make all our code available on GitHub. All the algorithms in this library match the versions described in this paper. More details about PAM and the functions it supports are in Appendix \ref{app:pam}. The library supports persistence by path-copying.

For 2D range queries, we test the range tree in Section \ref{sec:rangetree} (\emph{RangeTree}) and the sweepline algorithm in Section \ref{sec:rangesweep} (\emph{RangeSweep}). 
%The RangeSweep for reporting sum of weights and the full list differ in the augmentation, so we use RangeSweepS and RangeSweepA for the two \sweepstructure{}s respectively. 
For 2D segment queries, we test the \segtree{} in Section \ref{sec:segmenttree} (\emph{SegTree}), the sweepline algorithm in Section \ref{sec:segsweep} (\emph{SegSweep}) and the counting version in Section \ref{sec:segcount} (\emph{SegCount}). We compare with a sequential library CGAL \cite{overmars1996designing}. We test both queries on reporting sum of weights (\emph{query-sum}) and all queried elements (\emph{query-all}).  On reporting all queried elements, since the cost is largely affected by the output size, we test a small and a large query window with average output size less than $10$ and about $10^6$ respectively. We accumulate query time of $10^3$ large-window queries and $10^6$ small window queries. For query-sum we accumulate $10^6$ queries picked uniformly randomly in the whole range. For parallel queries we run all queries in parallel.
We use $n$ for the input size, $p$ for the number of threads. All coordinate ranges are set to be $0$ to $10^9$. For the sweepline algorithms we set $k=p$, and do not repeat applying the parallel paradigm to blocks.
%We do not test very large windows because we believe in real settings the queries tend to be a small fraction of the input set and are very unlikely to be, say, the same order of magnitude of the total input size. The theoretical bounds for all the tested functions are given in Table \ref{tab:allexpcost}.


We run experiments on a 72-core Dell R930 with 4 x Intel(R)
Xeon(R) E7-8867 v4 (18 cores, 2.4GHz and 45MB L3 cache) with 1GB memory.  Each core is
2-way hyperthreaded giving 144 hyperthreads.  Our code was compiled
using the g++ 5.4.1 compiler which supports the Cilk Plus extensions.
We compile with \ctext{-O2}.

In the rest of this section we first show results on range queries and segment queries respectively, and then give comparisons across all tested structures, as well as some conclusions in the summary part.

\begin{figure}[!h]
  \centering\small
\begin{minipage}{0.33\columnwidth}
 \centerline{\includegraphics[width=1\columnwidth]{figures/range-seq.pdf}}
\end{minipage}
\begin{minipage}{0.15\columnwidth}
\centering{\textbf{(a).} \\ \textbf{Range Query},\\ $p=1$,\\ varying $n$}
\end{minipage}
\begin{minipage}{0.33\columnwidth}
 \centerline{\includegraphics[width=1\columnwidth]{figures/range-speed.pdf}}
\end{minipage}
\begin{minipage}{0.15\columnwidth}
\centering{\textbf{(b).} \\ \textbf{Range Query},\\ $n=10^8$,\\ varying $p$}
\end{minipage}\\
\begin{minipage}{0.33\columnwidth}
 \centerline{\includegraphics[width=1\columnwidth]{figures/seg-seq.pdf}}
\end{minipage}
\begin{minipage}{0.15\columnwidth}
\centering{\textbf{(c).} \\ \textbf{Segment Query}, \\$p=1$,\\ varying $n$}
\end{minipage}
\begin{minipage}{0.33\columnwidth}
 \centerline{\includegraphics[width=1\columnwidth]{figures/seg-speed.pdf}}
\end{minipage}
\begin{minipage}{0.15\columnwidth}
\centering{\textbf{(d).} \\ \textbf{Segment Query},\\ $n=10^8$,\\ varying $p$}
\end{minipage}\\
  \caption{\small{The sequential time and speedup of building various data structures answering range queries and segment queries.}}\label{fig:expfigures}
\end{figure}

\para{2D Range Queries.}
We test our implementation on RangeTree and RangeSweep addressing 2D range queries, querying both the sum of weights and the full list, sequentially and in parallel. We show the running time on $n=10^8$ in Table \ref{tab:rangetable}. We also give the sequential running time over different input sizes and the speedup on $n=10^8$ points in Figure \ref{fig:expfigures} (a) and (b).
We compare our sequential version with the CGAL \cite{overmars1996designing} library, which is sequential and only supports query-all. We cannot find a comparable parallel C++ implementation of range query problems, so we just compare the two versions (RangeSweep vs. RangeTree) of our implementations. 

We first look at the sequential performance. Figure \ref{fig:expfigures}(a) show that the RangeSweep and RangeTree demonstrate similar performance and significantly outperform CGAL. RangeTree scales better to large data and outperforms RangeSweep on very large data. Among all, RangeTree constructs the fastest (see Table \ref{tab:rangetable}), which is about 25\% faster than RangeSweep and 50\% faster than CGAL.

We then discuss the parallel performance. As shown in Figure \ref{fig:expfigures}(b), on $n=10^8$, the speedup scale up to 144 threads. On $10^8$ points and all 144 threads, RangeTree can finish the construction in 4.7s, achieving a 55-fold speedup (see Table \ref{tab:rangetable}). RangeSweep has relatively worse parallel performance. It achieves a 35-fold speedup and spends 9s on construction using all 144 threads. This is mainly because of its theoretical parallel depth ($\tilde{O}(\sqrt{n})$ vs. logarithmic). As for RangeTree not only the construction is highly-parallelized, the combine function (\texttt{union}) is also parallelizable.
%Also, notice the algorithm itself and its parallel depth depends on the parameter $k$ (the number of blocks), which is set to be $p$ (the number of threads), so for different values of $p$ we are not comparing exactly the same algorithm.

For queries, if only the sum of weights is required, the RangeSweep algorithm shows the best performance in both theory and practice. It only requires two plain binary searches on the top level and then two range queries, while the RangeTree requires one range query on the top, and then at most $\log n$ of such range queries. On query-all, RangeSweep is much slower than the other two because of its bad theoretical bound (See table \ref{tab:allexpcost}) especially when query window is large. For small windows, it shows better performance (see Table \ref{tab:rangetable}), which is consistent with theoretical bounds. RangeTree, in the query-all case, largely outperforms the other two algorithms. As for speedup of parallel queries, except for the query-all of range trees, the speedup numbers are about 80-90 because they are embarrassingly parallelized. The bad speedup of the query-all using RangeTree is due to the limitation of the bandwidth. On reporting all large-window queries, in total $10^9$ elements are processed in $0.7$s, indicating a processing rate of $1.4\times 10^9$ elements per second. This is almost the upper limit of our machine.

\begin{table}
\small
  \centering
    \begin{tabular}{|@{}c@{}||r|r|r||r|r|r||r|r|r|r|r|r|}
    \hline
       \multirow{2}{*}{\textbf{Algorithm}}   &  \multicolumn{3}{c||}{\textbf{Build, s}} &        \multicolumn{3}{c||}{\textbf{Query-sum, $\boldsymbol{\mu}$s}} &      \multicolumn{3}{c|}{\textbf{Query-all (small), $\boldsymbol{\mu}$s}} &      \multicolumn{3}{c|}{\textbf{Query-all (large), ms}}\\
\cline{2-13}
          & \multicolumn{1}{c|}{\textbf{Seq.}} & \multicolumn{1}{c|}{\textbf{Par.}} & \multicolumn{1}{c||}{\textbf{Spd.}} &  \textbf{Seq.} &\textbf{Par.} & \textbf{Spd.} &  \multicolumn{1}{c|}{\textbf{Seq.}} & \multicolumn{1}{c|}{\textbf{Par.}} & \multicolumn{1}{c|}{\textbf{Spd.}}&  \multicolumn{1}{c|}{\textbf{Seq.}}&\textbf{Par.} & \textbf{Spd.}\\
    \hline\hline
{\bf RangeSweep} &    323.74 &      9.02 &   35.88 &      8.89 &      0.115 &   77.28 &          6.81 &          0.08 &   84.05       &          193.45  & 2.11 &   91.90 \\
\hline
%{\bf RangeSweepAll} &    341.19 &      9.67 &   35.27 &          - &          - &          - &     6.81& 0.08 & 84.05 &    193.45 &      2.11 &   91.90 \\
%\hline
{\bf RangeTree} &     258.59 &       4.71 &   54.90 &      50.16 &      0.63 &   80.00 &     27.43 &      0.34 &   81.89 &     24.28 &      0.71 &   34.30 \\
\hline
{\bf CGAL} &    525.94 &          - &          - &          - &          - &          - &    153.54 &          - &          - &    110.94 &          - &          - \\
%\hline
%{\bf Output Size} &   \multicolumn{3}{c||}{-} &       \multicolumn{3}{c||}{-} &        \multicolumn{3}{c|}{10.61} &      \multicolumn{3}{c|}{$1.05\times 10^6$} \\
    \hline \hline
{\bf SegSweep} &    383.12 &      8.94 &   42.88 &      5.60 &      0.072 &   77.72 &      5.42 &      0.072 &       75.29 &      94.10 &      1.43 &   65.67 \\
\hline
{\bf SegTree} &     582.68 &     11.30 &   51.56 &      47.54 &      0.571 &    83.26 &     38.17 &      0.43 &   83.26 &      30.12 &      1.16 &      26.01 \\
\hline
{\bf SegCount} &    239.91 &      4.38 &   54.84 &       31.40 &      0.44 &   71.05 &          - &          - &          - &          - &          - &          - \\
%\hline
%{\bf Output Size} &   \multicolumn{3}{c||}{-} &       \multicolumn{3}{c||}{-} &        \multicolumn{3}{c|}{10.61} &      \multicolumn{3}{c|}{$1.00\times 10^6$} \\
\hline
    \end{tabular}\vspace{-.3em}
    \caption{\small{The running time of different data structures on range queries ($n=10^8$) and segment queries ($n=5\times 10^7$). ``Seq.'', ``Par.'' and ``Spd.'' refer to the sequential, parallel running time and the speedup respectively.}}\vspace{-1em}
  \label{tab:rangetable}%
\end{table}%
\hide{For query-all we also adjust window size of the query (see details in Section \ref{sec:expsetting}). Seq. and Par. represent sequential and parallel time respectively. We give the CGAL range tree (sequential) time for comparison.}

%All structures in this table have $10^8$ elements in the tree. 
\para{2D Segment Query.}
In this section we show the running times on segment queries using SegSweep, SegTree and SegCount. We give all running times on $n=5\times 10^7$ in Table \ref{tab:rangetable}. We also show the sequential running time and the parallel speedup in Figure \ref{fig:expfigures}(c) and (d). Notice that for these structures on input size $n$, actually $2n$ elements are in the tree (two endpoints per segment). Thus we set input size to be $n=5\times 10^i$ for comparison with the range queries. We do not find comparable implementations on exactly the same problem we are addressing so that we just compare our three implementations with each other.

We first look at the sequential performance. As shown in Figure \ref{fig:expfigures} (c), SegCount constructs the fastest, while SegTree runs slower than the other two. This is fairly reasonable because SegTree stores four sets (the \opensets{} and the \symdiff{}) in each node, and calls two \texttt{diff} functions and two \texttt{union} functions in each combine process. Similarly, SegCount constructs faster than the other two probably because it only reports the sum of weight, indicating less information stored in the tree.

For parallel performance, all three data structures scale up to 144 threads (see Figure \ref{fig:expfigures} (d)). For $n=5\times 10^7$ input segments, SegCount has the least construction time of 4.38s. Comparing SegTree and SegSweep, even though SegTree has better speedup (51 vs. 43), it is still slower than SegSweep both sequentially and in parallel. The lack of parallelism of SegSweep is because of the same reason as RangeSweep.

We then discuss the performance on answering queries. On reporting the sum of weights, SegSweep shows significant efficiency compared to the other two because of its better theoretical cost. SegCount shows better performance than SegTree probably because of its simpler structure and more intuitive searching processing. As for querying all segments, SegTree is faster than SegSweep on large query window, but is slower when window is small. This may be of the reason that the secondary range query on y-coordinate, for SegSweep, is just a range searching on a large tree containing all segments across the x-coordinate in query. For SegTree, however, the y-range-query is conducted on many smaller trees (the \symdiff{}), and in all would save time when output size is large. The query speedup for all queries except SegTree on large windows is over 60. The low speedup of SegTree on large window queries is of the same reason (limitation of the bandwidth) as that of RangeTree.


\para{Summary.}
Since all results in Table \ref{tab:rangetable} are on $10^8$ elements, we briefly compare all the tree structures. There are two types of algorithms: sweepline algorithms SegSweep and RangeSweep, and multi-level trees RangeTree, SegTree and SegCount. For the construction of multi-level trees, with properly defined augmentation, the construction is automatically done by PAM augmented map constructor, which is highly-parallelized (logarithmic depth). For the sweepline algorithms, the parallelism comes from the blocking-and-batching process. Thus the speedup of the sweepline algorithms is slightly worse than the multi-level trees.
The two sweepline algorithms has close construction time, but RangeSweep performs better in parallel. A reason might be that the in SegSweep for each block insertions and deletions are batched separately (while in RangeTree all updates are insertions and are batched in one tree) such that parallelism is sacrificed. For the multi-level trees, SegTree is much slower than the other two. This is because it stores more information in each node (four maps) and has more complicated augmentation.

For range queries, RangeTree costs less construction time especially on large data, and is more efficient in reporting the full list of queried points for large output size. The RangeSweep algorithm is especially good in just reporting the sum of weights or the full list with small size. For the segment queries, although SegCount constructs faster, it only answers weight queries. SegSweep reports weight sum rather fast and requires reasonable constructing time. For query-all, SegTree answer queries the most efficiently on large output size, but requires longer construction time.

\hide{
\begin{table}[!h]
\small
  \centering
\begin{tabular}{|c||r|r|r||r|r||r|r|r|r|}
\hline
           &   \multicolumn{ 3}{c||}{{\bf Build}} & \multicolumn{ 2}{c||}{{\bf Query-sum}} &            \multicolumn{ 4}{c|}{{\bf Query-all}} \\
\hline
           & {\bf Seq.} & {\bf Par.} & {\bf speedup} &    {$\boldsymbol{m}$} & {\bf Time} &    {$\boldsymbol{m}$} & {\bf Small} & {\bf Medium} & {\bf Large} \\
\hline
{\bf Sweepline} &    339.64 &    13.99 & 24.28&    $10^5$ &   0.67 &    $10^3$ &   0.14 &    11.69 &    120.79 \\
\hline
{\bf SegTree} &    575.84 &    10.43 & 55.23 &    $10^5$ &    5.32 &    $10^3$ &   0.11 &    4.71 &    42.71 \\
\hline
{\bf SegCount} &    279.27 &    7.02 & 39.81 &    $10^5$ &    3.90 &          - &          - &          - &          - \\
\hline
\end{tabular}
    \caption{Seg Query}
  \label{tab:segtable}%
\end{table}%
}


\hide{
\begin{table*}[!h]
  \centering
    \begin{tabular}{|c||r|r|r||r|r|r||r|r|}
    \hline
          & \multicolumn{3}{c||}{\textbf{Build}} &        \multicolumn{3}{c||}{\textbf{Query-sum}} &      \multicolumn{2}{c|}{\textbf{Query-all}} \\
    \hline
          & \multicolumn{1}{c|}{\textbf{$\bf p=1$}} & \multicolumn{1}{c|}{\textbf{$\bf p=144$}} & \multicolumn{1}{c||}{\textbf{speedup}} & \multicolumn{1}{c|}{\textbf{$\bf p=1$}} & \multicolumn{1}{c|}{\textbf{$\bf p=144$}} & \multicolumn{1}{c||}{\textbf{speedup}} & \multicolumn{1}{c|}{\textbf{small}} & \multicolumn{1}{c|}{\textbf{large}} \\
    \hline
    {\textbf{RangeSweep}} & 352.54 & 9.21 & 38.26 & 9.91 & 0.11 & 90.94 &  0.026 & 5.318  \\
    \hline
    {\textbf{RangeTree}} & 245.23 & 4.90 & 50.03 & 63.56 & 0.67 & 94.47 & 0.017 & 0.283  \\
    \hline
    \textbf{CGAL} & 514.36 &    -   &   -    &   -    & -      &     -  & 0.210 & 2.624 \\
    \hline
    \end{tabular}%
    \caption{Range Query}
  \label{tab:range}%
\end{table*}%
} 

==> imple.tex <==
\section{Library Implementation}
\label{sec:imple}

We have implemented the library using the \join-based approach described in
previous sections for all four balancing schemes (AVL trees, RB trees,
WB trees, and treaps).  The only code that depends on the balancing
scheme are the implementations of \join{}.  For AVL trees we also
directly implemented \insertnew{} for the purposes of
comparison.  Our implementation is in C++ using the \texttt{Cilk-Plus}
extension to support nested parallelism (fork-join using spawn and
sync, and parallel loops).  For our reference counting garbage
collector we also make significant use of compare-and-swap for
lock-free synchronization among the threads.

\subsection{Implementing persistence}
One way to achieve persistence is to copy the entire input before the
function is applied.  This, however, can be much more costly than the
function itself (e.g. for \insertnew{}, \join{}, \split{}).  Instead
we copy the path from the root down to the modification being made.
Figure~\ref{fig:insert} shows an example of such path copying.  All
the nodes along the path that are copied share any pointers to nodes
off the path (in the example both copies of node $5$ share a pointer
to node 8).  In general this means that large parts of trees end up
being shared among different maps.  This is the same approach as used
by default in purely-functional languages.

If all nodes along the path have constant memory size (which is true
in binary trees), path copying only has a constant factor overhead
relative to mutating updates.  This constant, however, has
some practical significance
(we study this cost in our experiments).  Our \texttt{final} function
can be used to avoid this cost.  It allows for in-place updates when
safe.  In particular if the user indicates with \texttt{final} that
this is the final use of a tree, and for any node in the tree that is
not shared with any other trees, that node can be updated in place
rather than requiring a copy.  If the next node(s) in the path is
also updated in place, then no update is needed at all, avoiding some
writes, allocation, and later garbage collection.  The use of
destructive updates on the final copy is a well studied optimization in the
functional programming community~\cite{Hudak86,Wadler90,Odersky91}.

To determine if nodes are shared we use a reference counting collector, which is
described in more detail below.  For now assume that a reference count
of one indicates that there is only one pointer to the structure, and
therefore it is safe to update in place (the only pointer is the one
currently being used).  When entering a function on a map that is not
finalized, the reference count to the root is incremented indicating
that in addition to all existing pointers to the root, the function
itself now has a pointer.   However, when the map is finalized, then
the reference count is left unchanged, indicating that the pointer to the
map is now being handed to the function, and the pointer in the
finalized map is set to empty.    If the count is one, then updates
can be made in place (if not finalized, the reference count will never
be one).     Our map functions include code for updating reference
counts.

\begin{figure}
\centering
  \includegraphics[width=0.95\columnwidth]{figures/Tree_insertion} \\
  \caption{The figure shows the insertion of a node with key 4 into a tree which is shared among two sets. Since
	the root has a reference count of 2 the copying of nodes is propagated along the insertion path. On the last figure
	we fix the reference counts of the nodes which have been copied and adjust the pointers accordingly.}
  \label{fig:insert}
\end{figure}



\subsection{Reference Counting Collection}
We use a reference counting garbage collector for memory management of
the tree nodes.  Every node includes a reference count that indicates
the number of references to it, and a node is collected when its count
goes to zero.  The benefit of using a reference counting collector is
twofold.  Firstly, as discussed above, the reference count can detect
nodes that are not shared with any other tree, and can thus be
immediately reused.  This avoids having to allocate a new node, free
the old node, and copy values from the old to the new.  The second
benefit is that nodes can be collected as soon as their count goes to
zero, so that the memory footprint is always almost equal to the
number of reachable (live) nodes.  Since trees do not have cycles,
even when shared, there is no issue with collecting cycles.

Our collector is parallel, safe for concurrency, and lock-free.  We
use compare-and-swap to atomically update all reference counts.  To be
safe for concurrency, the collector also never decrements a counter before
all needed fields are extracted (sequential reference counting can
decrement first since no other thread can see the decrement).  When a
count is decremented to zero, the current thread returns the node to
the memory pool (described below) and recursively decrements the child
pointers.  The decrements could themsleves reduce the counts to zero,
possibly recursively collecting a large portion of the tree.  The
calls are therefore applied in parallel (using nested fork-join), so
the collector is parallel requiring at most $O(\log n)$ span to
collect a balanced tree of size $n$.

We implemented our own memory pool for the nodes.  The nodes are all
the same size, so no provisions are needed for different sized
objects.  To reduce the contention on a shared pool, we use the
standard approach of having each operating system thread maintain its
own local \emph{small stack} of free nodes as a linked list.
Allocations of new nodes are popped from the local small stack, and
freed nodes are pushed onto the local stack.
%all without synchronization as long as there are nodes remaining or
%the stack is not full.
In addition we maintain a global pool of small stacks using
a lock-free \emph{global stack}--each stack element is a small stack
of fixed size $s$ (16K nodes in our current version).  Whenever a
local stack runs out of nodes, the thread goes to the global stack and
pops off another small stack of $s$ nodes to use locally.  Also,
whenever a local stack reaches size $2 \times s$, the thread splits
the stack in half, and returns one of the two parts as a small stack
to the global stack.  It keeps the other half as the local stack.
This guarantees that there are at least $s$ push and pop steps on the
local stack before going back to the global stack.  The global stack
is maintained as a linked list accessed through a head structure, which
consists of a pair of adjacent words, the first pointing to the head
of the stack and the second to a version number.  A two-word (16 byte)
compare-and-swap is used to atomically update the pair, always
incrementing the version number.  This avoids locking or the ABA
problem.  The implementation currently aborts when the 64-bit version
number overflows, which would take over 1000 years on a current 64
core system running full tilt.

The user can specify how many nodes they use with the \texttt{reserve}
function, but if they underestimate and the global stack runs out of memory, the
first thread detecting it will initiate the allocation of more space.
New small stacks are constructed in parallel and placed into the
global stack.  This is the only place where threads can block on
another thread---while waiting for the small stacks to be added.

\subsection{Augmenting property}
Considering the definition of the augmented value attribute and the
associativity of the augmented reduce function $f$, the augmented value
of some node $T$,
although is defined based on the information in the whole subtree, can be
calculated directly from its two children and $T$ itself,
i.e.,
\begin{align*}
\augvalueone{T} = \begin{cases} g(k(T), v(T)) & T \mbox{ is a leaf}\\
f(\augvalueone{L(T)}, g(k(T), v(T)), \augvalueone{R(T)}) & \mbox{otherwise} \end{cases}
\end{align*}
This property guarantees that the asymptotically complexity of main functions unaffected supposing both $g$ and $f$
take constant time.

The only difference in maintaining the augmented value of different balancing schemes still lies in \join.
In each function, the update of the augmented values occurs only when any one of its children has its augmented value changed.
In the functions in \ourname{}, these are also the exact nodes whose heights or weight (size) may change. Thus the augmented values can be updated incidentally after updating the height or size.
\hide{
In \join{}, most of the nodes keep their augmented value unchanged, except those on the
path from the root to where the connecting point is determined. Note that if rotations are involved, the
rotation roots and pivots\footnote{Recall that in the tree rotation, we call the original subtree root (parent) node the \emph{rotation root} and the new subtree root (parent) the \emph{rotation pivot}. We view the double rotation as two consecutive single rotations.} also have new augmented values. These are also the exact
nodes whose heights or weight (size) may change during \join{}. Thus the augmented values can be updated incidentally after updating the height or size.
}

==> index-exp.tex <==
\subsection{Word Index Searching}

To test the performance of the inverted index data structure described
in Section~\ref{sec:index} we use the publicly available Wikipedia
database~\cite{Wikipedia} (dumped on Oct. 1, 2016) consisting of 8.13
million documents.  We removed all XML markup, treated everything
other than alphanumeric characters as separators, and converted all
upper case to lower case to make searches case insensitive.  This
leaves 1.96 billion total words with 5.09 million unique words.  We
assigned a random weight to each word in each document (the values of
the weights make no difference to the runtime).

For construction we measure the time for the constructor
\texttt{\small inv\_index}, which takes an array of \texttt{(word, (doc\_id, weight))}
triples and generates the full augmented inverted index.  For queries
we selected a set of 100K word pairs and for each we run the following
query:
\begin{quote}
\ttfamily\small
\begin{lstlisting}[numbers=none,language=C++,escapechar=@]
vector<post_elt> query(word w1, word w2) {
  post_list p1 = idx.get_list(w1);
  post_list p2 = idx.get_list(w2);
  post_list pr = idx.And(p1, p2);
  return idx.top_k(pr, 10);
}
\end{lstlisting}
\end{quote}
The query extracts the posting lists for the two words, take the
logical \cand{} over the lists (an intersection), and then returns the
10 documents with the highest scores.  The pairs of words were
selected as follows.  The first word is selected uniformly at random
across the whole input.  This makes common words more likely since
they appear more often.  The second word is selected uniformly at
random among words that appear in at least 100 documents, and with all
duplicates removed.  Even though this filters out low frequency words,
these words tend to be less frequent since they are not biased
by multiple occurrences.  The total size across all posting lists
selected (200K of them) is 181 billion entries.  The total result size
of the \cand{} is 267 Million (an average of about 1300 per result).
Of these the 10 highest scores are selected, as described above.

Timings are shown in Table~\ref{fig:word}.  It was surprising to us
that the structure can build the index of wikipedia in 15 seconds, and
can answer 100K queries with a total of close to .2 trillion documents
across the queries in under 7 seconds.  The space required by the
index is about 38 Gbytes, and an additional 30 Gbytes are required to
build the structure.

\begin{table}
\begin{center}
\begin{tabular}{|l||C||C|C||C|C|}
\hline
       & \multirow{3}{*}{\textbf{n}} & \multicolumn{2}{c||}{\textbf{1 Core}} & \multicolumn{2}{c|}{\textbf{72 Cores}} \\ \cline{3-6}
       &     & \textbf{Time} & \textbf{Gelts/} & \textbf{Time}& \textbf{Gelts/} \\[-.05in]
       &    & \textbf{(secs)} & \textbf{sec} & \textbf{(secs)} & \textbf{sec} \\ \hline
\textbf{Build}   &  1.96 \times 10^9 &  553  & .0035  &  15.1 & .13  \\ \hline
\textbf{Queries}  & 1.81 \times 10^{11} &  420  & .43   &  6.6 &  27.8 \\ \hline
\end{tabular}
\end{center}
\vspace{-0.2in}
\caption{The running time and rates for building
and queering an inverted index. Gelts/sec calculated as $n/(\mbox{time} \times 10^9)$.}
\label{fig:word}
\vspace{-.2in}
\end{table}


==> interface.tex <==

\section{Library Interface}
\label{interface}
\begin{newpart}
\subsection{The \texttt{augmented\_map} Class}
We implemented a C++ library for ordered sets and maps
based on the ideas presented in previous sections.  The library
supports persistence, is implemented so that aggregate functions run
in parallel, and is safe for concurrency.
The library uses the \texttt{augmented\_map} as the only interface and defined plain maps and sets as special case of it (maps are implemented as augmented maps with empty augment type, and sets are implemented as maps with empty value).
It is implemented by adding
an operation type to a normal tree, which contains the augmented reduce function $f(\cdot,\cdot)$, the augmented singleton function $g(\cdot,\cdot)$, and the augmented value type $\augtype$.
This $\augtype$ is not necessary to be the same type as the key type or value type.
In the library we use C++ templates to specialize to specific key and value types, as well as the augmented operation type such that it supports augmented maps of different types and operations simultaneously.
The interface \texttt{augmented\_map<K, V, Op>} requires the following templates:
\begin{itemize}
\item \textbf{\texttt{K}} -- The key type. This type must support a comparison function ($<$) that properly defines a total order over its elements.
\item \textbf{\texttt{V}} -- The value type.
\item \textbf{\texttt{Op}} -- The operation type. It must contains the following attributes and methods:
\begin{enumerate}
  \item \textbf{Typename \texttt{aug\_t}} -- The type $\augtype{}$ of the augmented value attribute. It is not necessary to be the same type as key type \texttt{K} or value type \texttt{V}.
  \item \textbf{Static method \texttt{from\_entry(K, V)}} -- This function defines the augmented singleton function $g:K\times V \mapsto \augtype$.
  \item \textbf{Static method \texttt{combine(aug\_t, aug\_t)}} -- This function defines the augmented reduce function $f:\augtype \times \augtype \mapsto \augtype$.
\end{enumerate}
\end{itemize}

\renewcommand{\arraystretch}{1.2}
\begin{table}
\begin{center}
	\begin{tabular}{l|c|c}
	\hline
	\textit{\textbf{Function}} & \textbf{Work} & \textbf{Span} \\
	\hline
\multicolumn{3}{l}{Tree Node attributes}\\
\hline
	\texttt{size}, \texttt{height} & $1$&$1$  \\
	\hline
\multicolumn{3}{l}{BST operations}\\
\hline
	\texttt{insert}, \texttt{delete}, \texttt{find} & \multirow{4}{*}{$\log n$} & \multirow{4}{*}{$\log n$}\\
	\texttt{next}, \texttt{previous},  & & \\
\texttt{first}, \texttt{last}, \texttt{item\_rank} & \\
\texttt{select} & & \\
\hline
\texttt{content} & $n$ & $\log n$\\
	\hline
\multicolumn{3}{l}{Aggregate operations}\\
\hline
	\texttt{union}, \texttt{intersect},  &  \multirow{2}{*}{$n \log (\frac{m}{n} + 1)$} & \multirow{2}{*}{$\log m \log n$} \\
\texttt{difference} & \\
	\hline
	\texttt{forall} & $n$ & $\log n$ \\
	\hline
	\texttt{filter} & $n$ & $\log^2 n$ \\
	\hline
	\texttt{range}, \texttt{split} & $\log n$ & $\log n$ \\
\hline
\multicolumn{3}{l}{Tree constructions}\\
\hline
\texttt{singleton}  & $1$ &$1$ \\
	\hline
	\texttt{build} (unsorted) & $n \log n$ & $\log n$ \\
    \hline
    \texttt{build} (sorted) & $n$ & $\log n$\\
	\hline
\multicolumn{3}{l}{Memory management}\\
\hline
\texttt{reserve}, \texttt{init} & n & $1$ \\
\hline
\texttt{clear}, \texttt{finish} & $1$ &$1$ \\
\hline
\multicolumn{3}{l}{Augmented operations}\\
	\hline
\texttt{aug\_right}, \texttt{aug\_left},  & \multirow{2}{*}{$O(\log n)$} & \multirow{2}{*}{$O(\log n)$}\\
\texttt{aug\_range} & &\\
\hline
	\end{tabular}
	\end{center}
	%\nocaptionrule
\caption{The core functions in our map and set library and their
      asymptotic costs (all big-O).  The cost is given under the assumption that
      the reduce function takes constant time to return. For \union{}, \intersect{} and
      \difference{}, $m$ is the size of the larger input, and $n$ of
      the smaller.}
    \label{tab:interface}
\end{table}




\subsection{Functions and Interfaces}
The list of core functions (described in Section \ref{sec:algorithm}) along with their costs is given in Table
\ref{tab:interface}.

Other than the
The library has its own memory manager.  Maps are allocated by the
various map functions that create them, and freed using
\texttt{clear}.  The library also supplies functions to initialize the
library (\texttt{init}), to reserve some number of nodes
(\texttt{reserve}), and to free the memory when no longer needed
(\texttt{finish}).
% The initialization needs to be called before any
%of the other library functions are called.
The \texttt{reserve} is a
hint for the memory manager, but the library will allocate nodes on
demand if none or not enough were reserved.
%No functions can be called after the \texttt{finish}.

By default all the functions over maps are persistent, meaning that
they do not modify their arguments.  However, the library also gives a
way to specify that one or more arguments are no longer needed when
the function completes.  In particular the user can wrap
\texttt{final} around any map that is an argument to a function, and
when the function is applied it will free (clear) that map.  For
example, \texttt{mapR = union(mapA,mapB)} will create a new map
without modifying \texttt{mapA} or \texttt{mapB}, but \texttt{mapR =
  union(mapA,final(mapB))} will create a new map, leave \texttt{mapA}
as it was, but free \texttt{mapB}.  As described in the next
section, the implementation is careful to only free the nodes that
are not shared among maps.  We note that
\texttt{union(mapA,final(mapB))} is semantically equivalent to
\texttt{union(mapA,mapB); clear(mapB)}, but, as discussed in the next
section, the prior can be more efficient.

\begin{comment}
 However, and obviously, it is
unsafe to call \texttt{clear} or \texttt{final} on a map that is still
being operated on concurrently by any other function.  All results are
fully deterministic independent of interleaving of concurrent tasks
since the functions create new values instead of mutating old ones
(unless final, in which case other copies should no longer be
accessed).
\end{comment}

\begin{comment}
The difference between a tree map and an augmented map is that the latter accepts a binary operator as its thrid argument.
Each node of an augmented map stores the application of the binary operator on the values of the tree rooted at itself.
For this reason augmented maps support an \texttt{accumulate} function. It accepts a key $k'$, and returns the application
of the binary operator on all nodes with a key $k \leq k'$. Table \ref{tab:interface} lists the core functions which are supported by all of our containers.

Most of the functions mentioned in Table \ref{tab:interface} are self-explanatory, and we won't go in much detail into them.
In Table \ref{tab:interface} we didn't list any of the methods which are responsible for allocating and freeing nodes.
The memory allocator is not bound to individual object instances, as it is usually implemented. The reason for this
is that due to persistence two or more objects can share a subset of nodes with each other. The memory allocator we provide
operates on the level of class instances and is accessed through three methods: \texttt{init} is used to initialize the memory allocator of a particular map or set class,
\texttt{reserve} accepts a number $n$ and allocates memory for $n$ nodes, and \texttt{finish} destroys the memory allocator and frees all the memory occupied by it. \\

The method responsible for freeing nodes of individual objects is \texttt{clear}, which effectively empties the content of the container.
\texttt{clear} invokes the garbage collection and recollects all nodes which don't belong to a tree anymore.
\end{comment}

All functions listed in Table~\ref{tab:interface} are safe to be called
concurrently even on the same maps.

The \texttt{build} function initialize an augmented map from a list of key-value pairs.
Except the begin and end iterator of the list, it also takes two other parameters: a flag
indicating if the input is pre-sorted or not, and a construct reduce function that will be applied
if duplicate keys exist. Building a tree from a pre-sorted list costs asymptotically less than
an arbitrary list. In the list, if multiple entries have the same key $k$, since $k$ can appear at most once in
the map, the construct reduce function will be applied on all values under $k$, and the result will be
the new value of $k$ in the final augmented map.

Also as mentioned in \ref{sec:algorithm}, the map versions of
\texttt{union} and \texttt{intersect} accept a third argument, which
is itself a function.  If any keys appear in both trees, the function
is applied to the corresponding pair of values to generate a new value
to associate with that key.  For example, this can be used to keep a
count for each key, and have union and intersection sum the counts.
By default the function returns its first argument, so that when two
keys are the same in a union or intersection, the first value (from the
argument on the left) is kept.
\end{newpart}

\begin{table*}
\begin{center}
	\begin{tabular}{l|c|c}
	\hline
	\textit{\textbf{Function}} &\textbf{Parameters} &\textbf{Description}  \\
	\hline
\multicolumn{3}{l}{\textbf{Map operations of $M$}}\\
\hline
\texttt{content}$()$ & & M\\
\hline
\texttt{insert}$(e)$& $e\in K \times V$ & $M\cup \{e\}$\\
\hline
\texttt{delete}$(e)$& $e\in K \times V$ & $M - \{e\}$\\
\hline
\texttt{find}$(k)$& $k\in K$ & $v:\langle k,v\rangle\in M$\\
\hline
\texttt{next}$(k)$& $k\in K$ & $e:e\in M, k(e)=\min_{e\in M} k(e)>k$\\
\hline
\texttt{previous}$(k)$& $k\in K$ & $e:e\in M, k(e)=\max_{e\in M} k(e)<k$\\
\hline
\texttt{first}$()$&  & $e:e\in M, k(e)=\min_{e\in M} k(e)$\\
\hline
\texttt{last}$()$&  & $e:e\in M, k(e)=\max_{e\in M} k(e)$\\
\hline
\texttt{item\_rank}$(k)$& $k\in K$ & $|\{e|e\in M, k(e)<k\}|$\\
\hline
\texttt{select}$(i)$ & $i\in \mathbb{Z_{+}}$ & $e:\left|\{e'|e'\in M, k(e')<k(e)\}\right|=i-1$\\
\hline
\texttt{forall}$()$ & ?? & ??\\
\hline
\texttt{filter}$(\phi)$ & $\phi:K\mapsto \{0,1\}$ & $\{e\,|\,\phi(k(e))\}$ \\
\hline
\texttt{range}$(k_1,k_2)$ & $k_1,k_2\in K$ & $\{e\,|\,k_1<k(e)<k_2\}$ \\
\hline
\texttt{split}$(k')$ &$k'\in K$ & $\langle \, \{e\,|\,e\in M, k(e)<k'\}, \mathbbm{1}\left[k'\in M\right], \{e\,|\,e\in M, k(e)>k'\} \,\rangle$\\
\hline
\multicolumn{3}{l}{\textbf{Augmented operations of map $M$}}\\
\hline
\texttt{aug\_left}$(k)$  & $k\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')<k\}$ \\
\hline
\texttt{aug\_right}$(k)$  & $k\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k(e')>k\}$ \\
\hline
\texttt{aug\_range}$(k_1,k_2)$  & $k_1,k_2\in K$ &$\augvalue{f}{g}{M'} \,:\, M'=\{e'\,|\, e'\in M, k_1<k(e')<k_2\}$ \\
\hline
\multicolumn{3}{l}{\textbf{Aggregate operations}}\\
\hline
\multirow{2}{*}{\texttt{join}$(M_1,k',M_2)$} & $M_1,M_2\subseteq U, k'\in K$ & \multirow{2}{*}{$M_1\cup\{k'\}\cup M_2$} \\
& $\max_{e\in M_1}k(e)<k'<\min_{e\in M_2}k(e)$ &\\
\hline
\multirow{2}{*}{\texttt{joinTwo}$(M_1,M_2)$} & $M_1,M_2\subseteq U$ & \multirow{2}{*}{$M_1\cup M_2$} \\
& $\max_{e\in M_1}k(e)<\min_{e\in M_2}k(e)$ &\\
\hline
\multirow{3}{*}{\texttt{union}$(M_1, M_2, \sigma)$}& \multirow{2}{*}{$M_1,M_2\subseteq U$} & $\{\langle k,v\rangle\,|\,\langle k,v\rangle\in M_1,\forall v', \langle k',v\rangle\notin M_2\}\cup$\\
&\multirow{2}{*}{$\sigma:V\times V \mapsto V$}&$\{\langle k,v\rangle\,|\,\langle k,v\rangle\in M_2,\forall v', \langle k',v\rangle\notin M_1\}\cup$\\
&&$\{\langle k,\sigma(v_1, v_2)\rangle\,|\,\langle k,v_1\rangle\in M_1,\langle k,v_2\rangle\in M_2\}$\\
\hline
\multirow{2}{*}{\texttt{intersection}$(M_1, M_2, \sigma)$}& \multirow{1}{*}{$M_1,M_2\subseteq U$} & \multirow{2}{*}{$\{\langle k,v\rangle\,|\,\langle k,v\rangle\in M_2,\forall v', \langle k',v\rangle\notin M_1\}$}\\
&\multirow{1}{*}{$\sigma:V\times V \mapsto V$}&\\
\hline
\texttt{difference}$(M_1,M_2)$ & $M_1,M_2\subseteq U$& $M_1-M_2$\\
\hline
\multicolumn{3}{l}{\textbf{Map constructions}}\\
\hline
\texttt{singleton}$(e)$  & $e\in K\times V$ &$\{e\}$ \\
\hline
\multirow{2}{*}{\texttt{build}$(s, \sigma)$} & $s=\langle e_1, e_2,\dots, e_n \rangle$ & $\{ (k(e),\Sigma_{\sigma}\langle s'\rangle)) \,|\, e\in s, s'=\langle v(e_{i_1}), v(e_{i_2}), \dots v(e_{i_m})\,:\, $ \\
&$\sigma:V\times V\mapsto V$& $\forall j, 1\le j\le m, e_{i_j}\in s,k(e_{i_j})=k(e), i_1<i_2\dots<i_m\rangle\}$\\
\hline

%\multicolumn{3}{l}{Memory management}\\
%\hline
%\texttt{reserve}, \texttt{init} & n & $1$ \\
%\hline
%\texttt{clear}, \texttt{finish} & $1$ &$1$ \\
%\hline
	\end{tabular}
	\end{center}
	%\nocaptionrule
\caption{The core functions.}
    \label{tab:functions}
\end{table*}


==> interval-exp.tex <==
\subsection{Interval Tree}
We tested our interval tree code (as shown in Section \ref{intro}). We vary the input tree size from $10^4$ to $10^8$.

We compare the sequential performance of our interval tree with a Python interval tree implementation~\cite{IntervalPython}. The Python implementation is sequential, and is very inefficient. We ran the Python interval tree only up to a tree size of $10^7$ because it already took about $200$s to build the tree when the size is $10^7$, and can hardly accept larger trees as input. The sequential running time of our code and the Python interval tree is reported in Table \ref{tab:interval}. In building the tree, our code is about dozens of times more efficient than the Python implementation, and in performing queries, is orders of magnitude faster. Our code can answer millions of queries in one second, while the Python interval tree can only do $418$ per second when $n$ is as small as $10^4$, and this processing rate deceases dramatically when $n$ gets larger. The sequential running time of our implementation is also given in Figure \ref{fig:it-exp} (a).

We also give the parallel performance of our PAM interval tree in Figure \ref{fig:it-exp} (b) and (c). Figure (b) shows the building time on 144 threads. On $10^8$ points, the parallel code can build an interval tree in less than 0.4 second. Figure (c) shows the speedup trend with various number of threads. The construction of an interval tree can get almost-linear speedup up to 32 cores, which is a 23-fold speedup.

\begin{table}[!h!t]
  \centering
    \begin{tabular}{|c||r|r||r|r|}
    \hline
    \multirow{3}{*}{\textbf{n}}     & \multicolumn{2}{c||}{\textbf{Build}}        & \multicolumn{2}{c|}{\textbf{Queries}}   \\
    \cline{2-5}
          & \multicolumn{1}{c|}{\textbf{Python}} & \multicolumn{1}{c||}{\textbf{PAM}} & \multicolumn{1}{c|}{\textbf{Python}} & \multicolumn{1}{c|}{\textbf{PAM}} \\[-.04in]
    & \multicolumn{1}{c|}{\textbf{Melts/sec}} & \multicolumn{1}{c||}{\textbf{Melts/sec}} & \multicolumn{1}{c|}{\textbf{queries/sec}} & \multicolumn{1}{c|}{\textbf{queries/sec}} \\
    \hline
    $\bf 10^4$ & 0.102 & 8.264 & 417.981 & 13.333$\times 10^6$ \\
    \hline
    $\bf 10^5$ & 0.059 & 17.147 & 26.105 & 28.169$\times 10^6$ \\
    \hline
    $\bf 10^6$ & 0.064 & 16.437 & 2.520 & 24.038$\times 10^6$ \\
    \hline
    $\bf 10^7$ & 0.049     & 13.063 & 0.209     & 22.845$\times 10^6$ \\
    \hline
    $\bf 10^8$ & -     & 12.247 & -     & 21.067$\times 10^6$ \\
    \hline
    \end{tabular}%
    \vspace{-.1in}
\caption{The processing rate of the Python interval tree and PAM interval tree on $n$ points. The ``Build'' column shows the millions of input entries processed per second (calculated as n/(build-time$\times 10^6$)). In ``Queries'' we show the number of queries processed per second (calculated as query-number/query-time).}  \label{tab:interval}%
\vspace{-.2in}
\end{table}%

\begin{figure*}[!h!t]
\begin{tabular}{ccc}
\includegraphics[width=0.66\columnwidth]{figures/interval/interval.pdf}&    \includegraphics[width=0.66\columnwidth]{figures/interval/interval2.pdf} &  \includegraphics[width=0.66\columnwidth]{figures/interval/it-speedup.pdf} \\
  (a) & (b) & (c)\\
\end{tabular}
  \caption{The performance of the interval tree implemented with PAM interface. Figure (a) shows the sequential running time of PAM interval tree on construction (left y-axis) and performing one query (right y-axis) respectively. Figure (b) shows the running time of construction on 144 threads. Figure (c) shows the speedup on various numbers of processors with $10^8$ points in the tree. }\label{fig:it-exp}
\end{figure*}


==> lib.tex <==
\section{The library: \ourname{}}
\label{sec:lib}


\subsection{Parallelism}
\subsubsection{The Parallel Model}


\subsubsection{The \texttt{split-join} Model}
We implement our functions based on the algorithms in \cite{ours}, which is built upon a \texttt{join-split} model.
In this model, ...

The \join$(L,k,R)$~\cite{Tarjan83} function takes a key $k$ and two
BSTs $L$ and $R$ storing two ordered sets, such that $k$ is greater than all keys in $L$
and less than all keys in $R$.  It returns the ordered set containing
$L \cup \{k\} \cup R$ (The map version also takes a value associated with the key).
We implement \join{} separately for each balancing schemes as described in \cite{ours}.
Based on \join{}, other operations and set functions can be implemented generally.
The function \split$(T,k)$ split a BST $T$ into two disjoint subsets storing
keys larger than and smaller than $k$ respectively. The set functions
\union{}, \intersect{} and \difference{} are defined as usual.
The functions are implemented as described in~\cite{ours}.

It has be shown that our implementations of all the set functions
are work-optimal and of polylog-span~\cite{ours}. The core functions along with
their costs are given in Figure \ref{tab:costs}.




\subsection{Memory Management}
Other than the
The library has its own memory manager.  Maps are allocated by the
various map functions that create them, and freed using
\texttt{clear}.  The library also supplies functions to initialize the
library (\texttt{init}), to reserve some number of nodes
(\texttt{reserve}), and to free the memory when no longer needed
(\texttt{finish}).
% The initialization needs to be called before any
%of the other library functions are called.
The \texttt{reserve} is a
hint for the memory manager, but the library will allocate nodes on
demand if none or not enough were reserved.
%No functions can be called after the \texttt{finish}.


\subsection{Reference Counting}

\textbf{History Persistence}. By default all the functions over maps are persistent, meaning that
they do not modify their arguments.  However, the library also gives a
way to specify that one or more arguments are no longer needed when
the function completes.  In particular the user can wrap
\texttt{final} around any map that is an argument to a function, and
when the function is applied it will free (clear) that map.  For
example, \texttt{mapR = union(mapA,mapB)} will create a new map
without modifying \texttt{mapA} or \texttt{mapB}, but \texttt{mapR =
  union(mapA,final(mapB))} will create a new map, leave \texttt{mapA}
as it was, but free \texttt{mapB}.  As described in the next
section, the implementation is careful to only free the nodes that
are not shared among maps.  We note that
\texttt{union(mapA,final(mapB))} is semantically equivalent to
\texttt{union(mapA,mapB); clear(mapB)}, but, as discussed in the next
section, the prior can be more efficient.

\textbf{Data Persistence}.

\textbf{Garbage Collector}.





==> lis.tex <==
\subsection{Longest Increasing Subsequence}
\label{sec:lis}
The longest increasing subsequence (LIS) problem is to find the longest subsequence (not necessarily contiguous) of a given sequence in which the subsequence's elements are in sorted order. It has been shown to be related to many applications in various areas such as patience sorting \cite{mallows1963patience,aldous1999longest}, Young tableaux \cite{schensted1961longest,aldous1999longest}, patience diff algorithm in version control systems such as Bazaar, etc. Straight-forward dynamic programming algorithm computes LIS at the cost of $O(n^2)$, which can be improved to $O(n\log n)$ \cite{donald1999art,fredman1975computing}. It has been shown that the lower bound of the cost of a comparison-based algorithm to find the LIS in a sequence of length $n$ is $O(n\log n)$ \cite{fredman1975computing}. There also exists work showing that finding LIS on a permutation of $[n]$ (which means that each element in the sequence is drawn from integers from $1$ to $n$, and each integer appears exactly once in the sequence), can be done in $O(n\log \log n)$ time~\cite{bespamyatnikh2000enumerating}.

In this section, we give a worst-case $O(n\log n)$ algorithm to compute both the length and the count of the longest increasing subsequence for an arbitrary given sequence. It is also not hard to output one longest increasing subsequence using a variant of our algorithm. In this section we use $s_{[i]}$ to denote the subsequence $\langle s_1, s_2,\dots s_i\rangle$ in $s$.

Most algorithms to compute LIS are based on the following formula:
\begin{align}
\label{eqn:lis1}
l(i) &= \max_{j:j<i,s_j<s_i} l(j)+1\\
\label{eqn:lis2}
c(i) &= \sum_{j:j<i,s_j<s_i,l(j)=l(i)-1} c(j)\\
L& = \max_{i} l(i)\\
C& = \sum_{j:l(j)=L} c(j)
\end{align}
, where the $l(i)$ denotes the LIS length in $s_{[i]}$ ending with $s_i$ (we call it the \emph{rear LIS length} of node $i$), and $c(i)$ denotes the number of LISes with length $l(i)$ in $s_{[i]}$ ending with $s_i$ (we call it the \emph{rear LIS count} of node $i$). $L$ and $C$ are the LIS length and count of the whole sequence respectively.

The code for computing the length and the count of a given sequence $s=\langle s_1, s_2,\dots s_n\rangle$ is shown in Fig. \ref{fig:lis}.
For computing the LIS length and count, we build an augmented tree from scratch by inserting the elements in $s$ from left to right into the tree. In each tree node the key stores the key of an element $s_i$ in the sequence, and the value stores a pair of integers $\langle l(i),c(i)\rangle$, i.e., the rear LIS length and the rear LIS count . Based on Eqn. \ref{eqn:lis1} and Eqn. \ref{eqn:lis2} we know that augmented reduce function takes the larger $l(i)$ along with its $c(i)$ in the two operand pairs. If the two pairs has the same $l(i)$, the augmented reduce function take this $l(i)$ as the new rear LIS length and the rear LIS count is computed from the sum of the two operands' rear LIS count.

On building the augmented-map $m$, we generate each entry from the left to right of $s$ and insert them in the tree. The $i$-th entry has the key of $s_i$, and we only need to compute the value of it. According to Eqn. \ref{eqn:lis1} and Eqn. \ref{eqn:lis2}, the set $S_i$ of elements that we use to compute the value of the current node are those with index $j$ in $s$ which are currently in $m$ (i.e., $j<i$) and whose keys are smaller than $s_i$ (i.e., $s_j<s_i$). These are the exact elements visited by \texttt{aug\_left\_ex}$(s_i)$ on the current tree $m$. The returned value $\langle l',c' \rangle$ of the function \texttt{aug\_left\_ex}, can be used to compute the value of the current node by $\langle l'+1, c'\rangle$. Then this entry $\langle s_i, \langle l'+1, c'\rangle \rangle$ is inserted into the tree. After the tree is built, the augmented value on the root is the answer of the whole sequence.

It is worth noting that the base case of an empty value, which means that no elements smaller than $s_i$ appears in front of it, is $\langle 0,1 \rangle$. This is because the empty sequence should be counted as one subsequence of $s$. Combining this answer with the current node $s_i$, it means that the rear LIS length is $1$ (just the element itself) and the count is $1$ (the single element is the only case).


\hide{
The code for computing the length and the count of a given sequence $s=\langle s_1, s_2,\dots s_n\rangle$ is shown in Fig. \ref{fig:lis}.
For computing the LIS length, we build an augmented tree from scratch by inserting the elements one by one into the tree. In each tree node the key stores the key of an element $s_i$ in the sequence, and the value stores the length of the LIS in $s_{[i]}$ ending with $s_i$ (i.e., the $l(i)$). Based on Eqn. \ref{eqn:lis1} we define the augmented reduce function to be the \texttt{max} on values, and the augmented singleton function accordingly just returns its value. On building the augmented-map $m$, we generate each entry from the left to right of $s$ and insert them in the tree. The $i$-th entry has the key of $s_i$, and according to Eqn. \ref{eqn:lis1}, its value can be computed from one plus the maximum value on all nodes with inserting order $j$ which are currently in $m$ ($j<i$) and whose keys are smaller than $s_i$ ($s_j<s_i$). This exact answer can be returned by \texttt{aug\_left\_ex}$(s_i)+1$ on the current tree $m$.

To get the count of the LIS, we record an extra field in the value, which is the $c(i)$ in Eqn. \ref{eqn:lis2}. The augmented value is a pair of $\langle l(i),c(i)\rangle$. The augmented reduce function takes the larger $l(i)$ along with its $c(i)$ in the two operand pairs.
If the two pairs has the same $l(i)$, the augmented reduce function take this $l(i)$ as the new LIS length and the LIS count is computed from the sum of the two operands' LIS count.
}


\begin{figure}[!t]
\ttfamily\small
\begin{lstlisting}[language=C, frame=lines]
typedef pair<int,int> ipair;
ipair LIScount(int* A, int n) {
  struct aug {
    using aug_t = ipair;
    static aug_t from_entry(int k, ipair v) {
      return v;}
    static aug_t combine(aug_t a, aug_t b) {
      if (b.first > a.first) return b;
      if (a.first > b.first) return a;
      return ipair(a.first,a.second+b.second);
    }
	static aug_t get_empty() {return ipair(0,1);}
  };
  augmented_map<int, ipair, aug> m;
  for (int i=0; i < n; i++) {
    ipair x = m.aug_left_ex(A[i]);
    ipair new_val = ipair(x.first+1, x.second);
    m.insert(make_pair(A[i], new_val));
  }
  return m.aug_val();
}
\end{lstlisting}
\caption{The data structure and construction of the LIS problem under our augmented tree framework.}
\label{fig:lis}
\end{figure} 

==> operations.tex <==
\begin{figure}[!h!t]
\begin{lstlisting}[frame=lines]
split$(T,k)$ =
  if $T$ = Leaf then (Leaf,false,Leaf)
  else $(L,m,R)$ = expose$(T)$;
    if $k = m$ then ($L$,true,$R$)
    else if $k < m$ then
      $(L_L,b,L_R)$ = split$(L,k)$;
      ($L_L$,$b$,join$(L_R,m,R)$)
    else $(R_L,b,R_R)$ = split$(R,k)$;
      (join$(L,m,R_L),b,R_R)$  @\vspace{.1in}@
splitLast($T$) =
  $(L,k,R)$ = expose$(T)$;
  if $R$ = Leaf then ($L,k$)
  else $(T',k')$ = splitLast($R$);
    (join($L,k,T'$),$k'$)@\vspace{.1in}@
join2($\Tl$,$\Tr$) =
  if $\Tl$ = $\leaf$ then $\Tr$
  else $(\Tl',k)$ = splitLast($\Tl$);
    join($\Tl',k,\Tr$)@\vspace{.1in}@
union($T_1$,$T_2$) =
  if $T_1$ = Leaf then $T_2$
  else if $T_2$ = Leaf then $T_1$
  else ($L_1$,$k_1$,$R_1$) = expose($T_1$);
    ($L_2$,$b$,$R_2$) = split($T_2$,$k_1$);
    ($\Tl$,$\Tr$) = union($L_1$,$L_2$) || union($R_1$,$R_2$);
    join($\Tl$,$k_1$,$\Tr$)@\vspace{.1in}@
intersect($T_1$,$T_2$) =
  if $T_1$ = Leaf then Leaf
  else if $T_2$ = Leaf then Leaf
  else ($L_1$,$k_1$,$R_1$) = expose($T_1$);
    ($L_2$,$b$,$R_2$) = split($T_2$,$k_1$);
    ($\Tl$,$\Tr$) = intersect($L_1$,$L_2$) || intersect($R_1$,$R_2$);
    if $b$ = true then join($\Tl$,$k_1$,$\Tr$)
    else join2($\Tl$,$\Tr$) @\vspace{.1in}@
singleton$(v)$ = join(Leaf,$v$,Leaf)@\vspace{.1in}@
build($A$,$n$) = @\label{line:builds}@
  if $n$ = $0$ then Leaf
  else if $n$ = $1$ then singleton($A[0]$)
  else ($T_1$,$T_2$) = build($A$,$\lfloor\frac{n}{2}\rfloor$) || build($A+\lfloor\frac{n}{2}\rfloor$,$n-\lfloor\frac{n}{2}\rfloor$);
    union($T_1$,$T_2$) @\label{line:builde}@ @\vspace{.1in}@
\end{lstlisting}
\caption{Pseudocodes of some functions implemented by \join.} \label{fig:pseudocode}
\end{figure}
\hide{
forall($T$,$f$) = @\label{line:forall}@
  if $T$ = Leaf then Leaf
  else ($L$,$(k,v)$,$R$) = expose($T$);
    join(forall($L$,$f$),$(k,f(v))$,forall($R$,$f$))@\vspace{.1in}@
filter($T$,$f$) =
  if $T$ = Leaf then Leaf
  else ($L$,$k$,$R$) = expose(T);
    if $f(k)$ then join(filter($L$,$f$),$k$,filter($R$,$f$))
    else join2(filter($L$,$f$),filter($R$,$f$))@\vspace{.1in}@
range$(T,l,r)$ =
  ($T_1$,$T_2$) = split($T,l$);
  ($T_3$,$T_4$) = split($T_2$,$r$);
  $T_3$@\label{line:last}@
join2($\Tl$,$\Tr$) =
  if $\Tl$ = $\leaf$ then $\Tr$
  else if $\Tr$ = Leaf then $\Tl$
  else if $r(\Tr)\ge r(\Tl)$ then
    ($L_R,k_R,R_R$) = expose($\Tr$);
    join(join2($\Tl$,$L_R$),$k_R$,$R_R$)
  else ($L_L,k_L,R_L$) = expose($\Tl$);@\label{line:join2expose}@
    join($L_L$,$k_L$,join2($R_L$,$T_R$))@\label{line:join2join}@ @\vspace{.1in}@
}

\section{Functions Using JOIN}
\label{sec:operations}
The \join{} function, as a subroutine, has been used and studied by many
researchers and programmers to implement more general set operations.
In this section, we describe algorithms for various functions that use
just \join{}.  Beyond \join{} the only access to the trees we make use of
is through \expose{} and $r(\cdot)$, which only read the root. The
main set operations, which are \union{}, \intersect{} and \difference{},
are optimal (or known as \emph{efficient}) in work.

The algorithms are generic across balancing schemes, but the cost
analysis depends on the scheme.  The pseudocodes for the algorithms in this section is shown in Figure \ref{fig:pseudocode}.

\para{Split.}
For a BST $T$ and key $k$, \split{}$(T,k)$ returns a triple $(\Tl,b,\Tr)$, where $\Tl$ ($\Tr$) is a tree containing all keys less (larger) than $k$ in $T$, and $b$ is a flag indicating whether $k \in T$.  The algorithm first searches for $k$ in $T$, splitting the tree along the path into three parts: keys to the left of the path, $k$ itself (if it exists), and keys to the right.  Then by applying \join{}, the algorithm merges all the subtrees on the left side (using keys on the path as intermediate nodes) from bottom to top to form $\Tl$, and merges the right parts to form $\Tr$.
Figure~\ref{fig:split} gives an example.
%The pseudocode is shown in Figure \ref{fig:insertandsplit}.

\begin{figure*}[t!h!]
\centering
  \includegraphics[width=1.9\columnwidth]{figures/split.pdf}\\
  \caption{An example of \split{} in a BST with key $42$. We first search for $42$ in the tree and split the tree by the searching path, then use \join{} to combine trees on the left and on the right respectively, bottom-top. }
\label{fig:split}
\end{figure*}


\begin{theorem}
\label{thm:split}
The work of \split{}$(T,k)$ is $O(\log |T|)$ for all balancing schemes described in Section \ref{sec:paradigm} (w.h.p. for treaps).
\end{theorem}
\proof{} We only consider the work of joining all subtrees on the left side.
The other side is symmetric. Suppose we have $l$ subtrees on the left side, denoted from bottom to top as $T_1,T_2,\dots T_l$.  We have that $r(T_1)\le r(T_2)\le\dots\le r(T_l)$. As stated above, we consecutively join $T_1$ and $T_2$ returning $T'_2$, then join $T'_2$ with $T_3$ returning $T'_3$ and so forth, until all trees are merged. The overall work of \split{} is the sum of the cost of $l-1$ \join{} functions.

For AVL trees, red-black trees and weight-balanced trees, recall Theorem \ref{thm:main} that we have $r(T_{i+1})\le r(T'_{i+1}) \le r(T_{i+1})+1$, so $r(T'_i)\le r(T_i)+1\le r(T_{i+1})+1$. According to Theorem \ref{thm:main}, the work of a single operation is $O(|r(T_{i+1})-r(T'_i)|)$. The overall complexity is $\sum_{i=1}^{l} |r(T_{i+1})-r(T'_i)|\le \sum_{i=1}^{l} r(T_{i+1})-r(T'_i)+2=O(r(T))=O(\log |T|)$.
\hide{
\begin{align*}
&\sum_{i=1}^{l} |h(T_{i+1})-h(T'_i)|\\
\le&\sum_{i=1}^{l} h(T_{i+1})-h(T'_i)+4\\
%\le& 4l+\sum_{i=1}^{l} (h(T_{i+1})-h(T_i))\\
\le& 5h(T)= O(h(T))
\end{align*}
}

For treaps, each \join{} uses the key with the highest priority since
the key is always on a upper level.  Hence by Lemma \ref{lem:treap}, the
complexity of each \join{} is $O(1)$ and the work of split is at
most $O(\log |T|)$ w.h.p.  \qed

%Notice that in the process of splitting a treap, when we call \join{}, the key is always of a higher priority since it is on a upper level than the two subtrees. Thus \join{} could be done in $O(1)$ time.

\para{Join2.}
\joinTwo{}$(\Tl,\Tr)$ returns a binary tree for which the in-order
values is the concatenation of the in-order values of the binary trees
$\Tl$ and $\Tr$ (the same as \join{} but without the middle key).
For BSTs, all keys in $\Tl$ have to be less than keys in $\Tr$.
\joinTwo{} first finds the last element $k$ (by following the right spine) in $\Tl$ and
on the way back to root, joins the subtrees along the path, which is similar to \split{}
$\Tl$ by $k$. We denote the result of dropping $k$ in $T_L$ as $\Tl'$. Then \join($\Tl',k,\Tr$)
is the result of \joinTwo. Unlike \join{}, the work of \joinTwo{} is
proportional to the log of size of both trees since
both \split{} and \join{} take at most logarithmic work..

\hide{$(\Tl,\Tr)$ returns a binary tree for which the in-order
values is the concatenation of the in-order values of the binary trees
$\Tl$ and $\Tr$ (the same as \join{} but without the middle value).
For BSTs, all keys in $\Tl$ have to be less than keys in $\Tr$.  The
algorithm is recursive.  Assume $\Tl$ has a higher rank than $\Tr$, it
then exposes the larger tree $\Tl$ into $(L_L,k_L,R_L)$
(line~\ref{line:join2expose}), recursively applies
\joinTwo{}$(R_L,\Tr)$ to get $T'$, and then applies
\join($L_L,k_L,T'$) to merge the three parts
(line~\ref{line:join2join}).
  Unlike \join{}, the work of \joinTwo{} is
proportional to the log of size of both trees.
}
\begin{theorem}
\label{thm:join2}
The work of $T=$ \joinTwo{}$(\Tl,\Tr)$ is $O(\log |\Tl| + \log |\Tr|)$ for all balancing schemes described in Section \ref{sec:paradigm} (bounds are w.h.p for treaps). %For AVL trees, RB trees and WB trees, $\max(r(\Tl),r(\Tr))\le r(T) \le 1+\max(r(\Tl),r(\Tr))$. %, where $c$ is a constant.
\end{theorem}
%The proof of the theorem is not trivial and will be presented in the final version.

\hide{ \proof{} We prove the case when $r(\Tl)\ge
  r(\Tr)$, the other case is symmetric.

We first prove that $\max(r(\Tl),r(\Tr))\le r(T) \le c+\max(r(\Tl),r(\Tr))$, where $c$ is a constant. Recall Theorem \ref{thm:main} that \join{} on AVL trees, RB trees and WB trees will increase the rank by at most one.

For AVL trees, we use induction on $r(\Tl)+r(\Tr)$. If $r(\Tl)=r(\Tr)=r$, it will recursively \joinTwo{} $R(\Tl)$ with $L(\Tr)$, getting $T'$ of rank at most $r$. Then \joinTwo$(L(\Tl),$\joinTwo$(T',R(\Tr)))$. Denote the intermediate result of \joinTwo$(T',R(\Tr))$ as $T''$. If $r(T')<r$, $r(T'')$ is at most $r$, and \joinTwo$(L(\Tl),T'')$ will get the final result of rank at most $r+1$. The rank increases by at most $1$. If $r(T')=r$, \joinTwo$(T',R(\Tr))$ will insert $R(\Tr)$ into the right spine of $T'$ without affecting the left spine, and \joinTwo$(L(\Tl),T'')$ will insert $L(\Tl)$ into $T''$'s (which is exactly $T'$'s) left spine. Each process could increase the rank of $T'$'s one child, and as a result, $T$'s rank will be at most $1+r(T')=1+r$. The rank increases by at most one.

If $r(\Tl)=r>r(\Tr)$, the \joinTwo$(R(\Tl),\Tr)$ will get $T'$ of rank at most $r$, and then $\join(L(\Tl),k(\Tl),T')$ will get the final result of rank at most $r+1$.

For red-black trees, we use induction on $r(\Tl)+r(\Tr)$. If $r(\Tl)=r(\Tr)=r$, it will recursively join $R(\Tl)$ with $L(\Tr)$, getting $T'$. Notice that if $k(R(\Tl))$ is red, the rank of $R(\Tl)$ is still $r$ (when processing the subtree $R(\Tl)$, we should first convert the root into black to guarantee it is valid). If so, $R(R(\Tl))$ must be black. Assume that $k(R(\Tl))$ and $k(L(\Tr))$ are both red, the algorithm should first let $T'=$\joinTwo$(R(R(\Tl)),L(L(\Tr)))$, then \join{} it with $R(L(\Tl))$, then with $L(R(\Tr))$, then with $L(\Tl)$, then with $R(\Tr)$. Notice that the left spine and the right spine still do not affect each other. We just show on the left spine, the process will make $r(T)$ to be $r+2$. From the inductive assumption we know that $r(T')$ is at most $r+1$. If $r(T')<r+1$, it is trivial that $r(T)\le r+2$. Assume $r(T')=r+1$. Notice that $r(R(L(\Tr)))=r-1$. When joining $R(L(\Tr))$ with $T'$, if the rank of the result is $1+r(T')$, it will make all the nodes from $k(R(L(\Tr)))$ to $T'$'s root to be black. Thus when further joining $L(\Tl)$, the double red case will not happen, and the rank of $T$ will stay $1+r(T')=r+2$. If $k(R(\Tl))$ and $k(L(\Tr))$ are not both red, similar analysis will lead the same result that $r(T)\le r+2$. If $r(\Tl)=r>r(\Tr)$, the analysis is similar.

For weight-balanced trees, the conclusion is trivial.

Now we prove the bound on the work of \joinTwo. We make induction on $r(\Tl)+r(\Tr)$. Denote the complexity to be $W(r_1,r_2)$ for \joinTwo{} two trees of rank $r_1$ and $r_2$. When $r_1+r_2=1$, the theorem obviously holds. Assuming the theorem holds for $r_1+r_2<k$, i.e., $W(r_1,r_2)\le c(r_1+r_2)$ holds for some constant $c$. When $r_1+r_2=k$, we have $W(r_1,r_2)\le W(r_1-1,r_2)+t_{\rm{join}}$, where $t_{\rm{join}}$ is the time required by the final \join{} step. From the inductive assumption, the rank of $T'$ (which is the result of \joinTwo($R_L,\Tr$) is at most $r(R_L)+2$. Thus from Theorem \ref{thm:main} we know that the \join($L(\Tl),k(\Tl),T'$) takes only constant time $c'$. Let $c=c'$, we have $W(r_1,r_2)\le c'(r_1+r_2-1)+c'=c'(r_1+r_2)=O(\log |\Tl| + \log |\Tr|)$.

For treaps, we substitute the rank $r(\cdot)$ in the above proof by the height $h(\cdot)$ and get the same conclusion.
\qed
}

\para{Union.}
\union{}$(T_1,T_2)$ takes two BSTs and returns a BST that contains the union
of all keys.   The algorithm uses a classic
divide-and-conquer strategy, which is parallel.   At each level of recursion,
$T_2$ is split by $k(T_1)$, breaking $T_2$ into three parts: one with all keys smaller than $k(T_1)$ (denoted as $L_2$), one in the middle either of only one key equal to $k(T_1)$ (when $k(T_1)\in T_2$) or empty (when $k(T_1) \notin T_2$), the third one with all keys larger than $k(T_1)$ (denoted as $R_2$).
%with keys equivalent to $T_1$'s root (just a bit $b$ to show if this part is empty).
%Meanwhile, all keys in the left (right) subtree of $T_1$ are originally smaller (larger) than $k(T_1)$.
Then two recursive calls to \union{} are made in parallel.  One unions
$L(T_1)$ with $L_2$, returning $\Tl$, and the other one unions
$R(T_1)$ with $R_2$, returning $\Tr$.  Finally the algorithm returns
\join$(\Tl,k(T_1),\Tr)$, which is valid since $k(T_1)$ is greater than
all keys in $\Tl$ are less than all keys in $\Tr$.

\hide{In general cases, \union{} tend to split the smaller tree instead of the larger one, while for treaps we use the root with a higher priority as the pivot. This exception is to guarantee that in the \join{} process, the key is always prior to the two tree roots, allowing the \join{} to take $O(1)$ time by directly creating \node$(\Tl,k(T_1),\Tr)$. Thus the algorithm will always uses the root of a higher rank as the pivot.}

%Use the similar method, we can implement union operation of two ordered sets. Since union should be applied to two sets, the two input trees should have no duplicates, and the returned tree should also have no duplicates. The only difference is to replace the line labeled with $(*)$ by $\left<T_2^L,T_2^M,T_2^R\right>=\texttt{split3}(T_2,T_1.\rm{root})$.

\begin{theorem}
\label{thm:unionwork}
For all the four balance schemes mentioned in Section \ref{sec:paradigm}, the work and span of the algorithm (as shown in Figure~\ref{fig:pseudocode}) to union two balanced BSTs of sizes $m$ and $n$ ($n\le m$) is $\displaystyle O\left(n\log\left(\frac{m}{n}+1\right)\right)$ and $O(\log m \log n)$ respectively (the bound is in expectation for treaps).
\end{theorem}

A generic proof of Theorem \ref{thm:unionwork} and \ref{thm:indiwork}
working for all the four balancing schemes will be shown in the next section.
\fullin{
The span of \textal{Union} can be reduced to $O(\log m)$ by
doing a more complicated divide-and-conquer strategy based on (1)
finding splitters that divide the result into blocks of size $(m \log
m)/(n \log(m/n +1))$, (2) for each block in parallel, extracting the
block from each input with \split{} and taking the union of the results,
and (3) joining the results in parallel using a tree.}


The work bound for \union{} is optimal in the comparison-based model.
In particular considering all possible interleavings, the minimum
number of comparisons required to distinguish them is $\log
{m+n \choose n}=\Theta\left(n\log
  \left(\frac{m}{n}+1\right)\right)$ \cite{hwang1972simple}.

\fullin{
\begin{theorem}
\label{thm:unionoptimal}
The parallel algorithm \textal{Union} is optimal in terms of work. %work-efficient \footnote{A \emph{work-efficent} algorithm is one that uses no more work than a comparable serial algorithm}.
\end{theorem}}
\hide{
\proof{} Here we prove that the theoretical lower bound of the work of \textal{Union} is $\Omega(n\log(\frac{m}{n}+1))$. We treat the BSTs as ordered lists, so union two sets are equivalent to merging two lists of size $m$ and $n$, and get a new list of size $m+n$. As the lists are ordered, it is equivalent to take $n$ positions out of all the $m+n$ slots for $T_1$ (which is also equivalent to choose $m$ slots for $T_2$). Thus the theoretical lower bound of this algorithm is:
%the total number of cases is equivalent to the number of cases to pick up $n$ positions in $m+n$ slots to put the elements in $T_1$, and the rest $m$ slots are filled in with the elements in $T_2$. Thus the theoretical lower bound of this algorithm is:
\begin{align*}
W(m,n)&=\log \left(\begin{array}{c}
m+n\\
n
\end{array}
\right)\\
%&\ge\log (\frac{M+N}{N})^N\\
&=\Omega\left(n\log\left(\frac{m}{n}+1\right)\right)
\end{align*}
Thus the parallel algorithm \textal{Union} is work-efficient.
\qed
}

\para{Intersect and Difference.}
The functions \intersect$(T_1,T_2)$ and \difference$(T_1,T_2)$ take
the intersection and difference of the keys in their sets,
respectively.  The algorithms are similar to \union{} in that they use one tree to split the other.  However, the
method for joining is different.  For \intersect{}, \joinTwo{} is used
instead of \join{} if the root of the first \emph{is not} found in the
second.  For \difference{}, \joinTwo{} is used if
the root of the first \emph{is} found in the second.  The base cases are
also different in the obvious way.

\begin{theorem}
\label{thm:indiwork}
For all the four balance schemes mentioned in Section \ref{sec:paradigm}, the work and span of the algorithm (as shown in Figure \ref{fig:pseudocode}) of \intersect{} or \difference{} on two balanced BSTs of sizes $m$ and $n$ ($n\le m$) are $\displaystyle O\left(n\log\left(\frac{m}{n}+1\right)\right)$ and $O(\log n \log m)$ respectively (the bound is in expectation for treaps).
\end{theorem}

%% The algorithm first uses the root of one tree as the pivot to split the other tree, and recursively intersects the left and right part respectively, getting two trees $\Tl$ and $\Tr$. If the pivot is found in the other tree, it should appear in the return tree, so \join{} is called to join $\Tl$, $\Tr$ and the pivot. Otherwise \joinTwo{} should be called to join $\Tl$ and $\Tr$. The function \difference{} is similar. The only difference is that if the root appears in the other tree, it should be excluded.

%% It is easy to see that the work and depth of \intersect{} and \difference{} is the same as \union.

\para{Build.}
\build{} takes a unsorted array and returns a valid BST containing all
keys in that array.  The algorithm divides the full array into two
parts of equal length and recursively build two smaller trees in
parallel, and then unions the results.  %Figure~\ref{fig:pseudocode}
%lines~\ref{line:builds}--\ref{line:builde} shows the pseudocode for
%\build. Here \textal{Singleton} denotes a function to initialize a
%tree with a single node.

\begin{theorem}
The work and span of \build{} on an array of size $n$ is $O(n\log n)$ and $O(\log^3 n)$ respectively for the four balancing schemes mentioned in Section \ref{sec:paradigm}.
\end{theorem}
\fullin{
{\bf [Yihan: Are we using depth or span.]}
\proof
We use $W(n)$ and $D(n)$ to denote the work and depth to build a BST from an array of size $n$. From Theorem \ref{mergework} we know that the work and depth of \union{} in the last step is $O(n)$ and $O(\log^2 n)$ respectively. Thus we have:
\begin{align*}
W(n)&=2W(\frac{n}{2})+n\\
%W(1)&=O(1)\\
D(n)&=1+D(\frac{n}{2})+O(\log^2 n)\\
%D(1)&=O(1)
\end{align*}
Considering $W(1)=D(1)=O(1)$, solve the recursion formula we can get $W(n)=O(n\log n)$ and $D(n)=O(\log^3 n)$.
\qed}

\fullin{
Similarly, if the \textal{Union} with $O(\log m)$ depth is applied, the depth of \build{} could be reduced to $O(\log^2 n)$.

\begin{corollary}
The parallel algorithm \build{} is optimal for the four balancing schemes in terms of work.
\end{corollary}
}

\para{Other Functions.}
Many other functions can be implemented with \join{}.  Pseudocode for
\insertnew{} and \delete{} was given in the introduction.  For a tree
of size $n$ they both take $O(\log n)$ work.
Pseudocode for
\forallnew{}, \filter{}, and \range{} is given in
Figure~\ref{fig:pseudocode}.  The \forallnew{} function only works
with maps, and applies a function to each value of the map, returning
a map with the same keys and new values.  The \filter{} function
applies a Boolean function to each key (or key-value for maps),
returning a set (or map) containing just the elements for which the
function returns true.  The \range{} function extracts a range of keys
between given keys.  Several functions only search the tree and make
no new structure.  These include \func{Find}$(T,k)$, which checks if
$k$ is in $T$; \func{First}$(T)$ (\func{Last}$(T)$), which returns the
first (last) key in $T$; and \func{Previous}$(T,k)$
(\func{Next}$(T,k)$), which returns the first key less (greater) than
$k$ in $T$.  These function only need \expose.

If the size of the subtree is kept with each node (as done in our
library), then it is possible to efficiently implement several other
functions.  These include \func{SplitAt}$(T,i)$, which splits at the
$i^{th}$ position in $T$; \func{Select}$(T,i)$, which returns the
$i^{th}$ element of $T$, and \func{Rank}$(T,k)$; which returns the
position (rank) of the key $k$ in $T$.  These operations all take
O$(\log |T|)$ work using just \join{}, \expose{} and $|\cdot|$.

As mentioned in Section \ref{sec:paradigm}, \join{} can be used for
sequences as well as sets and maps (it is defined for any binary tree,
not just binary search trees).  For sequences it can support an
interface with operations such as append, insertAt and deteleAt
(insert or delete an element at the $i^{th}$ location) in $O(\log n)$
work.  This compares to $O(n)$ work that is required for an array
implementation.  In fact, \joinTwo{} is append, and \func{splitAt} can
easily be used with \join{} and \joinTwo{} to implement subSequence,
insertAt, and deleteAt. \filter{} and \forallnew{} also apply to
sequences with effectively the same code, and would be parallel.


==> pam__.tex <==
\section{Preliminaries}
\label{sec:prelim}
\para{Parallel Cost Model.} To analyze the asymptotic theoretical
cost we use the \emph{work-depth} model, where \emph{work} $W$  is the
total number of operations performed and \emph{depth} $D$ is the length of the critical
path. We can bound the total runtime in terms of work and depth since
any computation with $W$ work and $D$ depth will run in time
$T < \frac{W}{P} + D$ assuming a CREW PRAM
with $P$ processors and a greedy scheduler~\cite{Graham69,Brent74,BL98}.

\para{The Augmented Map.} The \emph{augmented map} \cite{ourppopp} is an ordered \emph{map} structure which supports a ``sum'' operation (the ``augmentation'') to keep track of the sum over the entries in the map. We denote this ``sum'' as the \emph{augmented value} of the map. More formally, an augmented map $\langle M_{K,V}, f, g\rangle$ is an ordered map $M$ where keys belong to some ordered set $K$, values belong to a set  $V$, and which is associated with two functions: the \emph{base function} $g:K\times V \mapsto A$ that converts a key-value pair into an augmented value ($\in$ set $A$) and the \emph{combine function} $f: A\times A \mapsto A$ that combines two augmented values. We require $f$ to be associative and that the following holds:\vspace{-0.5em}
\begin{equation}
f(a_1) = a_1, \hspace{0.5em} f(a_1, a_2, \dots, a_n) = f(f(a_1, a_2, \dots a_{n-1}), a_n)\vspace{-0.5em}
\end{equation}
In addition, we assume that $f$ has an identity $a_{\emptyset}$ (i.e., set $A$ with $f$ and $a_\emptyset$ forms a monoid).

In this paper, we refer to one key-value pair
in a map as an \emph{entry} and denote it as $e=(k,v)$ and use $k(e)$ and $v(e)$ to
extract the key and the value from an entry. The augmented value of a map reflects some property of the whole map related to both keys and values of all entries. More specifically, the augmented value of a map $M=(e_1, e_2, \dots, e_n)$ (denoted as $\mathcal{A}(M)$) can be calculated using the augmented base function $g$ and the augmented combine function $f$ as follows:\vspace{-0.5em}
\begin{equation}
\mathcal{A}(M) = f(g(e_1), g(e_2), \dots, g(e_n))\vspace{-0.1em}
\end{equation}


%The augmented value of a set is unique because of the total order of $K$ and the associativity of $f$. Specifically, $\mathcal{A}(\emptyset)=a_{\emptyset}$ because $f$ has identity $a_{\emptyset}$.
%From the total order of $K$ and the associativity of $f$, we know the augmented value of a set is unique.
%Specifically, note that $f$ has identity $a_{\emptyset}$, we know the augmented value on an empty set $\mathcal{A}(\emptyset)=a_{\emptyset}$.

%In this paper, with clear context, we drop the subscript for simplicity.


Many computational geometry problems, as well as many other applications, can be adapted to the augmented map abstraction, so that solving them using PAM is as easy as properly defining the base and combine function. In this paper, we define an augmented map as:\vspace{0.1em}
\mapstructure{
{\small
\centering
\begin{tabular}{|r@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }l@{ }l|}
  \hline
  \textbf{AugMap} &=& \textbf{AM}&(& $\boldsymbol{K}$;\quad $\boldsymbol{V}$;\quad$\boldsymbol{\prec}: K\times K\mapsto\{T,F\}$;\quad $\boldsymbol{A}$; \quad$\boldsymbol{g}: K\times V \mapsto A$; \quad$\boldsymbol{f}:A\times A \mapsto A$; \quad $\boldsymbol{a_{\emptyset}}\in A$ &)\\
  \hline
\end{tabular}
}}\vspace{0.1em}

Here $K$, $V$ and $A$ represents the types of keys, values, and augmented values. $\prec$ defines the total order on $K$, and $g$, $f$ and $a_\emptyset$ are defined as above. The seven parameters define an augmented map.

To implement the augmented maps we use augmented balanced binary search trees. Entries are stored in tree nodes which are sorted by keys. Each node also keeps another attribute that is the \emph{augmented value} of the sub-map of the subtree rooted at $u$. 
%Usually the \emph{value} stores some extra information about \emph{the single tree node} in addition to \emph{key}, and the \emph{augmented value} reflects some property (like an abstract ``sum'') about \emph{the whole subtree}.
We denote $\lc{u}$ and $\rc{u}$ as the left and right child of a tree node $u$. Considering that the subtree rooted at $u$ consists of its left subtree, the entry at $u$ and its right subtree, the the augmented value of $u$ can be computed using the base and combine function as follows: $\mathcal{A}(u) = f(\mathcal{A}(\lc{u}), g(e(u)), \mathcal{A}(\rc{u}))$.
\\

The balanced binary search tree, as the underlying data structure, has many good properties such as well-studied efficient algorithms and being easy to parallelize. For example, lookup, insertion and deletion all require $O(\log n)$ time, and set functions like \texttt{union}, \texttt{intersection} and \texttt{difference} take sublinear work ($O(m\log (n/m))$, $n\ge m$) and logarithmic depth ($O(\log n \log m)$) \cite{ours}. Constructing a tree holding $n$ elements costs $O(n\log n)$ work and $O(\log n)$ depth. Theoretically these are all asymptotically optimal in terms of work.

In the rest of the paper we directly use the interfaces and properties introduced in this section and show solutions to range queries and segment queries on top of the framework.

\para{Persistence.} A persistent data structure \cite{driscoll1986making} is a data structure that preserves the previous version of itself when it is modified and always yields a new updated structure. For tree structures persistence is often achieved by path copying, meaning that only the path affected by an update is copied, such that the asymptotical cost remains unchanged. Nodes are largely shared across different versions of trees, making implementations space-efficient. In this paper we assume underlying persistent data structures, which is essential in guaranteeing the efficiency both in space and time. For our experiments we use the PAM library which supports persistence for all its tree structures~\cite{ourppopp}.

\hide{
\subsection{The Parallel Augmented Map Library}
In this paper, to implement the applications using the augmented map abstraction, we the Parallel Augmented Map Library \cite{ourppopp}. This library supplies very simple and practical interfaces for augmented maps, which are efficient, parallel and persistent. This library uses augmented binary search trees as underlying data structure. Entries are stored in tree nodes, sorted by keys. Besides keys and values, each node also keeps another attribute that is the \emph{augmented value} of the sub-map in the subtree rooted at $u$. Usually the \emph{value} stores some extra information about \emph{the single tree node} in addition to \emph{key}, and the \emph{augmented value} reflects some property (usually an abstract ``sum'') about  \emph{the whole subtree}
%, related to both the keys and values of the entries in the tree.
We denote $\lc{u}$ and $\rc{u}$ as the left and right child of a tree node $u$. Considering the subtree rooted at $u$ consists of its left subtree, the entry stored in $u$ and its right subtree, then the augmented value of $u$ can be computed using the base function and combine function as:\vspace{-.4em}
$$\mathcal{A}(u) = f(\mathcal{A}(\lc{u}), g(k(u),v(u)), \mathcal{A}(\rc{u}))\vspace{-.9em}$$
because of the associativity of function $f$.

In the PAM library, all the functions are work-efficient, which means that they are optimal in parallel work and is also optimal when run sequentially. This is essential in guaranteeing the efficiency of our implementations on geometry applications. For example, set functions like \texttt{union} and \texttt{diff} have sublinear work ($O(m\log (n/m))$ on two sets of maps $m$ and $n\ge m$) and logarithmic depth ($O(\log n \log m)$). Some functions used in this paper along with their sequential and parallel costs are listed in Appendix \ref{app:pam} Table \ref{tab:costs}.

The PAM library supports data persistent, which means that any update to a data structure creates a new version, without affecting the old version. This is done by path copying, meaning that only the affected path related to the update is copied, such that the functions are still asymptotically efficient. Tree nodes are largely shared across different versions of trees, making implementations space-efficient. For example, the insert function copies the path from the root to where the key should be inserted to. Only $O(\log n)$ extra space is costed. This is crucial in guaranteeing the efficiency and correctness of many applications mentioned in this paper.

More information about the PAM library and is C++ interface can be found in Appendix \ref{app:pam}. In the rest of the paper we will directly use the interfaces and properties introduced in this section and show solutions to range queries and segment queries on top of the library.

\hide{From the ordered property of the tree structure and the associative of $f$, we know that the augmented value at a tree node $u$ can be calculated from the augmented values of its two subtrees and the entry of the node itself:
$\mathcal{A}(u) = f(\mathcal{A}(\lc{u}), g(k(u),v(u)), \mathcal{A}(\rc{u}))$.}


\hide{An augmented map \texttt{augmented\_map<K,V,Aug>} is defined using C++ templates specifying the key type, value type and the necessary information about the augmented values. The interface of PAM can be summarized as follows:
\begin{itemize}\setlength\itemsep{-.15em}\vspace{-.25em}
\item \texttt{\textbf{K}} - The key type, which must support a comparison function($<$) that defines a total order over its elements.
\item \texttt{\textbf{V}} - The value type.
\item \texttt{\textbf{Aug}} - The augmentation type. It is a struct containing the following attributes and methods:
\begin{itemize}\setlength\itemsep{-.20em}\vspace{-.5em}
\item \texttt{Typename \textbf{aug\_t}} that is the augmented value type $A$.
\item Static method \texttt{\textbf{base}(K, V)} that defines the augmented base function $g : K \times V \mapsto A$.
\item Static method \texttt{\textbf{combine}(aug\_t, aug\_t)} that defines the augmented combine function $f : A \times A \mapsto A$.
\item Static method \texttt{\textbf{identity}()} that returns $a_{\emptyset}$.
\end{itemize}
\end{itemize}
}
}
\hide{
\subsection{Sweepline Algorithms}
A sweep line algorithm (or plane sweep algorithm) is an algorithmic paradigm that uses a conceptual sweep line to process elements in order in Euclidean space. It uses a virtual line (often a vertical line) sweeping across the plane, stopping at some points to make updates to some data structure. Usually the positions that the sweep line stops are determined by the input data, e.g., the points or endpoints of segments. We call them the \emph{event points}. In many sweepline algorithms, especially the two mentioned in this paper, a special data structure is maintained corresponding to the event points, in order to track some information from the beginning up to this event point.

In this paper, we propose sweepline algorithms dealing with the range query and the segment query respectively. We also provide parallel version of these algorithms with reasonable parallel depth.
} 


==> paradigm.tex <==
\section{The JOIN Function}
\label{sec:paradigm}
Here we describe algorithms for \join{} for the four balancing schemes
we defined in Section~\ref{sec:prelim}.  We use a generalized version
of \join{} that works for any binary tree, whether a BST or not.  The
function \join$(\Tl,k,\Tr)$ for binary trees, takes two binary trees
$\Tl$ and $\Tr$, and a value $k$, and returns a new binary tree for
which the in-order values are a concatenation of the in-order values
of $\Tl$, then $k$, and then the in-order values of $\Tr$.  If the
binary trees are BSTs, then this is the same as the definition in the
introduction.  However, binary trees can also be used to represent
sequences, and \join{} might be useful for sequences.

%is useful in this context as describe at the end of Section~\ref{sec:??}.

As mentioned in the introduction, \join{} fully captures what is
required to rebalance a tree and can be used as the only function that
knows about and maintains the balance invariants.  For AVL, RB and WB
trees we show that \join{} takes work that is proportional to the
difference in rank of the two trees.  For treaps the work depends on
the priority of $k$.  All versions of \join{} are sequential so the
span is equal to the work.  We show in the next section that all
balancing schemes we consider lead to optimal work algorithms for many
other functions on maps and sets.  Due to space limitations, we
describe the algorithms, state the theorems for all balancing schemes,
but only show pseudocode and a proof (outline) for AVL trees.

\begin{figure}
\small
\begin{lstlisting}[frame=lines]
joinRight$(\Tl,k,\Tr)$ =
  $(l,k',c)$ = expose$(\Tl)$;
  if $h(c) \leq h(\Tr) + 1$ then @\label{line:avlbase}@
    $T' = \node(c,k,\Tr)$; @\label{line:avlnew}@
    if $h(T') \leq h(l) + 1$ then $\node(l ,k', T')$
    else rotateLeft($\node$($l, k',$ rotateRight$(T')$)) @\label{line:avldouble}@
  else
    $T'$ = joinRight$(c,k,\Tr)$;
    $T''$ = $\node(l, k',T')$;
    if $h(T') \leq h(l) + 1$ then $T''$
    else rotateLeft$(T'')$@\vspace{.1in}@ @\label{line:avlup}@
join$(\Tl,k,\Tr)$ =
  if $h(\Tl) > h(\Tr) + 1$ then joinRight$(\Tl,k,\Tr)$ @\label{line:avljoinright}@
  else if $h(\Tr) > h(\Tl) + 1$ then joinLeft$(\Tl,k,\Tr)$
  else $\node(\Tl,k,\Tr)$
\end{lstlisting}
\caption{AVL \join{} algorithm.}
\label{fig:avljoin}
\end{figure}

\begin{figure}
\small
\begin{lstlisting}[frame=lines]
joinRightRB$(\Tl,k,\Tr)$ =
  if ($r(\Tl) = \lfloor r(\Tr)/2 \rfloor\times 2$) then
    $\node(\Tl,\left<k,\texttt{red}\right>,\Tr)$;
  else
    $(L',\left<k',c'\right>,R')$=expose($\Tl$);
    $T'$ = $\node(L', \left<k',c'\right>$,joinRightRB$(R',k,\Tr))$;
    if ($c'$=black) and ($c(R(T'))=c(R(R(T')))$=red) then
      $c(R(R(T')))$=black;
      $T''$=rotateLeft$(T')$
    else $T''$@\vspace{.1in}@
joinRB$(\Tl,k,\Tr)$ =
  if $\lfloor r(\Tl)/2 \rfloor > \lfloor r(\Tr)/2 \rfloor$ then
    $T'=$joinRightRB$(\Tl,k,\Tr)$;
    if ($c(T')$=red) and ($c(R(T'))$=red) then
      $\node(L(T'),\left<k(T'),\texttt{black}\right>,R(T'))$
    else $T'$
  else if $\lfloor r(\Tr)/2 \rfloor > \lfloor r(\Tl)/2 \rfloor$ then
    $T'=$joinLeftRB$(\Tl,k,\Tr)$;
    if ($c(T')$=red) and ($c(L(T'))$=red) then
      $\node(L(T'),\left<k(T'),\texttt{black}\right>,R(T'))$
    else $T'$
  else if ($c(\Tl)$=black) and ($c(\Tr)$=black) then
    $\node(\Tl,\left<k,\texttt{red}\right>,\Tr)$
  else $\node(\Tl,\left<k,\texttt{black}\right>,\Tr)$
\end{lstlisting}
\caption{RB \join{} algorithm.}
\label{fig:rbjoin2}
\end{figure}

\begin{figure}
\small
\begin{lstlisting}[frame=lines]
joinRightWB$(\Tl,k,\Tr)$ =
  ($l,k',c$)=expose($\Tl$);
  if (balance($|\Tl|,|\Tr|$) then $\node(\Tl,k,\Tr))$;
  else
    $T'$ = joinRightWB$(c,k,\Tr)$;
    $(l_1,k_1,r_1)$ = expose$(T')$;
    if balance$(|l|,|T'|)$ then $\node$($l, k', T'$)
    else if (like$(|l|,|l_1|)$) and (like$(|l|+|l_1|,r_1)$) then
      rotateLeft($\node$($l, k', T'$))
    else rotateLeft($\node$($l,k'$,rotateRight$(T')$))@\vspace{.1in}@
joinWB$(\Tl,k,\Tr)$ =
  if heavy($\Tl, \Tr$) then joinRightWB$(\Tl,k,\Tr)$
  else if heavy($\Tr,\Tl$) then joinLeftWB$(\Tl,k,\Tr)$
  else $\node(\Tl,k,\Tr)$
\end{lstlisting}
\caption{WB \join{} algorithm.}
\label{fig:wbjoin}
\end{figure}

\begin{figure}
\small
\begin{lstlisting}[frame=lines]
joinTreap$(\Tl,k,\Tr)$ =
  ($l_1,k_1,r_1$)=expose($\Tl$);
  ($l_2,k_2,r_2$)=expose($\Tr$);
  if prior($k_1, k$) and prior($k_1,k_2$) then
    $\node$($l_1,k_1$,joinTreap$(r_1,k,\Tr)$)
  else if prior($k_2,k$) and prior($k_2$,$k_1$) then
    $\node$(joinTreap($\Tl,k,l_2$),$k_2,r_2$)
  else $\node(\Tl,k,\Tr)$
\end{lstlisting}
\caption{Treap \join{} algorithm.}
\label{fig:treapjoin}
\end{figure}

\para{AVL trees.}
Pseudocode for AVL \join{} is given in Figure~\ref{fig:avljoin} and
illustrated in Figure~\ref{avlrebalance}.  Every node stores its own
height so that $h(\cdot)$ takes constant time.  If the two trees $\Tl$
and $\Tr$ differ by height at most one, \join{} can simply create a
new \node$(\Tl,k,\Tr)$.  However if they differ by more than one then
rebalancing is required.  Suppose that $h(\Tl) > h(\Tr) + 1$ (the
other case is symmetric).  The idea is to follow the right spine of
$\Tl$ until a node $c$ for which $h(c) \leq h(\Tr) + 1$ is found
(line~\ref{line:avlbase}).  At this point a new $\node(c,k,\Tr)$ is
created to replace $c$ (line~\ref{line:avlnew}).  Since either $h(c) =
h(\Tr)$ or $h(c) = h(\Tr) + 1$, the new node satisfies the AVL
invariant, and its height is one greater than $c$.  The increase in
height can increase the height of its ancestors, possibly invalidating
the AVL invariant of those nodes.  This can be fixed either with a
double rotation if invalid at the parent (line~\ref{line:avldouble})
or a single left rotation if invalid higher in the tree
(line~\ref{line:avlup}), in both cases restoring the height for any
further ancestor nodes.  The algorithm will therefore require at most
two rotations.

\begin{figure*}[t!h!]
\centering
  \includegraphics[width=1.9\columnwidth]{figures/AVL.pdf}\\
  \caption{An example for \join{} on AVL trees ($h(\Tl) > h(\Tr)+1$).
    We first follow the right spine of $\Tl$ until a subtree of height at most $h(T_r) +
    1$ is found (i.e., $T_2$ rooted at $c$).  Then a new \node$(c,k,\Tr)$
    is created, replacing $c$ (Step 1).    If $h(T_1) = h$ and $h(T_2)
    = h + 1$, the node $p$ will no longer satisfy the AVL invariant.
    A double rotation (Step 2) restores both balance and
    its original height.}
\label{avlrebalance}
\end{figure*}

\begin{lemma}
\label{lem:AVL}
For two AVL trees $\Tl$ and $\Tr$, the AVL \join{} algorithm works
correctly, runs with $O(|h(\Tl)-h(\Tr)|)$ work, and returns a
tree satisfying the AVL invariant with height at most
$1 +\max(h(\Tl),h(\Tr))$.
\end{lemma}

\proofoutline{} Since the algorithm only visits nodes on the path from
the root to $c$, and only requires at most two rotations, it does work
proportional to the path length.   The path length
is no more than the difference in height of the two trees since
the height of each consecutive node along the left spine of $\Tr$
differs by at least one.  Along with the case when
$h(\Tr) > h(\Tl) + 1$, which is symmetric, this gives the stated work
bounds.  The resulting tree satisfies the AVL
invariants since rotations are used to restore the invariant (details
left out).    The height of any node can increase by at most
one, so the height of the whole tree can increase by at most one.
\qed

\fullin{
\proof
For symmetry, here we only prove the case when $h(\Tl)>h(\Tr)$. In our algorithm, we will first go right down to a proper level then apply rebalance along the path upwards. We first prove that after applying rebalance at some node $v$, $v$ will be AVL-balanced, and the height of the subtree rooted at $v$ will increase at most $1$. Recall that we denote the node that we stop going down in $\Tl$ as $c$, its parent as $p$, and $p$'s parent as $g$. Suppose $h(\Tr)=h$. We prove this theorem by induction.

As shown in Fig. \ref{avlrebalance}, after appending $\Tr$ to $\Tl$ by the intermediate key $k$, $k$ is guaranteed to be balanced, and the subtree rooted at $k$ has a height of $h+1$. We discuss the three possible scenarios based on the height of $p$' left tree (i.e., $T_1$ rooted at $a$ as shown in Fig. \ref{avlrebalance}), i.e., $h-1$, $h$ and $h+1$. The only case that an unbalance will occur at $p$ is when the height of the left child of $p$ is $h-1$. We apply a left rotation here and the subtree originally rooted at $p$ is now rooted at $k$, and is now balanced. The whole subtree height is now $h+2$ instead of original $h+1$. If $p$'s left child has a height of $h$, the height of the original subtree is $h+1$. In this case, $p$ is now balanced, and the height is currently $h+2$. If the height of the left child of $p$ is $h+1$, $p$ is also naturally balanced, and the height of $p$ does not increase. Thus in all three scenarios the proposition holds at the very first linking of $\Tl$ and $\Tr$. If we have reached the root, the rebalance stops and the current tree is a valid AVL. Otherwise we call rebalance for $p$'s parent.

When we reach some interior nodes $v$, $v$ is originally balanced, and the height of the right child (denoted as $u$) of $v$ increases by at most $1$. If $v$ is still balanced, the whole height of $v$ is increased by at most $1$. Suppose originally the height of the right child of $v$ is $h$. The only case that $v$ is now unbalanced is when $v$'s left child's height is $h-1$, and the current height of $v$'s right child (i.e., $u$) is $h+1$. Similar as stated above, based on the height of $u$'s left child ($h_L$) and right child ($h_R$), we apply the following rotations:
\begin{center}
\begin{tabular}{c|c|c|c|c}
  \hline
  \multirow{2}{*}{$h_L$} & \multirow{2}{*}{$h_R$} & \multirow{2}{*}{Operation} & Original & Final\\
  &&&Height & Height\\
  \hline
  $h$ & $h$ &  Left rotation & $h+1$ & $h+2$\\
  \hline
  \multirow{2}{*}{$h$} & \multirow{2}{*}{$h-1$} & Right rotation  & \multirow{2}{*}{$h+1$} & \multirow{2}{*}{$h+1$} \\
  &&then left rotation&\\
  \hline
  $h-1$ & $h$ & Left rotation & $h+1$ & $h+1$ \\
  \hline
\end{tabular}
\end{center}
In each case the subtree originally at $v$ will be balanced and the height will increase by at most $1$. If we have reached the root, the rebalance stops and the current tree is a valid AVL. Otherwise we call rebalance for $v$'s parent.

As the process will guarantee that current node to be rebalanced will go up one level, we finally will reach the root and end rebalance process, hence get a valid AVL.
\qed
}

\para{Red-black Trees.}
Tarjan describes how to implement the \join{} function for red-black
trees~ \cite{Tarjan83}.  Here we describe a variant that does not
assume the roots are black.  We store at every node its black height
$\bh(\cdot)$.  The first case is when $\bh(\Tr)=\bh(\Tl)$.  Then if
both $k(\Tr)$ and $k(\Tl)$ are black, we create red
$\node(\Tl,k,\Tr)$, otherwise we create black $\node(\Tl,k,\Tr)$.  The
second case is when $\bh(\Tr)<\bh(\Tl)=\bh$ (the third case is symmetric).
Similarly to AVL trees, \join{} follows the right spine of $\Tl$ until
it finds a black node $c$ for which $\bh(c) = \bh(\Tr)$.  It then
creates a new red \node$(c,k,\Tr)$ to replace $c$. Since both $c$
and $\Tr$ have the same height, the only invariant that can be
violated is the red rule on the root of $\Tr$, the new node, and its
parent, which can all be red.  In the worst case we may have three red
nodes in a row.  This is fixed by a single left rotation: if a black
node $v$ has $R(v)$ and $R(R(v))$ both red, we turn $R(R(v))$ black
and perform a single left rotation on $v$. %turning the new node black, and then performing a single left rotation on $v$.
The update is
illustrated in Figure~\ref{rbrebalance}.  The rotation, however can
again violate the red rule between the root of the rotated tree and
its parent, requiring another rotation.
% but expect the bottommost level, a triple-red issue does not happen.
The double-red issue might
proceed up to the root of $\Tl$. If the original root of $\Tl$ is red,
the algorithm may end up with a red root with a red child, in which
case the root will be turned black, turning $\Tl$ rank from $2\bh+1$
to $2\bh+2$.  If the original root of $\Tl$ is black, the algorithm
may end up with a red root with two black children, turning the rank
of $\Tl$ from $2\bh$ to $2\bh+1$.  In both cases the rank of the
result tree is at most $1+r(\Tl)$.

\hide{Similarly to AVL trees, the algorithm
follows the right spine of $\Tl$ until it finds a black node $c$ for
which $\bh(c) = \bh(\Tr)$.  It then creates a new red \node$(c,k,\Tr)$
to replace $c$.  Since both $c$ and $\Tr$ are black and have the same
height, the only invariant that can be violated is the red rule
between the new node and its parent, which can be red.  This is fixed
by turning the new node black, and then performing a single left
rotation on its grandparent to restore the black rule.  The update is
illustrated in Figure~\ref{rbrebalance}.  The rotation, however can
again violate the red rule between the root of the rotated tree and
its parent, requiring another rotation.  This
might proceed up to the root of $\Tl$, which is turned black if red,
therefore possibly incrementing the overall black height by one.
}

\begin{lemma}
\label{lem:RB}
For two red-black trees $\Tl$ and $\Tr$, the RB \join{} algorithm works
correctly, runs with $O(|r(\Tl)-r(\Tr)|)$ work, and
returns a tree satisfying the red-black invariants and with rank
at most $1+\max(r(\Tl),r(\Tr))$.
\end{lemma}

The proof is similar as Lemma \ref{lem:AVL}.
\hide{
\proofoutline{} Since the algorithm only visits nodes on the path from
the root to $c$, and only requires at most a single rotation per node
on the path, the overall work for the algorithm is proportional to the
depth of $c$ in $\Tr$.  This in turn is no more than twice the
difference in black height of the two trees since the black height
decrements at least every two nodes along the path.  Along with the
case when $\bh(\Tr) > \bh(\Tl)$, which is true by symmetry, this gives the stated
work bounds.  The algorithm returns a tree that satisfies the
RB invariants since rotations are used to restore the invariant on
every visited node. \qed}

\fullin{
\proof
For symmetry, here we only prove the case when $h(\Tl)>h(\Tr)$. We prove the proposition by induction.

As shown in Fig. \ref{rbrebalance}, after appending $\Tr$ to $\Tl$, if $p$ is black, the rebalance has been done, the height of each node stays unchanged. Thus the RB tree is still valid. Otherwise, $p$ is red, $p$'s parent $g$ must be black. By applying a left rotation on $p$ and $g$, we get a balanced RB tree rooted at $p$, except the root $p$ is red. If $p$ is the root of the whole tree, we change $p$'s color to black, and the height of the whole tree increases by 1. The RB tree is still valid. Otherwise, if the current parent of $p$ (originally $g$'s parent) is black, the rebalance is done here. Otherwise a similar rebalance is required on $p$ and its current parent. Thus finally we will either find the current node valid (current red node has a black parent), or reach the root, and change the color of root to be black. Thus when we stop, we will always get a valid RB tree. And the black height of the whole tree will increase by at most 1.
\qed
}

\begin{figure}[t!h!]
\centering
  \includegraphics[width=1.0\columnwidth]{figures/RB.pdf}\\
  \caption{An example of \join{} on red-black trees ($\bh=\bh(\Tl) >
    \bh(\Tr)$).  We follow the right spine of $\Tl$ until we find a
    black node with the same black height as $\Tr$ (i.e., $c$).  Then
    a new red \node$(c, k, \Tr)$ is created, replacing $c$ (Step 1).
    The only invariant that can be violated is when either $c$'s
    previous parent $p$ or $\Tr$'s root $d$ is red.  If so, a left
    rotation is performed at some black node. Step 2 shows the
    rebalance when $p$ is red. The black height of the rotated subtree
    (now rooted at $p$) is the same as before ($h+1$), but the parent
    of $p$ might be red, requiring another rotation.  If the red-rule
    violation propagates to the root, the root is either colored red,
    or rotated left (Step 3).}
\label{rbrebalance}
\end{figure}



\para{Weight Balanced Trees.}
We store the weight of each subtree at every node.  The algorithm for
joining two weight-balanced trees is similar to that of AVL trees and
red-black trees.  If $\Tl$ and $\Tr$ have like weights the algorithm
returns a new \node$(\Tl,k,\Tr)$.  Suppose $|\Tr|\le|\Tl|$, the
algorithm follows the right branch of $\Tl$ until it reaches a node
$c$ with like weight to $\Tr$.  It then creates a new
$\node(c,k,\Tr)$ replacing $c$.  The new node will have weight
greater than $c$ and therefore could imbalance the weight of $c$'s
ancestors.  This can be fixed with a single or double
rotation (as shown in Figure~\ref{wbtree1}) at each node assuming
$\alpha$ is within the bounds given in Section~\ref{sec:prelim}.
\begin{figure}[!t!h]
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=0.95\columnwidth]{figures/WB.pdf}\\
  \caption{An illustration of single and double rotations possibly
    needed to rebalance weight-balanced trees.   In the figure the
    subtree rooted at $u$ has become heavier due to joining in $\Tl$ and its
    parent $v$ now violates the balance invariant.}
\label{wbtree1}
\end{figure}

\begin{lemma}
\label{lem:wbvalid}
For two $\alpha$ weight-balanced trees $\Tl$ and $\Tr$ and
$\alpha <1-\frac{1}{\sqrt{2}}\approx 0.29$, the weight-balanced
\join{} algorithm works correctly, runs with $O(|\log(w(\Tl)/w(\Tr))|)$ work, and returns a tree satisfying the $\alpha$ weight-balance invariant and with rank
at most $1+\max(r(\Tl),r(\Tr))$..
\end{lemma}

The proof is intuitively similar as the proof stated in \cite{weightbalanced,blum1980average}, which proved that when $\frac{2}{11}\le \alpha \le 1-\frac{1}{\sqrt{2}}$, the rotation will rebalance the tree after one single insertion. In fact, in our \join{} algorithm, the ``inserted'' subtree must be along the left or right spine, which makes the analysis much easier.
%of the leaf weight is increased to at most twice of its original weight. In our version, the weight of one subtree (in fact, the subtree must be along the left or right spine, which makes the analysis much easier) will be increased to at most $\frac{1}{\alpha}$ times of its original weight. Using similar proof as in \cite{weightbalanced,blum1980average}, the rotation still works.

\fullin{
\proof
Recall that in a weight balanced tree, for a certain node, neither of its child is $\beta$ times larger than the other one. W.L.O.G, we prove the case when the $|\Tl|<|\Tr|$, where $\Tl$ is inserted along the left branch of $\Tr$. Then we rebalance the tree from the point of key $k$ and go upwards. As shown in Fig. \ref{wbtree1} (0), suppose the rebalance has been proceed to $u$. Thus the subtree rooted at $u$ is balanced, and $\Tl$ is part of it. We name the four trees from left to right as $A,B,C$ and $D$, and the number of nodes in them as $a,b,c$ and $d$. From the balance condition we know that $A$ is balanced to $B+C$, and $B$ is balanced to $C$, i.e.:
\begin{align}
\label{b+ctoa}
\frac{1}{\beta}(b+c)<&a<\beta (b+c)\\
\label{btoc}
\frac{1}{\beta}b<&c<\beta c
\end{align}
We claim that at lease one of the two operations will rebalanced the tree rooted at $v$:
\begin{enumerate}[Op. (1).]
  \item Single rotate: right rotate at $u$ and $v$ (as shown in Fig. \ref{wbtree1} (1)).
  \item double rotate: Left rotate then right rotate (as shown in Fig. \ref{wbtree1} (2)).
\end{enumerate}

Also, notice that the unbalance is caused by the insertion of a subtree at the left-most branch. Suppose the size of the smaller tree is $x$, and the size of the original left child of $v$ is $y$. Note that in the process of \texttt{join}, we didn't append the smaller tree at $v$'s parent, instead, we went down for further nodes. Also, note that the original subtree of size $y$ is weight balanced with $D$. This means we have:

\begin{align}
x&<\frac{1}{\beta}(d+y)\\
\frac{1}{\beta} d &< y<\beta d\\
x+y&=a+b+c
\end{align}

From the above three inequalities we get $x\le \frac{1}{\beta}d+d$, thus:
\begin{equation}
\label{a+b+csmallerd}
a+b+c=x+y<(1+\beta+\frac{1}{\beta})d
\end{equation}

Since a unbalance occurs, we have:
\begin{equation}
\label{a+b+clargerd}
a+b+c>\beta d
\end{equation}

We discuss the following 3 cases:

\begin{enumerate}
  \item $B+C$ is weight balanced with $D$.

  In this case, we apply a right rotate. The new tree rooted at $u$ is now balanced. $A$ is naturally balanced. Now we prove that $A$ is balanced with $B+C+D$.

  First, $b+c>\betaone a$, so $b+c+d>\betaone a$.

  Then we discuss in two cases:

  \begin{enumerate}[1).]
  \item If $\beta d >a+b+c$. In this case, $D$ is balanced to $A+B+C$, $B+C$ is balanced to $D$.
  \hide{If $b+c<(\beta-1)d$. We have:
  \begin{align}
  \beta a &>\beta(\beta d-b-c)\\
  &({\rm{applying (\ref{a+b+clargerd})}})\\
  &=\beta^2 d-\beta b-\beta c -b-c-d+b+c+d\\
  &=(\beta+1)(\beta-1)d-(\beta+1)(b+c)+b+c+d\\
  &=(\beta+1)((\beta-1)d-(b+c))+b+c+d\\
  &>b+c+d
  \end{align}}
  Thus one right rotation will rebalance the tree rooted at $v$.

  \item If $\beta d<a+b+c$. In this case, we apply the double rotation, which is one right rotation followed by a left rotation. Now we need to prove the balance of all the subtrees.
  When $\beta d<a+b+c$, we have:
  \begin{align}
  &\beta d <a+b+c<\betaone(b+c+d)+b+c\\
  \Rightarrow &(\beta-\betaone)d<(\betaone+1)(b+c)\\
  \Rightarrow &(\beta-1)d<b+c
  \end{align}
  , i.e., $(\beta-1)d<b+c<\beta d$, so:
  \begin{align}
  \label{btod}
  b>\frac{1}{\beta+1}(b+c)>\frac{\beta-1}{\beta+1}d\\
  \label{ctod}
  c>\frac{1}{\beta+1}(b+c)>\frac{\beta-1}{\beta+1}d
  \end{align}

  We discuss the following three conditions of subtrees' balance:
  \begin{enumerate}[I.]
    \item \textbf{$A$ is weight balanced to $B$}.
    \begin{enumerate}[i.]
    \item $\bm{b<\beta a}$. Since $\beta a>b+c$, we have $\beta a>b$.

    \item $\bm{a<\beta b}$. When $\beta>1+\sqrt{2}\approx 2.414$, we have $\frac{\beta+1}{\beta-1}<\beta$.
    \begin{align}
    a&<\frac{1}{\beta}(b+c+d)\\
    &<\betaone(b+\beta b +\frac{\beta+1}{\beta-1}b)\\
    &\apply{\ref{btod}}\\
    &<\frac{\beta+1}{\beta-1}b\\
    &<\beta b
    \end{align}
    \end{enumerate}
    \item \textbf{$C$ is weight balanced to $D$}.
    \begin{enumerate}
    \item $\bm{c<\beta d}$. Since $b+c<\beta d$, we have $c<\beta d$.

    \item $\bm{d<\beta c}$. From (\ref{ctod}), we know that when $\beta>1+\sqrt{2}$, $\frac{\beta+1}{\beta-1}<\beta$. Thus:
    \begin{align}
    d<\frac{\beta+1}{\beta-1}c<\beta c
    \end{align}
    \end{enumerate}
    \item \textbf{$A+B$ is weight balanced to $C+D$}.
    \begin{enumerate}[i.]
    \item $\bm{a+b<\beta (c+d)}$.
    Note that when $\beta>1+\sqrt{2}\approx 2.414$, we have $\frac{\beta+1}{\beta-1}<\beta$. Thus:
    \begin{align}
    \nonumber
    &d<\frac{1}{\beta-1}(b+c)<\frac{1}{\beta-1}(\beta c+c)\\
    &=\frac{\beta+1}{\beta-1}c<\beta c\\
    \Rightarrow&\betaone d< c\\
    \Rightarrow&(1+\betaone)d<(1+\beta)c\\
    \Rightarrow&(1+\betaone+\beta)d<\beta(c+d)+c\\
    \Rightarrow& a+b+c<(1+\betaone+\beta)d<\beta(c+d)+c\\
    \Rightarrow& a+b<\beta(c+d)
    \end{align}
    \item $\bm{c+d<\beta (a+b)}$. When $\beta>2$, we have $\frac{\beta}{\beta-1}<\beta$. Thus:
    \begin{align}
    d<\frac{1}{\beta-1}(b+c)<\frac{\beta}{\beta-1}a<\beta a
    \end{align}
    Obviously we have $c<\beta b$. Thus $c+d<\beta (a+b)$.
    \end{enumerate}
  \end{enumerate}
  \end{enumerate}
  \item $B+C$ is too light that cannot be balanced with $D$.

  In this case, we have $a<\beta (b+c)<d$, which means that $a+b+c<d+\betaone d < \beta d$ when $\beta>\frac{1+\sqrt{5}}{2}\approx 1.618$. This contradicts with the condition that $A+B+C$ is too heavy to $D$ ($a+b+c>\beta d$). Thus this case is impossible.

  \item $B+C$ is too heavy that cannot be balanced with $D$, i.e.,
  \begin{align}
  &b+c>\beta d\\
  \label{alargerd}
  \Rightarrow &a>\betaone (b+c)>d
  \end{align}
  In this case, we apply a right rotation then a left one.

  We need to prove the following balance conditions:

  \begin{enumerate}[I.]
    \item \textbf{$A$ is weight balanced to $B$}.
    \begin{enumerate}[i.]
    \item $\bm{b<\beta a}$. Since $\beta a>b+c$, we have $\beta a>b$.
    \item $\bm{a<\beta b}$. Suppose $c=kb$, where $\betaone<k<\beta$. Since $b+c>\beta d$, we have:
    \begin{equation}
    \label{dtob}
    d<\frac{1+k}{\beta}b
    \end{equation}

    From the above inequalities, we have:
    \begin{align}
    a+b+c&=a+b+kb\\
     &<(1+\beta+\betaone)d \\
     & ({\rm{applying (\ref{a+b+csmallerd}}}))\\
     &<(1+\beta+\betaone)\times \frac{1+k}{\beta}b\\
     & ({\rm{applying (\ref{dtob}}}))\\
    \Rightarrow a&< \left(\frac{1+\beta+\betaone}{\beta}-1\right)(1+k)b\\
    &=\frac{\beta+1}{\beta}(1+k)b\\
    &<\frac{(\beta+1)^2}{\beta^2}b
    \end{align}
    When $\beta> \frac{7}{9}\times (\frac{\sqrt{837}+47}{54})^{-1/3}+(\frac{\sqrt{837}+47}{54})^{1/3} + \frac{1}{3} \approx 2.1479$, we have $\frac{(\beta+1)^2}{\beta}<\beta$. Hence $a<\beta b$.
    \end{enumerate}
    \item \textbf{$C$ is weight balanced to $D$}.
    \begin{enumerate}[i.]
    \item $\bm{d<\beta c}$. When $\beta>\frac{1+\sqrt{5}}{2}\approx 1.618$, we have $\beta>1+\betaone$. Suppose $c<\betaone d$, we have $b<\beta c < d$. Thus:
    \begin{align}
    b+c<(1+\betaone)d<\beta d
    \end{align}
    , which contradicts with our assumption that $B+C$ is too heavy to be balanced with $D$.
    \item $\bm{c<\beta d}$. Plug (\ref{alargerd}) in (\ref{a+b+csmallerd}) and get $b+c<(\beta+\betaone)d$. Recall that $d>1$, we have:
    \begin{align}
    &\betaone c+c < b+c < (\beta+\betaone)d\\
    \Rightarrow& c<\frac{\beta^2+1}{\beta+1}d < \beta d
    \end{align}
    \end{enumerate}
    \item $A+B$ is weight balanced with $C+D$.
    \begin{enumerate}[i.]
    \item $\bm{c+d<\beta(a+b)}$. Obviously $c<\beta b$, also $d<a<\beta a$ (applying (\ref{alargerd})), thus $c+d<\beta(a+b)$.
    \item $\bm{a+b<\beta(c+d)}$. Recall when $\beta>\frac{1+\sqrt{5}}{2}\approx 1.618$, we have $\beta>1+\betaone$.
    \begin{align}
    &d<\betaone(b+c)<c+\betaone c <(1+\betaone)c<\beta c\\
    \Rightarrow&\betaone d< c\\
    \Rightarrow&(1+\betaone)d<(1+\beta)c\\
    \Rightarrow&(1+\betaone+\beta)d<\beta(c+d)+c\\
    \Rightarrow& a+b+c<(1+\betaone+\beta)d<\beta(c+d)+c\\
    \Rightarrow& a+b<\beta(c+d)
    \end{align}
    Taking all the three conclusions into consideration, the new subtree rooted at $v$ is weight-balanced.
    \end{enumerate}
  \end{enumerate}
\end{enumerate}
\qed
}

\begin{comment}
Notice that this upper bound is the same as the restriction on $\alpha$ to yield a valid weighted-balanced tree when inserting a single node.% to make the balance algorithm work when inserting a single node.
Then we can induce that when the rebalance process reaches the root, the new weight-balanced tree is valid.
\end{comment}

%Notice that the upper bound is the same as the restriction to guarantee the balance algorithm to work when inserting a single node. The proof of the theorem is shown in the Appendix.

\para{Treaps.}
The treap \join{} algorithm first creates the \node$(\Tl,k,\Tr)$,
and then as long as one of the children of $k$ has a higher priority
than $k$, rotates the tree around $k$ so the highest priority key is at
the root.  The cost of \join{} is therefore the depth of the key $k$
in the result tree (each rotation pushes it down one level).  In
treaps the shape of the result tree, and hence the depth of $k$, depends
only on the keys and priorities and not the history.  Specifically, if
a key has the $t^{th}$ highest priority among the keys, then its
expected depth in a treap is $O(\log t)$.  If it is the highest
priority, for example, then it remains at the root.

\begin{lemma}
\label{lem:treap}
For two treaps $\Tl$ and $\Tr$, if the priority of $k$ is the $t$-th
highest among all keys in $\Tl \cup \{k\} \cup \Tr$, the treap \join{}
algorithm works correctly, runs with $O(\log t+1)$ work 
in expectation, and returns a tree satisfying the treap 
invariant with rank at most $1 +\max(r(\Tl),r(\Tr))$.
\end{lemma}

From the above lemmas we can get the following fact for \join.

\begin{theorem}
\label{thm:main}
For AVL, RB and WB trees \join$(\Tl,k,\Tr)$ does $O(|r(\Tl)-r(\Tr)|)$
work. For treaps \join{} does $O(\log t)$ work in expectation if $k$ has the $t$-th 
highest priority among all keys.
For AVL, RB, WB trees and treaps, \join{} returns a tree $T$ for which the rank satisfies
$\max(r(\Tl),r(\Tr))\le r(T)\le 1+\max(r(\Tl),r(\Tr))$.
\end{theorem}

%This could be seen by the theorems and statements above.% For general height of RB tree, it is at most $2+\max(h(\Tl),h(\Tr))$.



==> prange.tex <==
\subsection{Prefix-Union Trees} 
\label{sec:prangeapp}
This data structure is a series of trees. Assume that all points in $P$ are sorted by the x-coordinate, which means $\forall i, j$ where $i<j$, we have $x_i\le x_j$. Then each point is assigned a BST $T_i$ storing all points $\{(x_j, y_j)|1\le j\le i\}$. This means that $T_i$ stores the ``prefix sum (union)'' of the points prior to it. We call $T_i$ \emph{prefix-union trees}. In these prefix-union trees, elements are organized by the key of y-coordinate, and the weight as value. If we define the reduction operation to be ``add'', then because of the augmenting property of the tree, the total weight of all points in a subtree can be returned in constant time given the pointer to the subtree root. To report the total weight of points in the box of $(x_L, x_R, y_L, y_R)$, we first binary search $x_L$ and $x_R$ in the sequence of $\{x_i\}$, which means to find $l$ and $r$ that satisfy $x_l<x_L\le x_{l+1}$ and $x_r\le x_R< x_{r+1}$. We can narrow the range of x-coordinate into $(x_L,x_R)$ by looking at only the points in $T_r-T_l$. Then the final answer is to report the sum of weight of all points within range of $(y_L,y_R)$ in $T_r-T_l$.
%$(T_r-T_l).$\texttt{range}$(y_L,y_R)=T_r.$\texttt{range}$(y_L,y_R)-T_l.$\texttt{range}$(y_L,y_R)$.

\emph{Tree Construction.} From a practical point of view, we do not calculate the prefix union one by one, which means to insert $(x_i, y_i)$ into $T_{i-1}$ to get $T_i$ because it lacks parallelism. Instead, after sorting all points by x-coordinate, we partition all points into $k$ blocks, each block having $t=\lfloor\frac{n}{k}\rfloor$ points. Points from $p_{(j-1)t}$ to $p_{jt-1}$ are in block $k$. We first build $k$ small trees $T'_{i}$ ($0\le i \le k$) corresponding to the $k$ blocks in parallel using \texttt{build\_fast}. This takes work $O(k\cdot \frac{n}{k}\log \frac{n}{k})=O(n\log \frac{n}{k})$ and depth $O(\log \frac{n}{k})$.

Next, we compute the prefix union among these $k$ small trees. These trees are the exact prefix-union trees of $T_{jt}$. This can be done sequentially using $T_{jt}=$\texttt{union}$(T_{(j-1)t}, T'_{j})$. Consider that the work of union is $O\left(m\log (\frac{n}{m}+1)\right)$, the total cost of this step is bounded by:
\begin{align*}
&c\sum_{i=1}^{k} t\log (\frac{it}{t} +1)\\
=&ct\sum_{i=1}^{k} \log (i+1)\\
=&O(n\log k)
\end{align*}
, where $c$ represents the constant hidden by big-O. The depth is:
\begin{align}
&\sum_{i=1}^{k}\log t \log it\\
=&\log t\cdot \left(k\log t+\sum_{i=1}^{k}\log i\right)\\
=&k\log \frac{n}{k}\left(\log \frac{n}{k}+\log k\right)\\
=&O(k\log \frac{n}{k}\log n)
\end{align}
%$O(k\log \frac{n}{k}\log n)$.

In the final step we build all the other prefix-union trees based on the above-built $T_{jt}$ in the corresponding blocks. All the $k$ blocks can be done in parallel. In each block, the points $p_i$ are inserted in order sequentially into its previous tree $T_{i-1}$. The total work is bounded by:
\begin{align*}
c'\sum_{i=1}^{n} \log i=O(n\log n)
\end{align*}
, where $c'$ represents the constant hidden by big-O. The depth can be reduced to $O(\frac{n}{k}\log n)$.

In total, this process costs work $O(n\log n)$ and depth $O(k\log^n+\frac{n}{k}\log n)$. When $k=\Theta(\sqrt{\frac{n}{\log n}})$, the depth is $O(\sqrt{n}\log^{1.5}n)$.

In practice, we set $k=O(p)$ where $p$ is the number of available cores.

\emph{Answering Queries.} With the prefix-union tree constructed, we can answer a query in $O(\log n)$ time. We first see how to return the total weight of all nodes in a certain range $(y_L,y_R)$ of y-coordinate in a single prefix-union tree. This is the same as in 1D range tree: we search $y_L$ and $y_R$ in the tree until we get a node $v_{\tiny\mbox{split}}$ that $y_L$ and $y_R$ go to different subtrees; then we continue to search $y_L$ in the left subtree, and if we go left, report the sum (the \texttt{accumulation} field) of weights in the right subtree. Similarly we continue to search $y_R$ in the right subtree, and report the accumulation in the left tree when we go right. %We call this process \texttt{reportRange}$(y_L,y_R)$.

As for prefix-union trees, the query an be answered by simply binary search $x_L$ and $x_R$ in the sequence of $\{x_i\}$, which means to find $l$ and $r$ that $x_l<x_L\le x_{l+1}$ and $x_r\le x_R< x_{r+1}$. Then we report the sum of weights of all nodes within range $(y_L,y_R)$ in $T_{x_l}$ and $T_{x_r}$ respectively, and the difference of the two weight sums is the answer. Two independent binary searches costs work $O(\log n)$ respectively, and reporting the answer for y-coordinate in each tree costs work $O(\log n)$. Thus total cost of a single query is $O(\log n)$.


==> proof.tex <==
\section{Proof}
\label{sec:proof}
The work and span of \union{} on two treaps has been proven by \cite{BR98}. In this section we give a new proof working for all the four balance schemes. Here for \difference($T_1,T_2$) we assume that we are always returning keys in $T_1$ without in $T_2$. Also, assume $|T_1|=m$ and $|T_2|=n$.

To show the work of \union{}, \intersect{} and \difference{}, we first give some definitions and lemmas.

\hide{
We use $W(m,n)$ to denote the work and depth of \union{} two trees $T_1$ and $T_2$ of size $m$ and $n$, where $m\ge n$, and the result is denoted as $T$.
In our algorithm, the root of the smaller tree will always serve as the pivot, so the smaller tree will always be divided into two children. The work bound will stay the same if we use the root of the larger tree as the pivot (will be proved later).

Considering that the running time of the first \split and the last \join{} step is at most $2\log m$. We have:
\begin{align}
W(m,n) &\le W(m_1, n_L)+W(m_2,n_R)+2\log m\\
%D(m,n)&=\max\left(D(m_1, n_L),D(m_2,n_R)\right)+1+2\log m\\
\label{boundary1}
W(m,1)&=\log (m+1)\\
W(m,0)&=O(1)
\end{align}
, where $n_L$ is the size of the left subtree of $T_2$, and $n_R$ is the size of the right subtree, $n_L+n_R=n$. Also, $m_1$ and $m_2$ are two subtrees in $T_1$ divided by $T_2$'s root. After the algorithm goes to deep enough, the pieces of smaller tree will be of size $1$.
}

The work of a single \union{}, \intersect{} or \difference{} consists of three components: a \split{}, two recursive calls and a \join{} (or \joinTwo). We call the overall work cost by all \split{} as \emph{split work}, and call the overall work cost by all \join{} (or \joinTwo) \emph{join work}. When the recursion is at the bottommost level, which is the boundary case, it directly processes the two trees (at least one of them is empty) and returns a result. We call all the work cost by the bottommost level recursion \emph{boundary work}. The total work of a \union{}, \intersect{} or \difference{} is the sum of split work, join work and boundary work.

First consider the split work. Assume that we always use the splitting pivot from a certain tree, called the \emph{pivot tree}, and the other tree called \emph{decomposed tree}. WLOG, suppose the pivot tree is $T_2$. $T_2$ splits $T_1$ into pieces, and each key in $T_2$ will in charge of a piece in $T_1$. We define the \emph{splitting size} of a node in the pivot tree to be the size of the piece in the decomposed tree it will split. We also define a \emph{splitting tree} of the pivot tree $T_2$ to be a tree of the same shape as $T_2$, and each node is assigned a weight as the splitting size of its corresponding node in $T_2$. Figure \ref{workproof} (a) shows an example of the splitting tree. The tree is a copy of $T_2$ in shape, and $|T_1|=50$ in this example. We call this splitting tree a splitting tree over $|T_1|$. Since \union{} and \intersect{} are both symmetric, the only thing worth noting here is that in \difference{} we return the keys in the decomposed tree but not in the pivot tree.

%From the recurrence relation we can see that on each level of the smaller tree, the nodes will split the larger tree into pieces.
Roughly, $T_1$ will be split by the root of $T_2$ into two pieces, which will then be assigned to $T_2$'s two subtrees for recursive call. Then the two pieces of $T_1$ are further split into two parts respectively (four pieces in total now) and so forth.
This process will end when it reaches the leaves in $T_2$. The total split work is the sum of the log of all the splitting sizes on the splitting tree.

%The analysis of the divide-and-conquer work is equivalent to divide the number $m$ by $T_2$ from the root into pieces for each node. Notice that besides the two subproblem, the algorithm also costs $2\log m$ by \split{} and \join{}. Thus other than the cost of all boundary conditions, there will be extra cost of twice the sum of the log of the sizes of each piece in total. As shown in the figure, this is equivalent to the sum of log of all the numbers on the tree. %Since the boundary condition will cost only constant time and in total there will be at most $n/2$ leaves in $T_2$, the total cost of boundary condition is $O(n)$. The dominant part in the cost is the sum-of-log part.

\begin{figure}[!h!t]
  % Requires \usepackage{graphicx}
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/work.pdf}\\
  \caption{An illustration of the labeling in the calculation of \textal{Union} work on AVL or weight-balanced tree. The tree in (a) is $T_2$, the dashed circle denotes the exterior nodes. The number on the node is the size of the piece of $T_1$ to be split by this node, i.e., the ``splitting size'' $m_{kj}$. In (b) is an illustration of labeling.}\label{workproof}
\end{figure}

\begin{definition}
In a BST, a set of nodes $v_i$ is called a \emph{independent set} if and only if for all $v_i, v_j$ ($i\ne j$) in the set, $v_i$ is not the ancestor of $v_j$.
\end{definition}

Notice that this definition is not the conventional independent set in a tree. It requires none of the node is the \emph{ancestor} of the other one in the set, instead of parent.

\begin{lemma}
\label{lem:lessthanm}
In the pivot tree, if a set of nodes $v_i$ with splitting size $m_{i}$ is a independent set, we have $\sum_i m_{i}\le m$.
\end{lemma}

This follows directly from the definition of ``independent set''.

Now we see the splitting tree from bottom up. We group nodes from leaves upwards into ``layer''s. Denote $x_i$ as the number of nodes in layer $i$. We use $v_{kj}$ to denote the $j$-th node on layer $k$, and $m_{kj}$ to be the splitting size of $v_{kj}$, and $n_{kj}$ to be the size of the subtree rooted at $v_{kj}$. Consider when we process to node $v_{kj}$ in the splitting tree. Denote the subtree rooted at $v_{kj}$ as $T^{2}_{kj}$, and the piece in the decomposed tree it will split as $T^1_{kj}$. We should have $|T^1_{kj}|=m_{kj}$ and $|T^{2}_{kj}|=n_{kj}$.
An example is shown in Figure \ref{workproof}. Here $m_{kj}$ are shown as the number on each associate node. Denote the top layer in the tree (where the root is) as $l$. We construct layers as stated in Lemma \ref{lem:shrink}.

\begin{lemma}
\label{lem:neighbor}
In AVL, a leaf $v$ and one of its neighboring leaf will have LCA at $p(v)$ or $p^2(v)$.
\end{lemma}
\begin{proof}
It is easy to see that in an AVL, if $v$ is a leaf, it is unlikely that $p(v)$ is the only child of $p^2(v)$. Thus one of the neighboring leaf must be the child of $p(v)$ or $p^2(v)$.
\end{proof}

\begin{lemma}
\label{lem:shrink}
For AVL, red-black tree, treap and weight balanced tree, there exists a partition of tree nodes that each subset is a independent set, and if denote $x_i$ as the cardinal of set $i$, $x_i\le \frac{n}{ c^{\lfloor i/2\rfloor}}$ ($n$ is the size of the tree) holds for some constant $c>1$. We call the $i$-th set as layer $i$.% and each node in layer $i$ will be assigned a label $i$.
\end{lemma}
\begin{proof}
For all the four balancing schemes, we group those with rank $i$ in layer $i$.% For weighted-balanced trees, a node of rank $i$ will be put in layer $\lceil i \rceil$. For treaps the partition is similar as weight-balanced trees: we attach a node in layer $i$ if and only if the subtree rooted at it has size in range $[2^i,2^{i+1})$ \footnote{we use $[a,b)$ to denote $\{x|a\le x < b\}$}.

For AVL, a layer is obviously an independent set: a node and its parent cannot lies in the same layer.
%: all leaves (layer 0) in $T_2$ split $T_1$ into pieces, whose sizes sum up to at most $m$. All nodes of an upper layer than leaves, who are in layer $1$, cut $T_2$ into pieces, whose sizes sum up to at most $m$, etc.
Figure \ref{workproof} (b) shows the labeling on an AVL. Since an AVL with all leaves removed is still an AVL, Lemma \ref{lem:neighbor} directly follows that, $x_i\ge 2x_{i+2}$ in AVL. Since $x_0$ is the number of leaves, which is less than $n/2$, we can get that $x_i<\frac{n}{2^{\lfloor i/2 \rfloor}}$.

For RB trees, the number of black nodes in layer $2i$ will shrink by exactly a half than layer $2(i-1)$, and the number of red nodes in layer $2i-1$ is at most as the number of black nodes in layer $2i$ layer. Since $x_0$ is the number of exterior nodes, which are all black, $x_0\le n$. We further have $x_i<\frac{n}{2^{\lfloor i/2 \rfloor}}$.

%For weight balanced tree, we label nodes in the same way as AVL. For all nodes on layer $0$, the weight (the number of leaves) is at most one, and a node on layer $1$ has at least $\frac{1}{1-\alpha}$ leaves, and so forth - a node on layer $i$ has at least $\frac{1}{(1-\alpha)^i}$ leaves. Notice that for all nodes in the same layer, the subtrees do not intersect with each other. Considering that the number of leaves is at most $n$, we have $x_i\le (1-\alpha)^i n$.

For WB trees, if a node $v$ has the subtree weight of $N$, its parent $p(v)$ will have a tree size at least $N/\alpha>2N$, and they must be in different layers. Thus a layer is obviously a independent set, and the subtrees rooted at the nodes in one layer do not intersect with each other. Considering that there are at most $n$ leaves in total, and a node at layer $i$ has at least $\left(\frac{1}{\alpha}\right)^i$ leaves, we have $x_i\le \alpha^in$.

For treaps, we define a \emph{layer root} as those who has no ancestors in the same layer with it. In the following we discuss the layer roots in layer $i$ instead of all nodes in layer $i$, so that all layer roots in layer $i$ form an independent set (i.e., $x_i$ is the number of layer roots in layer $i$ instead of all nodes, $v_{kj}$ counts only the layer roots, etc.). Obviously, $x_i\le \frac{n}{2^i}$. Another observation is that all subtrees in the same layer should be a chain (a node should be on layer $i+1$ if both children are on layer $i$). Assume the chain rooted at $v_{kj}$ has length $l_{kj}$. In the following we will show $l_{kj}$ is a constant on expectation.

Thus for AVL trees, red-black trees, treaps and weight-balanced trees, we can find a valid partition s.t. $x_i\le \frac{n}{ c^{\lfloor i/2\rfloor}}$.
\end{proof}

\begin{lemma}
\label{lem:treapchain}
For treaps, the expected value of $l_{kj}$ (the length of the chain rooted at $v_{kj}$ in each level) is less than a constant. All the random variables $l_{kj}$ are i.i.d.
\end{lemma}
\begin{proof}
For $v_{kj}$ on layer $k$, who has a subtree of size $N\in[2^k,2^{k+1})$. The probability that $l_{kj}\ge 2$ is equal to the probability that one of its grandsons has subtree size at least $2^k$. This probability $P$ is:

\begin{align}
P&=\frac{1}{2^k}\sum_{i=2^k+1}^{N}\frac{i-2^k}{i}\\
&\le\frac{1}{2^k}\sum_{i=2^k+1}^{2^{k+1}}\frac{i-2^k}{i}\\
%&=1-\sum_{i=2^k+1}^{2^{k+1}}\frac{1}{i}\\
&\approx 1-\ln 2
\end{align}
We denote $1-\ln 2$ as $p_c$. Similarly, the probability that $l_{kj}\ge 4$ should be less than $p_c^2$, and the probability shrink geometrically as $l_{kj}$ increase. Thus the expected value of $l_{kj}$ is a constant.

Since treap comes from a random permutation, it is obviously that all $l_{kj}$ are i.i.d.
\end{proof}

\begin{theorem}
\label{thm:workofsplit}
The split work in \union{}, \intersect{} and \difference{} on two trees of size $m$ and $n$ is $O\left(N\log(\frac{M}{N}+1)\right)$ if one tree always serves as the pivot tree. Here $N=\min(n,m)$ and $M=\max(n,m)$.
\end{theorem}
\begin{proof}
The total work of \split{} is the sum of log of all the splitting sizes on the splitting tree. Assume the tree of size $n$ is the splitting tree. Notice that from Lemma \ref{lem:shrink} we know that $x_k\le \frac{n}{ c^{\lfloor i/2\rfloor}}$. Applying the concavity of $\log$ function, and considering that $\sum_{j}m_{kj}\le m$ holds for all $k$, we can get whole work is:

Also, notice that in the splitting tree, each level there are at most $m$ nodes with weight $m_{kj}>0$. Since those nodes with splitting sizes of $0$ will not cost any work, we can assume $x_i\le m$.
\begin{align}
\label{workequation}
\sum_{k=0}^{l} \sum_{j=1}^{x_k} \log (m_{kj}+1) &\le  \sum_{k=0}^{l} x_k \log (\frac{\sum_j m_{kj}+1}{x_k})\\
&=\sum_{k=0}^{l} \log\left(\frac{m}{x_k}+1\right)
\end{align}
If $m\ge n$ we have:
\begin{align}
\nonumber
&\sum_{k=0}^{l} x_k \log (\frac{m}{x_k}+1)\\
\nonumber
&{\rm{(Applying~Lemma~\ref{lem:shrink}~and~the}}\\
\nonumber
&{\rm{monotonously~increasing~of}} f(x)=x\log {m\over x} {\rm{)}}\\
\nonumber
\le &\sum_{k=0}^{l} \frac{n}{c^{\lfloor k/2 \rfloor}} \log (\frac{m}{n/c^{\lfloor k/2 \rfloor}}+1)\\
\nonumber
\le & 2\sum_{k=0}^{l/2} \frac{n}{c^k} \log (\frac{m}{n/c^k})\\
\nonumber
\le& 2\sum_{k=0}^{l/2} \frac{n}{c^k} \log \frac{m}{n}+2\sum_{k=0}^{l/2} k\frac{n}{c^k}\\
\nonumber
=& O(n\log(\frac{m}{n}+1))+O(n)\\
\label{eq:mlargern}
=&O(n\log(\frac{m}{n}+1))
\end{align}
%Here we use the concavity of function $\log$, and $f(x)=x\log \frac{m}{x}$ monotonously increases when $x<m$.

If $m<n$, we have:
\begin{align}
\nonumber
&\sum_{k=0}^{l} x_i \log (\frac{m}{x_i}+1)\\
\nonumber
&{\rm{(Applying~Lemma~\ref{lem:shrink}~and~the}}\\
\nonumber
&{\rm{monotonously~increasing~of}} f(x)=x\log {m\over x} {\rm{)}}\\
%\nonumber
%\le & 2\sum_{k=0}^{l/2} x_i \log (\frac{m}{x_i}+1)\\
\nonumber
\le & \sum_{k=0}^{2\log n/m} m \log (\frac{m}{m}+1) + \sum_{k=2\log n/m}^{l} \frac{n}{c^{\lfloor k/2 \rfloor}} \log (\frac{m}{n/c^{\lfloor k/2 \rfloor}}+1)\\
\nonumber
\le & O(m\log \frac{n}{m}) + \sum_{k=\log n/m}^{l/2} \frac{n}{c^k} \log (\frac{m}{n/c^k}+1)\\
\nonumber
\le& O(m\log \frac{n}{m}) + 2\sum_{k'=0}^{\frac{l}{2}-\log \frac{n}{m}} \frac{m}{c^{k'}} \log c^{k'}\\
%\nonumber
%=& O(m\log(\frac{n}{m}))+O(m)\\
\label{eq:nlargerm}
=&O(m\log(\frac{n}{m}+1))
\end{align}

Thus the conclusion of the two cases $m\ge n$ (Equation \ref{eq:mlargern}) and $n>m$ (Equation \ref{eq:nlargerm}) are consistent. Suppose $m$ is the size of the larger tree and $n$ is the smaller tree, the work of \split{} in \union{}, \intersect{} and \difference{} is $O\left(N\log(\frac{M}{N}+1)\right)$.

For treap, the calculation above only includes the log of splitting size on layer roots. We need to further prove the total sum of the log of all splitting size is still $O(n\log(\frac{m}{n}+1))$ under big $O$ notation.

We re-calculated the expectation as:
\begin{align*}
\mathbb{E}\left[2\sum_{k=0}^{l} \sum_{j=1}^{x_k} l_{kj}\log (m_{kj}+1)\right]=&\mathbb{E}[l_{kj}]\times2\sum_{k=0}^{l} \sum_{j=1}^{x_k} \log (m_{kj}+1)\\
=&O(n\log(\frac{m}{n}+1))
\end{align*}
Here we applied that $l_{kj}$ are i.i.d. with expected value of a constant.

To conclude, if one tree always serves as the pivot tree, the total split work of \union{}, \intersect{} or \difference{} on two trees of size $m$ and $n$ is $O\left(N\log(\frac{M}{N}+1)\right)$ where $N=\min(n,m)$ and $M=\max(n,m)$.
\end{proof}

\begin{theorem}
\label{thm:workofboundary}
The overall boundary work in \union{}, \intersect{} or \difference{} on two trees of size $m$ and $n$ is $O(\min(m,n))$.
\end{theorem}
\begin{proof}
Notice that the cost of the boundary condition on each leaf is $O(1)$. Also, if the splitting size on a node in the splitting tree is $0$, it will not go further down. If the smaller tree is the pivot tree, there are at most $\min(n,m)$ leaves. Thus the total boundary cost is $O(\min(n,m))$. If the larger tree is the pivot tree, we remove all nodes with splitting size $0$. The remaining tree has at most $\min(n,m)$ leaves, which are the boundary conditions. The overall boundary cost is also $O(\min(n,m))$.
\end{proof}

\begin{lemma}
\label{lem:sumlog}
If $T$ is an AVL tree, RB tree, WB tree or treap, $\sum_{T'\subseteq T}\log |T'| = O(|T|)$. Here $T'\subseteq T$ means $T'$ is a subtree rooted at some node in $T$. This holds on expectation for treaps.
\end{lemma}
\begin{proof}
Assume $|T|=n$. Considering each subtree in a balanced BST is also a valid balanced BST, we have $r(T')=\Theta(\log |T'|)$. Notice that in the tree there are $x_i$ nodes with rank $i$, and from Lemma \ref{lem:shrink} we know that $x_i\le n/c^{\lfloor k/2 \rfloor}$ nodes with rank $i$. The total result is $\sum_{T'\subset T}\log |T'|\le O(\sum_{T'\subset T}r(T')) \le O(\sum_{i=1}^{l}i\cdot\frac{n}{c^{\lfloor k/2 \rfloor}})=O(n)$.
\end{proof}

\begin{theorem}
The total work of \union{}, \intersect{} or \difference{} on two trees $T_1$ (decomposed tree) and $T_2$ (pivot tree) of size $m$ and $n$ is $O\left(n\log(\frac{m}{n}+1)\right)$ if $m\ge n$.
\end{theorem}
\begin{proof}
If $m\ge n$, according to Theorem \ref{thm:workofsplit} and \ref{thm:workofboundary}, the split work and the boundary work is $O\left(n\log(\frac{m}{n}+1)\right)$.

If the smaller tree is the pivot tree, the join work in each step is at most $O(\log m_{kj}+\log n_{kj})$. The $\log m_{kj}$ part has the cost same as the \split{} cost. The $n_{jk}$ part, from Lemma \ref{lem:sumlog}, is at most $O(n)$. Thus the total work is at most $O\left(n\log(\frac{m}{n}+1)\right)$.
\end{proof}

\begin{lemma}
\label{lem:treapconstant}
For treaps, when \union{}$(T_1,T_2)$, if $T_2$'s root is the pivot and $|T_2|>|T_1|$, the final \join{} step takes constant work on expectation.
\end{lemma}
\begin{proof}
The root of $T_2$ has the highest priority among those $|T_2|$ keys, so on expectation it takes the $\frac{|T_2|+|T_1|}{|T_2|}\le 2$-th place among all the $|T_1|+|T_2|$ keys. From Lemma \ref{lem:treap} we know that the cost on expectation is at most ($\log 2+1$), which is a constant.
\end{proof}

\begin{lemma}
\label{lem:AVLRBranksum}
Assume $r(T_1)< r(T_2)$. For $T=$\union$(T_1,T_2)$ on AVL, RB or WB trees, if the pivot is the root of $T_2$, $r(T)\le r(T_1)+r(T_2)$.
\end{lemma}
\begin{proof}
For AVL and RB trees we induce on $r(T_1)+r(T_2)$. When $r(T_1)+r(T_2)=1$ the conclusion is trivial. If $r(T_1)=r(T_2)=r$, the two recursive \union{} will get two trees of rank at most $2r-1$, and the result of \join{} the two trees will of height at most $2r$ (applying Lemma \ref{lem:AVL}). If $r=r(T_1)>r(T_2)$, and the pivot is $k(T_1)$, $T_1$ will be split into two subtrees, with height at most $r(T_1)-1$. $T_2$ will be split into two parts with height at most $r(T_2)$. From the inductive hypothesis, the two recursive call will get two trees of height at most $r(T_1)-1+r(T_2)$. The result of the final \join{} is at most $r(T_1)+r(T_2)$.

For WB trees, $|T|\le |T_1|+|T_2|\le 2|T_1|$. Thus $r(T)\le r(T_1)+1 \le r(T_1)+r(T_2)$.
\end{proof}
\hide{
\begin{lemma}
\label{lem:WBconstant}
For WB trees, if the larger tree is the pivot tree, the ranks of the two recursive call result trees differs by at most a constant, and the work of \join{} them is a constant.
\end{lemma}
\proof{} If the larger tree is the pivot tree, we assume the two subtrees of it have sizes $s_1$ and $s_2$, where $s_1\ge s_2$. We have $s_1\le \frac{1-\alpha}{\alpha}s_2$. Also, assume the smaller tree has size $s_3$, we have $s_3\le s_1+s_2$. The size of the result of the recursive call is at least $s_2$, and at most $s_1+s_3\le\frac{3-2\alpha}{\alpha}s_2$. The difference between the ranks of the two recursive calls is at most $\log \frac{3-2\alpha}{\alpha}$, which is a constant. According to Lemma \ref{lem:wbvalid}, the cost of \join{} them is a constant.
\qed
}
\begin{theorem}
\label{thm:joinlarger}
The join work of \union{}, \intersect{} or \difference{} on two trees $T_1$ (decomposed tree) and $T_2$ (pivot tree) of size $m$ and $n$ is at most as large as the work of \split{} if $m < n$.
\end{theorem}
\begin{proof}
When processing node $v_{kj}$ in the pivot tree ($T_2$), the split work is $\log m_{kj}$. We then prove the join work on this point is less than that.

For \intersect{} or \difference{}, the cost of \join{} (or \joinTwo{}) is at most $\log m_{kj}$ since the result tree $T$ of intersection (or difference) $T_1$ and $T_2$ should satisfy $T\subseteq T_1$. Thus the join work is at most as large as the work of \split{}.

For \union{}, if $r(T^1_{kj})\ge r(T^2_{kj})$, the \join{} will cost $O(r(T^1_{kj}))=O(\log m_{kj})$, which is the same as the cost of \split.
Assume $r(T^1_{kj})< r(T^2_{kj})$. For AVL, RB or WB trees, the subtree $T^2_{kj}$ in the pivot tree will always break into two subtrees, whose ranks differ from $r(T^2_{kj})$ by at most a constant. Thus the ranks of the two subtrees differ from each other by at most a constant.
According to Lemma \ref{lem:AVLRBranksum}, the rank of the two return trees of the two recursive calls will differ by at most $O(r(T^1_{kj}))=O(\log m_{kj})$. Thus the join cost is $O(\log m_{kj})$, which is no more than split work. For treaps, if $r(T^1_{kj})< r(T^2_{kj})$, which means $m_{kj}<n_{kj}$, according to Lemma \ref{lem:treapconstant}, the \join{} work is only a constant.% For WB trees, according to Lemma \ref{lem:treapconstant} and Lemma \ref{lem:WBconstant}, the \join{} work is only a constant. Thus the join work is at most the same as the split work.
\end{proof}

\begin{theorem}
\label{thm:mainworklarger}
The total work of \union{}, \intersect{} or \difference{} on two trees $T_1$ (decomposed tree) and $T_2$ (pivot tree) of size $m$ and $n$ is $O\left(m\log(\frac{n}{m}+1)\right)$ if $m < n$.
\end{theorem}
\proof{} This could be induced by Theorem \ref{thm:workofsplit}, \ref{thm:workofboundary} and \ref{thm:joinlarger}. \qed

\begin{theorem}
\label{thm:mainwork}
The total work of \union{}, \intersect{} or \difference{} on two trees of size $m$ and $n$ ($m\ge n$) is $O\left(n\log(\frac{m}{n}+1)\right)$ if the one tree always serves as the pivot tree.
\end{theorem}

\begin{theorem}
\label{thm:mainspan}
The span of \union{} and \intersect{} or \difference{} is $O(\log n \log m$). Here $n$ and $m$ are the sizes of the two tree, and $n\le m$.
\end{theorem}
\begin{proof}
For the span of these algorithms, we denote $D(h_m,h_n)$ as the span to union two trees of height $h_m$ and $h_n$, where $h_m\ge h_n$. If the smaller tree is the pivot tree, the split and join will both take time $h_m$. As the smaller tree will always be split into two subtrees, we have:
$$D(h_m,h_n)\le D(h_m,h_{n}-1)+2h_m$$
Thus $D(h_m,h_n)\le 2h_m h_n=O(h_nh_m)=O(\log n \log m)$.

If the larger tree is the pivot tree, as the \join{} work will be no more than \split{} work, by similar analysis, we can find that the overall span is still $O(\log n \log m)$.
\end{proof}

\hide{
\begin{figure}
\small
\begin{lstlisting}
joinRightRB$(\Tl,k,\Tr)$ =
  ($l,k',c$)=expose($\Tl$);
  if ($r(c) = r(\Tr)$) and ($c$.color=black) then
    $k$.color=red;
    $\node(l,k',\node(c,k,\Tr))$;
  else
    $T'$ = joinRight$(c,k,\Tr)$;
    $(l_1,k_1,r_1)$ = expose$(T')$;
    $(l_2,k_2,r_2)$ = expose$(r_1)$
    $T''$ = $\node$($l, k', T'$);
    if ($k_1$.color=red) and ($k_2$.color=red) then
    $k_2$.color=black;
    rotateLeft$(T'')$
    else $T''$@\vspace{.1in}@
joinRB$(\Tl,k,\Tr)$ =
  if $r(\Tl) > r(\Tr)+1 $ then joinRight$(\Tl,k,\Tr)$
  else if $r(\Tr) > r(\Tl) + 1$ then joinLeft$(\Tl,k,\Tr)$
  else $\node(\Tl,k,\Tr)$
\end{lstlisting}
\caption{RB \join{} algorithm.}
\label{fig:rbjoin}
\end{figure}
}

\hide{
\begin{figure}
\small
\begin{lstlisting}
joinRightRB$(\Tl,k,\Tr)$ =
  if ($r(\Tl) = \lfloor r(\Tr)/2 \rfloor\times 2$) then
    $\node(\Tl,\left<k,\texttt{red}\right>,\Tr)$;
  else
    $(L',\left<k',c'\right>,R')$=expose($\Tl$);
    $T'$ = $\node(L', \left<k',c'\right>$,joinRightRB$(R',k,\Tr))$;
    if ($c'$=black) and ($c(R(T'))=c(R(R(T')))$=red) then
      $c(R(R(T')))$=black;
      $T''$=rotateLeft$(T')$
    else $T''$@\vspace{.1in}@
joinRB$(\Tl,k,\Tr)$ =
  if $\lfloor r(\Tl)/2 \rfloor > \lfloor r(\Tr)/2 \rfloor$ then $T'=$joinRightRB$(\Tl,k,\Tr)$;
    if ($c(T')$=red) and ($c(R(T'))$=red) then
      $\node(L(T'),\left<k(T'),\texttt{black}\right>,R(T'))$
    else $T'$
  else if $\lfloor r(\Tr)/2 \rfloor > \lfloor r(\Tl)/2 \rfloor$ then $T'=$joinLeftRB$(\Tl,k,\Tr)$;
    if ($c(T')$=red) and ($c(L(T'))$=red) then
      $\node(L(T'),\left<k(T'),\texttt{black}\right>,R(T'))$
    else $T'$
  else if ($c(\Tl)$=black) and ($c(\Tr)$=black) then
    $\node(\Tl,\left<k,\texttt{red}\right>,\Tr)$
  else $\node(\Tl,\left<k,\texttt{black}\right>,\Tr)$
\end{lstlisting}
\caption{RB \join{} algorithm.}
\label{fig:rbjoin2}
\end{figure}

\begin{figure}
\small
\begin{lstlisting}
joinRightWB$(\Tl,k,\Tr)$ =
  ($l,k',c$)=expose($\Tl$);
  if (balance($|\Tl|,|\Tr|$) then $\node(\Tl,k,\Tr))$;
  else
    $T'$ = joinRightWB$(c,k,\Tr)$;
    $(l_1,k_1,r_1)$ = expose$(T')$;
    if balance$(|l|,|T'|)$ then $\node$($l, k', T'$)
    else if (balance$(|l|,|l_1|)$) and (balance$(|l|+|l_1|,r_1)$) then
      rotateLeft($\node$($l, k', T'$))
    else rotateLeft($\node$($l,k'$,rotateRight$(T')$))@\vspace{.1in}@
joinWB$(\Tl,k,\Tr)$ =
  if heavy($\Tl, \Tr$) then joinRightWB$(\Tl,k,\Tr)$
  else if heavy($\Tr,\Tl$) then joinLeftWB$(\Tl,k,\Tr)$
  else $\node(\Tl,k,\Tr)$
\end{lstlisting}
\caption{WB \join{} algorithm.}
\label{fig:wbjoin}
\end{figure}

\begin{figure}
\small
\begin{lstlisting}
joinTreap$(\Tl,k,\Tr)$ =
  ($l_1,k_1,r_1$)=expose($\Tl$);
  ($l_2,k_2,r_2$)=expose($\Tr$);
  if prior($k_1, k$) and prior($k_1,k_2$) then
    $\node$($l_1,k_1$,joinTreap$(r_1,k,\Tr)$)
  else if prior($k_2,k$) and prior($k_2$,$k_1$) then
    $\node$(joinTreap($\Tl,k,l_2$),$k_2,r_2$)
  else $\node(\Tl,k,\Tr)$
\end{lstlisting}
\caption{Treap \join{} algorithm.}
\label{fig:treapjoin}
\end{figure}
} 

==> related_.tex <==
\section{Related Work}
\label{sec:related}

There has been significant work on solving computational geometry problems using tree structures.
Range trees~\cite{bentley1979decomposable} and segment trees\footnote{Many data structures are referred to as segment trees~\cite{bentley1980optimal,de2000computational} for various of segment query problems, but are not identical in low-level details (e.g., how to organize segments in tree nodes, etc.).
The common theme is that on the top level the whole interval is all partitioned hierarchically.}~\cite{bentley1980optimal} have been extensively studied in research papers \cite{bentley1979data,pagel1993towards,blankenagel1994external} and introduced in textbooks~\cite{de2000computational,samet1990design}.
In distributed systems,there has also been work studying range trees \cite{agarwalparallel} and segment trees~\cite{zheng2006distributed}.
In parallel settings, Atallah et al.~\cite{Atallah89} propose cascading divide-and-conquer scheme for solving many computational geometry problems in parallel. The approach is complicated and likely very hard to implement in code.

Many previous results focus on developing fast sweepline algorithms on specific problems such as ~\cite{arge2005cache,arge2006simple,mehlhorn1994implementation,chazelle1992optimal,fortune1987sweepline,jin2006sweepline,vzalik2005efficient,domiter2008sweep,nurmi1985fast}. All of the mentioned work is are in the sequential setting.
There are also papers making effort to parallelize the sweepline algorithms. Goodrich et al.~\cite{goodrich1996sweep} propose a framework to parallelize several sweepline-based algorithms. Instead of using a vertical line sweeping over the plane, they use a moving point around a planar subdivision. McKenney and McGuire~\cite{mckenney2009parallel} propose parallel sweepline algorithms by segmenting the input into stripes. No theoretical bound is provided in this paper. Besides, the optimizations are specific for their tested problem, and do not scale on large number of threads.


\begin{SCtable}
  \centering\small
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \multicolumn{ 2}{|c|}{} & \multicolumn{ 2}{c|}{\textbf{Build}} & \multicolumn{ 2}{c|}{\textbf{Query}} \\
\cline{3-6}
 \multicolumn{ 2}{|c|}{} &       \textbf{Work} &      \textbf{Depth} &  \textbf{Query-all} &  \textbf{Query-sum} \\
\hline
     \textbf{Range} & \textbf{RangeSweep} & $O(n\log n)$ & $\tilde{O}(n^{-\epsilon})$ & $O(\log^2 n+k)$ & $O(\log^2 n)$ \\
%\cline{2-6}
     \textbf{Query} &  \textbf{RangeTree} & $O(n\log n)$ & $O(\log^3 n)$ & $O(k\log (n/k+1)))$ & $O(\log n)$ \\
\hline
   \multirow{2}{*}{\textbf{Segment}} &   \textbf{SegSweep} & $O(n\log n)$ & $\tilde{O}(n^{-\epsilon})$  & $O(\log n+k)$ & $O(\log n)$ \\
%\cline{2-6}
     \multirow{2}{*}{\textbf{Query}} &    \textbf{SegTree} & $O(n\log n)$ & $O(\log^3 n)$ & $O(\log n + k)$ & $O(\log^2 n)$ \\
%\cline{2-6}
           &   \textbf{SegCount} & $O(n\log n)$ & $O(\log^3 n)$ &          - & $O(\log^2 n)$ \\
\hline
\end{tabular}
  \caption{\par Theoretical (asymptotical) costs of all tested functions. $n$ is the input size. $k$ is the output size. $\epsilon<1$ can be any given constant.}\label{tab:allexpcost}\vspace{-.7em}
\end{SCtable} 

==> related__.tex <==
\section{Related Work}
\label{sec:related}

There has been significant work on solving computational geometry problems using tree structures.
Range trees~\cite{bentley1979decomposable} and segment trees\footnote{Many data structures are referred to as segment trees~\cite{bentley1980optimal,de2000computational} to address various versions of segment query problems, but are not identical in low-level details (e.g., how to organize segments in tree nodes, etc.).
The common theme in these trees is that on the top level the whole interval is all partitioned hierarchically.}~\cite{bentley1980optimal} have been extensively studied in research papers \cite{bentley1979data,pagel1993towards,blankenagel1994external} and have been introduced in many textbooks~\cite{de2000computational,samet1990design}.
For distributed systems there has also been work involving range trees \cite{agarwalparallel} and segment trees~\cite{zheng2006distributed}.
Atallah et al.~\cite{Atallah89} propose a cascading divide-and-conquer scheme for solving many computational geometry problems in parallel, which is quite complicated and very unlikely to be implemented by code.

Many of the previous results focus on developing fast sweepline algorithms for specific problems such as range queries~\cite{arge2005cache,arge2006simple}, segment intersection~\cite{mehlhorn1994implementation,chazelle1992optimal}, Voronoi diagrams~\cite{fortune1987sweepline,jin2006sweepline}, Delaunay triangulation~\cite{vzalik2005efficient,domiter2008sweep}, and many more~\cite{nurmi1985fast}. All of the mentioned work is only concerned about the
sequential setting. There are also papers which have made effort to parallelize such sweepline algorithms. Goodrich et al.~\cite{goodrich1996sweep} propose a framework to parallelize several sweepline-based algorithms. Instead of using a vertical line, sweeping over the plane, they use a moving point around a planar subdivision. McKenney and McGuire~\cite{mckenney2009parallel} propose parallel sweepline algorithms by segmenting the input into stripes. However, no theoretical bounds are provided in this paper. Moreover, the optimizations are specific for their tested problem and do not scale on a large number of threads.


\begin{SCtable}
  \centering\small
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 \multicolumn{ 2}{|c|}{} & \multicolumn{ 2}{c|}{\textbf{Build}} & \multicolumn{ 2}{c|}{\textbf{Query}} \\
\cline{3-6}
 \multicolumn{ 2}{|c|}{} &       \textbf{Work} &      \textbf{Depth} &  \textbf{Query-all} &  \textbf{Query-sum} \\
\hline
     \textbf{Range} & \textbf{RangeSweep} & $O(n\log n)$ & $\tilde{O}(n^{-\epsilon})$ & $O(\log^2 n+k)$ & $O(\log^2 n)$ \\
%\cline{2-6}
     \textbf{Query} &  \textbf{RangeTree} & $O(n\log n)$ & $O(\log^3 n)$ & $O(k\log (n/k+1)))$ & $O(\log n)$ \\
\hline
   \multirow{2}{*}{\textbf{Segment}} &   \textbf{SegSweep} & $O(n\log n)$ & $\tilde{O}(n^{-\epsilon})$  & $O(\log n+k)$ & $O(\log n)$ \\
%\cline{2-6}
     \multirow{2}{*}{\textbf{Query}} &    \textbf{SegTree} & $O(n\log n)$ & $O(\log^3 n)$ & $O(\log n + k)$ & $O(\log^2 n)$ \\
%\cline{2-6}
           &   \textbf{SegCount} & $O(n\log n)$ & $O(\log^3 n)$ &          - & $O(\log^2 n)$ \\
\hline
\end{tabular}
  \caption{\par Theoretical (asymptotical) costs of all tested functions. $n$ is the input size. $k$ is the output size. $\epsilon<1$ can be any given constant.}\label{tab:allexpcost}\vspace{-.7em}
\end{SCtable} 


==> rt-exp.tex <==
\subsection{Range Trees}
We tested our 2D range tree as described in Section \ref{sec:rangetreeapp}. We tested the build time on various input sizes and various number of processors as well as the corresponding query time. We accumulate the query time on $10^6$ queries, and for parallel version we just run all the queries in parallel. For all the results, we ran $20$ iterations and took the median. A brief summary of running time is in Table \ref{tab:rt-exp}.

\begin{figure*}[!h!t]
\begin{tabular}{ccc}
    \includegraphics[width=0.66\columnwidth]{figures/rt/rt-parallel.pdf} &  \includegraphics[width=0.66\columnwidth]{figures/rt/rt-speedup.pdf} &
    \includegraphics[width=0.66\columnwidth]{figures/rt/rt-cgal.pdf}\\
  (a) & (c) & (e)\\
      \includegraphics[width=0.66\columnwidth]{figures/rt/rt-parallel2.pdf}
       & \includegraphics[width=0.66\columnwidth]{figures/rt/rt-speedup2.pdf} &
       \includegraphics[width=0.66\columnwidth]{figures/rt/rt-cgal2.pdf}  \\
  (b) & (d) & (f)\\
\end{tabular}
\vspace{-0.2in}
  \caption{The performance of the range tree implemented with PAM interface. Figure (a) and (b) are results on different sizes on 144 threads. Figure (a) shows the running time on construction (left y-axis) and queries (right y-axis) respectively. The left y-axis in Figure (b) shows the number of input entries the construction function processes per microsecond. The right y-axis in Figure (b) shows the number of queries processed per microsecond. Figure (c) shows the speedup on various numbers of threads with $10^8$ points in the tree. Figure (d) shows the number of processing rate in the same setting as Figure (c). Figure (e) and (f) compare the sequential performance of our range tree implemented with PAM interface with the range tree implementation in CGAL library on different input sizes. Figure (e) compares the running time, and Figure (f) shows the processing rate. }\label{fig:rangetree}
\end{figure*}


Figure \ref{fig:rangetree} (a) and (b) show the result on input sizes varying from $10^4$ to $10^8$ on all 72 cores. It only took less than $6$ seconds to build a tree on $100$ million points, which means about $17.8$ input entries per microsecond. When the input size is as small as $1$ million, the number of entries it processes per microsecond can be about $24.4$. As the input size increases, the process ability revealed a trend of gradual decrease, but not significantly. When the input size increases a hundred-fold, the input entries processed in unit time only reduce by about 28\%. For queries, the time required per query increases as the tree getting larger. Even when the tree size is as large as $10^8$, the PAM range tree can process $1.55$ million queries per second.

Figure \ref{fig:rangetree} (c) and (d) shows the result on various numbers of threads of our range tree on $10^8$ points. Figure \ref{fig:rangetree} (c) demonstrates the speedup. The queries are just ran independently in parallel, and the speedup is almost perfectly-linear. On $144$ threads (all $72$ cores with hyper-threads) the speedup can get up to $100$. The building process, which mainly uses a divide-and-conquer scheme, gets almost-linear speedup when less than $64$ cores are involved, and hardly increases after that. On $144$ threads the speedup is up to $50$. Figure \ref{fig:rangetree} (d) shows the number of entries our algorithm processes per microsecond on various number of threads, which also increases in linear speed. On all $144$ threads building rate can be about $17.77$M entries per second, and the query rate is $154.62$M queries per second.

We also compared our implementation with the range tree in CGAL library~\cite{overmars1996designing}, which is a sequential implementation of unweighted range tree. Instead of accumulate the weights in the queried window, the CGAL range tree aims at reporting the list of all the points in the range. Hence it does not store the weight of each point. As reporting the whole list of points in the range is very sensitive to the output size, and does not highlight the augmenting property of our PAM implementation, we do not compare the query time with them. Figure \ref{fig:rangetree} (e) shows the building time of PAM range tree on one core compared with CGAL range tree. Notice that our range tree also stores the weight of each point (and also, reference counting) in the tree while CGAL only stores the x- and y-coordinates, which means CGAL implementation is more space-efficient than our version. Even considering this our implementation is about half the running time of CGAL.

\begin{table}[!h!t]
  \centering
\begin{tabular}{|l||c|c||c|c||c|c|}
\hline
       &\multirow{3}{*}{\textbf{n}}&\multirow{3}{*}{\textbf{m}}& \multicolumn{2}{c||}{\textbf{1 Core}} & \multicolumn{2}{c|}{\textbf{72 Cores}} \\ \cline{4-7}
         &&  & \textbf{Time} & \textbf{Melts} & \textbf{Time}& \textbf{Melts} \\[-.05in]
          && &\textbf{(secs)}&\textbf{/sec}&\textbf{(secs)}&\textbf{/sec}\\ \hline
\textbf{PAM Build}& $10^8$& -  &   241.7  & 0.41  &  5.63 & 17.77 \\ \hline
\textbf{PAM Query}& $10^8$ & $10^6$ &  55.83  & 1.79   &  .65 &  1.55 \\ \hline
\textbf{CGAL} & \multirow{2}{*}{$10^8$} & \multirow{2}{*}{-} & \multirow{2}{*}{478.6} &\multirow{2}{*}{0.21} &\multirow{2}{*}{-}&\multirow{2}{*}{-} \\
\textbf{Build}&&&&&&\\ \hline
\end{tabular}
  \caption{The running time and process rate of the range tree implemented with PAM interface on $n$ points in the tree and $m$ queries.  The process rate
  Melts/sec (millions of elements per second) for build and queries are calculated as
   $n$/(build-time$\times 10^6$) and $m$/(query-time$\times 10^6$) respectively. On the bottom we give the result on CGAL range tree for comparisons.}\label{tab:rt-exp}
\end{table}


==> sweepline_.tex <==
\section{A Parallel Sweepline Paradigm}
\label{sec:sweepline}
A sweepline algorithm (or plane sweep algorithm) is an algorithmic paradigm that uses a conceptual sweep line to process elements in order in Euclidean space. It uses a virtual line sweeping across the plane, stopping at some points to make updates. Often the positions that the sweep line stops at are determined by the input data, e.g., the endpoints of segments. We call them the \emph{event points}, and note them as $p_i\in P$. Here we limit ourselves to cases where the events are known ahead of time. As the algorithm processing the points, a data structure $T$ is maintained and updated at each event point to track the status at that point. Sarnak and Tarjan~\cite{Sarnak86} first noticed that by being persistent, one can keep all intermediate structures $t_i\in T$ at all event points, such that they can be used for further queries.
We call them the \emph{\sweepstructure{}} at each point. In the sweepline algorithms in this paper, we adopt the same methodology, but parallelize it.
On meeting an event point $p_i$ we compute $t_i$ based on the previous structure $t_{i-1}$ and the new point $p_i$ using an \emph{update function} $h:P\times T\mapsto T$, i.e.,$t_i=h(p_i,t_{i-1})$, from an initial structure $t_0$. Because of the persistence, this function will not affect $t_{i-1}$. This update function is similar to the form of a \emph{prefix sum}. We define it in an abstraction as follows:
\mapstructure{
{\small
\centering
\begin{tabular}{|r@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }l@{ }l|}
  \hline
\textbf{Sweep} &=& \textbf{SW}&(& $\boldsymbol{P}$; \quad $\boldsymbol{\prec}$: $P\times P\mapsto \{T,F\}$; \quad $\boldsymbol{T}$; \quad $\boldsymbol{t_0\in T}$; \quad$\boldsymbol{h}:P\times T \mapsto T$ &)\\
  \hline
\end{tabular}
}}

Then the input of this sweepline paradigm would be a sequence of $p_i\in P$, and $\prec$ defines the processing order of all  $p_i$. $T$ is the type of the \sweepstructure{}, and $h$ defines the update function.
The PrefixSweep paradigm then gives a map from $P$ to $T$ which is the \sweepstructure{} at each event point.
%a sequence of \sweepstructure{}s of type $T$ and maps each input .
The computation in this equation is intuitively sequential\footnote{Although the prefix sum problem can be parallelized easily, some more complicated combine functions other than ``add'', conversional divide-and-conquer algorithm would lead to inefficient solutions.}, but in special cases we can parallelize it. Define $h^{(k)}(\{p_i\},t)$ as repeatedly applying $h$ to a sequence of points $p_i$ in turn starting from structure $t\in T$. We say $h$ can be \emph{batched} if there exist functions $\funca (\{P_i\})\mapsto T'$ that converts a sequence of points into an intermediate type $T'$, and $\funcb:T\times T' \mapsto T$ that folds some intermediate type with a \sweepstructure{}, s.t. $h^{(k)}(\{p_i\},t) = \funcb(\funca(\{p_i\}), t)$. This means that to repeatedly update a sequence of points $\{p_i\}$ onto \sweepstructure{} $t$ using $h$ is equivalent to first combining the points using $\funca$ (denoted as \emph{reduce}) and then adding that to $t$ by $\funcb$ (denoted as \emph{fold}). Then we can split the points to be processed into blocks and batch $h$ by $\funcb$ in each block to achieve parallelism. We propose a parallel paradigm to address these sweepline algorithms (see Algorithm \ref{algo:sweepline}):

\begin{algorithm}[!tp]
\label{algo:sweepline}
\fontsize{10pt}{10pt}\selectfont
\KwIn{A list $p$ of length $n$ storing all the points to be processed in order, functions $h$, $\phi$, $\rho$, the empty \sweepstructure{} $t_0$ and the number of blocks $k$}
\KwOut{A series of \rangesweep{} $t_i$.}
    \vspace{0.5em}
    \DontPrintSemicolon
    $m = \lfloor n/k \rfloor$;\\
    \lFor(*) {$i\leftarrow 0$ to $k$} { \label{line:rwstep111}
        $t'_i=\funca(p[i\times m], \dots, p[\min\{(i+1)\times m-1, n\}])$ \label{line:rwstep1e}
    }
    \lFor {$i\leftarrow 1$ to $k-1$} {\label{line:rwstep222}
        $t_{i\times m} = \funcb(t_{(i-1)\times m}, t'_{i-1})$ \label{line:rwstep2ee}
    }
    \For(*) {$i\leftarrow 0$ to $k-1$} { \label{line:rwstep333}
        $s = i\times m$; $e = \min\{s+m, n+1\}$\\
        \lFor {$j\leftarrow s$ to $e-1$} {
            $t_{j} = g(t_{j-1}, p[j])$
        }
        \label{line:rwstep3ee}
    }
    \Return {$\langle p_i \mapsto t_i:0\le i < n\rangle$}
\caption{The construction of the \rangesweep{}. The for-loops noted with $*$ can run in parallel.}
\end{algorithm}

\vspace{-1em}
\begin{enumerate}\setlength\itemsep{-.3em}
\item \textbf{Batching} (Line \ref{line:rwstep111}). We evenly split the list into $k$ blocks and build $k$ units of the intermediate type $t'_{i}\in T'$ using $\funca$ corresponds to the $k$ blocks in parallel.

\item \textbf{Sweeping} (Line \ref{line:rwstep222}) We combine these $t'_i$ in turn by $\funcb$ to get the first \sweepstructure{} $t_0,t_{m},t_{2m}\dots$ in each block. %by $t_{i\times m} = \funcb (t_{(i-1)\times m}, t'_i)$

\item \textbf{Refining}. (Line \ref{line:rwstep333} to \ref{line:rwstep3ee}) We build all the other \sweepstructure{}s based on the above-built $t_0, t_m,t_{2m}\dots$ in the corresponding blocks. All the $k$ blocks can be done in parallel. In each block, the points $p_i$ are processed in turn to update its previous \sweepstructure{} $t_{i-1}$ using $h$.
\end{enumerate}
%\vspace{-1em}
Thus we define a parallel scheme of this problem to be:\vspace{-1em}
\mapstructure{
{\small
\centering
\begin{tabular}{|r@{ }@{}c@{}@{ }c@{}@{ }c@{ }@{ }l@{ }l|}
  \hline
\textbf{ParaSweep} &=& \textbf{PS}&(& $\boldsymbol{P}$;~~ $\boldsymbol{\prec}$: $P\times P\mapsto \{T,F\}$;\quad $\boldsymbol{T}$; \quad $\boldsymbol{t_0}\in T$;\quad $\boldsymbol{T'}$;\quad $\boldsymbol{h}:P\times T \mapsto T$;\quad  $\boldsymbol{\funca}:\{P_i\}\mapsto T'$;\quad $\boldsymbol{\funcb}:T'\times T\mapsto T$ &)\\
  \hline
\end{tabular}
}}

Here $T'$ is the intermediate type. $\funca$ and $\funcb$ are defined as introduced above. In many non-trivial instantiations of this framework (especially the two in this paper), the \sweepstructure{} keeps an ordered structure tracking a some elements related to a subset of swept points, having size $O(i)$ at point $i$. The function $h$ simply updates one element (e.g., insertions or deletions) to the structure, costing $O(\log n)$ on a structure of size $n$. Such update functions can be batched using aggregate operations (e.g., \texttt{union} for insertions), which typically cost $O(m\log (n/m+1))$ on combining a bulk (type $T'$) of size $m$ with the previous \sweepstructure{} (type $T$) of size $n\ge m$. Creating a bulk of type $T'$ from a sequence of $n$ points (function $\funca$), considering the ordering, will result in a $T'$ structure of size at most $n$ and cost time $O(n\log n)$. A common setting of the related functions can be summarized as in Table \ref{tab:sweepcost}, and the corresponding bounds of the sweepline algorithm is given in Theorem \ref{thm:sweeptheory}.
\begin{SCtable}
  \centering
  \small{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Function} &$\boldsymbol{h(p,t)}$ & $\boldsymbol{\funca(s)}$ & $\boldsymbol{\funcb(t',t)}$ \\
\hline
\textbf{Work} & $O(\log |t|)$ & $O(|s|\log |s|)$ & $O(|t'|\log (|t|/|t'|+1))$\\
\hline
\textbf{Depth} & $O(\log |t|)$ & $O(\log |s|)$ & $O(\log |t|\log |t'|)$\\
\hline
\textbf{Output Size} & $O(|t|)$ & $O(|s|)$ & $O(|t'|+|t|)$\\
\hline
\end{tabular} }
  \caption{A typical setting of the function costs in a sweepline paradigm.}\label{tab:sweepcost}
\end{SCtable}

%In many non-trivial instantiations of this framework (especially the two in this paper), the \sweepstructure{} keeps an ordered set related to the event points from the beginning up to this point, having size $O(i)$ at point $i$. The update operation simply inserts or deletes of some element to the structure. Such update functions can be batched using set operations like \texttt{union} or \texttt{diff}, which means to first organize all points in each block into sets (batching), separating those triggering insertions and deletions respectively, and then combine the whole bulk into the \sweepstructure{} in the previous block (getting prefix). Considering the theoretical bounds of ordered maps mentioned in Section \ref{sec:prelim}, we an get the work and depth of the parallel paradigm as follows:
\begin{theorem}
\label{thm:sweeptheory}
For a sweepline paradigm Sweep in which the update function $h$ can be batched by $\funca$ and $\funcb$, if the bounds as shown in Table \ref{tab:sweepcost} hold, then its corresponding parallel paradigm ParaSweep in Algorithm \ref{algo:sweepline} can construct all \sweepstructure{} in work $O(n\log n)$ and depth $O(\sqrt{n}\log^{1.5}n)$.
\end{theorem}
\begin{proof}
%We adapt it to the proposed parallel paradigm, using reduce function as the set construction function on elements to be inserted and deleted separately, and the batching function to be \texttt{union} and \texttt{diff}. Then we can convert a sequential paradigm $A_S$ into a parallel one $A_P$ as follows:
\hide{
\vspace{-.5em}
\mapstructure{
{\small
\centering
\begin{tabular}{|r@{ }@{ }c@{ }@{ }c@{ }@{ }c@{ }@{ }lllllll@{ }l|}
  \hline
  $\boldsymbol{A_S}$ &=& \textbf{PS}&(& $\boldsymbol{P}$: $P_0$; & $\boldsymbol{\prec}$: $<_P$; &$\boldsymbol{T}$: $T_0$; & $\boldsymbol{h}$: insert or delete &&&&)\\
  $\Rightarrow\boldsymbol{A_P}$ &=& \textbf{PP}&(& $\boldsymbol{P}$: $P_0$; & $\boldsymbol{\prec}$: $<_P$; &$\boldsymbol{T}$: $T_0$; & $\boldsymbol{h}$: insert or delete&$\boldsymbol{T'}$: $\langle T_0, T_0\rangle$; & $\boldsymbol{\funca}$: $\rho_{0}$; &$\boldsymbol{\funcb}$: $(\langle t_I,t_D\rangle,t)\mapsto t\cup t_I \backslash t_D$ &)\\
  \multicolumn{1}{|r}{, where}&\multicolumn{11}{l|}{$T_0$ is a set of element $E$, $\boldsymbol{\funca_{0}}: \{p_i\}\mapsto \langle t_I, t_D\rangle$. $t_I$ stores all $e\in E$ to be inserted related to points in sequence $\{p_i\}$,} \\
  &&&&&&\multicolumn{5}{l}{$t_D$ for those to be deleted.}&\\
  \hline
\end{tabular}
}}}
The algorithm and its cost is analyzed as follows:
\begin{enumerate}%\setlength\itemsep{-.3em}
\item \textbf{Batching}. Build $k$ units of intermediate type $T'$ using function $\funca$ in each block in parallel. There are $k$ such structures, each of size at most $m=\lceil n/k\rceil$, so it takes work $O(2k\cdot \frac{n}{k}\log \frac{n}{k})=O(n\log \frac{n}{k})$ and depth $O(\log \frac{n}{k})$.

\item \textbf{Sweeping}. Compute $t_m,t_{2m}\dots$ by combining the intermediate result of the each block with the previous \sweepstructure{} using function $\funcb$. The size of each intermediate structure is no more than $O(n/k)$. Considering the given work bound of the function, the total work of this step is bounded by: $O\left(\sum_{i=1}^{k} t\log (\frac{im}{m} +1)\right)=O(n\log k)$. The depth is:
$O\left(\sum_{i=1}^{k}\log m \log im\right)=O(k\log \frac{n}{k}\log n)$.
%$O\left(\sum_{i=1}^{k} t\log (\frac{it}{t} +1)\right)=O\left(t\sum_{i=1}^{k} \log (i+1)\right)=O(n\log k)$
%$O\left(\sum_{i=1}^{k}\log t \log it\right)=O\left(\log t\cdot \left(k\log t+\sum_{i=1}^{k}\log i\right)\right)=O(k\log \frac{n}{k}\log n)$.
\item \textbf{Refining}. For each block, build all the other \sweepstructure{}s using the function $h$. The total work is: $c\sum_{i=1}^{n} \log i=O(n\log n)$. The depth is the cost to finish all work in one block, which is $O(\frac{n}{k}\log n)$.\vspace{-.5em}
\end{enumerate}

In total, it costs work $O(n\log n)$ and depth $O\left(\left(k\log \frac{n}{k}+\frac{n}{k}\right)\log n\right)$. When $k=\Theta(\sqrt{n/\log n})$, the depth is $O(\sqrt{n}\log^{1.5}n)$.
\end{proof}
By repeatedly applying this process to each block in the refining step, we can further reduce the depth.

\begin{corollary}
\label{coro:depth}
For a sweepline paradigm Sweep in which the update function $h$ can be batched by $\funca$ and $\funcb$, if the bounds as shown in Table \ref{tab:sweepcost} hold, then its corresponding parallel paradigm ParaSweep in Algorithm \ref{algo:sweepline} can construct all \sweepstructure{} in work $O(\frac{1}{\epsilon}n\log n)$ and depth $\tilde{O}(n^{\epsilon})$ for arbitrary small $\epsilon>0$.
\end{corollary}
We give the proof in Appendix \ref{app:rangesweepdepth}, and introduce the implementation of such a paradigm in Appendix \ref{app:sweepcode}. 

In this paper we give sweepline algorithms for range queries and segment queries. They both fit the proposed parallel paradigm, and accord with the assumption on the function cost in Theorem \ref{thm:sweeptheory}.
%In the following parts we will show how to fit the range queries and segment queries into this paradigm and develop efficient algorithms on top of that by properly defining functions $h$, $\funca$ and $\funcb$. 

==> word.tex <==
\newcommand{\cfont}[1]{\textbf{#1}}
\newcommand{\cand}{\cfont{and}}
\newcommand{\cor}{\cfont{or}}
\newcommand{\candnot}{\cfont{and-not}}

\subsection{Word Index Searching}
\label{sec:index}

Our second application of augmented trees is for building and
searching an inverted index of the kind used by search
engines~\cite{WittenMB99,rajaraman2011} (also called an inverted file
or posting file).  For a given corpus, the index stores a mapping from
words to the set of documents they appear in.  The set of documents
corresponding to a word is sometimes called a \emph{posting list}.
With such an inverted index, queries for a conjunction of words
(\cand{}) can be implemented by looking up the posting list for each
word, and then taking an intersection of the corresponding sets.
Similarly, a disjunction (\cor{}) is the union of the sets, and
difference can be used to exclude documents with a given term
(\candnot{}).  Because of the importance of inverted indices in
document and web search there has been significant research on
developing efficient implementations of set operations for this
purpose, e.g.,~\cite{barbay2006faster,Sanders07,Schlegel11,inoue2014faster}.
As discussed in previous papers, it can be important for unions and
intersections to take time that is sublinear in the sum of the sizes
since the size of the lists can be very different---e.g. consider the
lists for ``set'' (5.8 billion hits in Google) and ``cacomistle'' (54
thousand hits in Google).

%PAM is well suited for such inbalanced
%queries since the time is mostly a function of the smaller size.

It is most often useful not just to report a flat set of documents
that satisfy the query, but instead to report a reasonably small
subset of the most important documents.  Here we discuss how augmented
maps can be used to efficiently implement such queries.  The idea is
to keep a \emph{document-word weight} with each document-word pair.
This weight represents a combination of the importance of the word in
the document and the importance of the document in the corpus.  The
importance of the word in a document is often measured by the
\emph{term frequency-inverse document frequency}
(tf-idf)~\cite{rajaraman2011}, which measures how frequently a word
appears in a document relative to how frequently it appears in the
corpus as a whole.  In practice, it is also important to consider
where the word appears in a document, giving words in titles,
associated with an anchor, or near the beginning a heavier weight.
The importance of the document in the corpus can be measured by
algorithms such as pagerank~\cite{page1999pagerank}, which gives a
rank to each document in the database.  The importance of the word in
the document and document in corpus can then be combined to give an
overall document-word weight.  A zero weight is given to document-word
pairs that do not appear in the corpus so the representation can be
kept sparse.

The weights can be maintained in an inverted index by augmenting each
posting list so it is not just a set of documents, but a map from
documents to weights, and further augmenting the maps to keep the
maximum weight in the map.  When taking unions or intersections the
weights can be added for documents that appear in both sets.  The map
returned by a query is therefore a mapping from documents that satisfy
the query to weights corresponding to importance of that document
relative to the query.  In this way, returning the document with
maximum weight will return the most important document relative to the
query in constant time.  The next $k$ most important documents can be
found in $k \log n$ time ($n$ is the size of the posting list).  For
example, a query could be of the form (``posting'' \cand{} ``file'')
\cor{} (``inverted'' \cand{} ``index'') with the objective of
returning the most relevant documents.  The number of documents that
match the query could be large given that the words have multiple
meanings, but the number relevant documents might be small.

\begin{figure}[t]
{\ttfamily\small
\begin{lstlisting}[language=C++,frame=lines,escapechar=@]
struct inv_index {
  using word = char*;
  using doc_id = int;
  using weight = float;@\cspace@
  struct a_max {
    using aug_t = weight;
    static aug_t get_empty() {return 0;}
    static aug_t from_entry(doc_id k,weight v) {
      return v;}
    static aug_t combine(aug_t a, aug_t b) {
      return (b > a) ? b : a;} };@\cspace@
  using post_elt = pair<doc_id, weight>;
  using post_list = aug_map<doc_id,weight,a_max>;
  using index_elt = pair<word, post_elt>;
  using index = map<word,post_list,str_less>;
  index idx;@\cspace@
  inv_index(index_elt* start, index_elt* end) {
    auto plist= [] (post_elt* s, post_elt* e) {
      return post_list(s,e,add); };
    idx.build_reduce<post_elt>(start,end,plist);} @\cspace@
  post_list get_list(word w) {
    maybe<post_list> p = idx.find(w);
    if (p) return *p;
    else return post_list();  }@\cspace@
  post_list And(post_list a, post_list b) {
    return map_intersect(a,b,add);}@\cspace@
  post_list Or(post_list a, post_list b) {
    return map_union(a,b,add);}@\cspace@
  post_list And_Not(post_list a, post_list b) {
    return map_diff(a,b);}@\cspace@
  vector<post_elt> top_k(post_list a, int k) {
    int l = min<int>(k,a.size());
    vector<post_elt> vec(l);
    post_list b = a;
    for (int i=0; i < l; i++) {
      weight m = a.aug_val();
      auto f = [m] (weight v) {return v < m;};
      vec[i] = *b.aug_find(f);
      b.remove(vec[i].first); }
    return vec; }
};
\end{lstlisting}
}
\vspace{-0.2in}
\caption{The data structure and construction of an inverted index, and the
  query operations.}
\label{fig:index_code}
\vspace{-.2in}
\end{figure}

Figure~\ref{fig:index_code} gives the code for implementing such an
augmented map in PAM.  Words are stored as character strings
(\ctext{char *}), document identifiers are integers, and weights are
floats.  A posting list is an augmented map using the maximum of the
weights (defined in \ctext{a\_map}).  The \ctext{build\_reduce}
function builds a map from a sequence of key-value pairs (not
necessarily sorted) and uses the supplied function to combine the
values of equal keys.  In our case the documents with equal words
(keys) should be combined by creating a posting list
(\ctext{post\_list}) over them, and combining weights of equal words
within a document with \ctext{add}).

The implementation uses at least four important features of PAM.
Firstly, when taking unions and intersections it uses the combining
function to specify how the weights of the common documents that
appear in both document sets should be combined.  Secondly, augmenting
the map with the maximum weight document in the result of the query
allows it to quickly find the most important documents.  Thirdly, PAM
takes time that is mostly proportional to the smaller list, making it
efficient when the posting lists have significantly different sizes.
And, fourthly, it makes use of history persistence since the input
posting lists (maps) are not destroyed, but instead a new list is
created when applying unions or intersections.  Note that supporting
history persistence by copying both input lists would be very
inefficient if one is much larger than the other (PAM will only take
time mostly proportional to the smaller).

